FloMore: Meeting bandwidth requirements of flows

Wide-area cloud provider networks must support the bandwidth requirements of diverse services (e.g., applications, product groups, customers) despite failures. Existing traffic engineering (TE) schemes operate at much coarser granularity than services, which we show necessitates unduly conservative decisions. To tackle this, we present FloMore, which directly considers the bandwidth needs of individual services and ensures they are met a desired percentage of time. Rather than meet the requirements for all services over the same set of failure states, FloMore exploits a key opportunity that each service could meet its bandwidth requirements over a different set of failure states. FloMore consists of an offline phase that identifies the critical failure states of each service, and on failure allocates traffic in a manner that prioritizes those services for which that failure state is critical. We present a novel decomposition scheme to handle FloMore's offline phase in a tractable manner. Our evaluations show that FloMore outperforms state-of-the-art TE schemes including SMORE and Teavar, and also out-performs extensions of these schemes that we devise. The results also show FloMore's decomposition approach allows it to scale well to larger network topologies.

==> backup.tex <==
\begin{table}[t]
  %\small
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|| c || p{6cm}||} 
    \hline
      notation  & meaning\\
    \hline\hline
$Q$ & Set of all scenarios \\
$A$ & Set of applications \\
$G$ & Set of groups\\
$Q_k$ & Set of scenarios in group $k$\\
$F$ & Set of flows\\
$R(i)$ & Set of tunnels for flow $i$\\
$E$ & Set of edges\\
$d_i$ & Demand of flow $i$\\
$\beta$ & Target availability\\
$p_q$ & probability of scenario q\\
$x_{lq}$ & allocated bandwidth on tunnel $l$ in scenario $q$(routing variable)\\
$y_{lq}$ & 1 if tunnel $l$ is alive in scenario $q$, 0 otherwise\\
$t_{qi}$ & loss of flow $i$ in scenario $q$\\
$w_{qi}$ & the contribution of scenario $q$ to worst scenarios for flow $i$ \\
$\theta$ & worst cvar across flows\\
$\theta_i$ & cvar of flow $i$\\
$\alpha_i$ & dual variable, can be interpreted as 'threshold' loss between good and bad scenarios\\
$s_{qi}$ & dual variable, can be interpreted as the loss exceeding the threshold\\
$Z_{ik}$ & Bound on sum of probabilities of scenarios in group $k$ that are excluded for flow $i$(later it gets scaled by $\gamma_i$) \\
$z_{iq}$ & $w_{qi}$ scales by $\gamma_i$(the weight of flow $i$)\\
$\gamma_i$ & importance of flow $i$, can be interpreted as the probability of flow $i$ being the bottleneck. \\
    \hline    
    \end{tabular}
    }
    \caption{Notation}
    \label{tab:notations}
    \vspace{-0.3in}
\end{table}


\begin{figure*}[t]

\begin{minipage}[t]{0.3\textwidth}
	    \includegraphics[trim={7.5cm 8cm 8.1cm 5cm}, clip, width=\textwidth]{figures/graphs.001.png}
        \label{fig:flow_example}

    \vspace{-0.25in}
    \caption{Example topology where scenario-based design doesn't work well.}
        \label{fig:flow_example}
\end{minipage}\hspace{0.1in}
%
\begin{minipage}[t]{0.28\textwidth}
	    \includegraphics[ trim={7.8cm 8.5cm 10.3cm 4.1cm}, clip, width=\textwidth]{figures/graphs.002.png}
        \label{fig:flow_example_1}

    \vspace{-0.25in}
    \caption{Failure scenario where only $A-D$ link fails.}
        \label{fig:flow_example_1}
\end{minipage}\hspace{0.1in}
%
\begin{minipage}[t]{0.32\textwidth}  

    \vspace{-0.8in}
    \begin{tabular}{| c | c| c|} \hline
Scenarios & probability & loss on AC  \\
\hline
        Only AD fails & $0.997\%$ & $50\%$ \\
         \hline
        AB or BC fails                                     & $0.1999\%$ & $100\%$ \\   
        \hline
        Others & $98.8031\%$ & uncertain \\ 
        \hline
    \end{tabular}
    
        
    %\vspace{0.1in}
         \caption{Different scenarios and loss on AC flow when using Teavar or SMORE.}
        \label{fig:scenarios}
\end{minipage}\hspace{0.1in}
\end{figure*}

==> derivingRoutingMechanisms.tex <==
%\section{Deriving response mechanisms from models}

\section{Realizing \System{}'s mechanisms}
\label{sec:practical}
In this section, we discuss how to realize \System{}'s network
response mechanisms associated with the models in \S\ref{sec:system}.

First, \FFCimp{} employs \FFC{}'s response mechanism. Under any failure scenario, traffic across tunnels between a source $s$ and destination $t$ is carried on all live tunnels, and in proportion to the reservations on the tunnels. Consider three tunnels from $s$ to $t$ with reservations of $(2,3,5)$. When all the tunnels are alive, the $(s,t)$ traffic is split across the tunnels in the ratio $(0.2, 0.3, 0.5)$. If the first tunnels fails, the traffic is sent across the tunnels in the ratio $(0, \frac{0.3}{0.8}, \frac{0.5}{0.8})$.

We next discuss the response mechanisms associated with our models based on \LS{}s. 
First, we  discuss a mechanism that works for arbitrary \LS{}s (\S\ref{sec:Centralized_LS_scheme}). We then show that when \LS{}s are topologically sorted (more formally explained later), a response mechanism similar to \FFC{} may be used (\S\ref{sec:topsortls}).

%As for our \LS{} model, we claim that (i) it can be implemented as a centralized routing scheme which only requires to solve linear systems upon link failures; (ii) with an additional assumption on the choice of \LS{}s, our \LS{} model can be implemented as a distributed routing scheme which does proportional assigning traffic just as FFC does. 

\subsection{Realizing general logical sequences}
\label{sec:Centralized_LS_scheme}

\begin{figure*}[t]
%
\begin{minipage}[t]{0.95\textwidth}
  %\vspace{-0.8in}
  \includegraphics[ trim={1cm 13cm 7cm 5cm}, clip, width=\textwidth]{figures/packetrouting.pdf}
  \vspace{-0.25in}
        \label{fig:implementation_example_com}
        
         \caption{Realizing \System{} in practice. (a) Example abstract model; (b) a practical realization using only tunnels applicable for arbitrary \LS{}s (\S\ref{sec:Centralized_LS_scheme}); (c) an alternate realization when \LS{}s can be topologically sorted
         (\S\ref{sec:topsortls}).}
   
       \label{fig:implementation_example_com}
\end{minipage}\hspace{0.1in}
%
\vspace{-0.15in}
\end{figure*}

%  \begin{figure}[t]
%	\centering
        
%	    \includegraphics[ trim={3.6cm 11.6cm 12.5cm 3.3cm}, clip, width=0.45\textwidth]{figures/implementation_example.pdf}
%        \label{fig:implementation_example}

 %   \caption{A topology with 5 physical tunnels and two \LS{}s, and the associated   reservations computed by \System{}'s models.}
 %       \label{fig:implementation_example}
%\end{figure}

Consider Fig.~\ref{fig:implementation_example_com}(a) which shows the physical
tunnels and the \LS{}s used with our offline \SysLS{}, and \SysCLS{} models for
an example setting (e.g., $l1$ is a physical tunnel between $A$ and $C$, while 
$q1$ is a \LS{} between $A$ and $D$) where traffic is carried
from $A$ to $B$. These models determine the reservations associated with each tunnel, 
and each \LS{} (e.g., $a_{l1}$ and $b_{q1}$ are respectively the reservation on $l1$ and $q1$). 

We discuss an approach to realize this abstract model only using tunnels (in \S\ref{sec:topsortls}, we discuss an alternate implementation). While in \FFC{}, a tunnel $l$ from $i$ to $j$ may carry traffic only from $i$ to $j$, \System{} permits some flexibility -- e.g., $l$ may carry traffic from $s$ to $t$ if in the abstract model, $(i,j)$ is a segment in a \LS{} from $s$ to $t$.  

%Given the traffic demand, our \LS{} model tells us how to make reservations on physical tunnels and \LS{}s so that they are sufficient to serve the demand for a set of failure scenarios. Note that no matter how reservation is made on \LS{}s, it will eventually be supported by some underlying physical tunnels. Thus, to implement \LS{} model as a routing scheme, we need to figure out how much reservation we are using exactly on each physical tunnel. In other words, under a failure scenario, we need to get the value $r_{lt}$ which stands for how much each alive tunnel $l$ needs to carry for traffic destinated at $t$. Then we can normalize $r_{lt}$ and install the value as weights in the routers. Fig.~\ref{fig:implementation_example} shows an example topology and reservations on the logical sequences and physical tunnels. Suppose we are serving 1 unit of traffic from $A$ to $B$, $r_{lt}$ for each tunnel $l$ to destination $t$ is shown in the figure. 

Like \FFC{}, our models are run at the granularity of several minutes to periodically recompute reservations (e.g., to handle significant shifts in traffic demands). Once computed for a given traffic matrix, we show that the traffic carried on tunnel $l$ to destination $t$ for any failure scenario may be computed online by solving a system of linear equations, which is much faster than solving linear programs (LPs)
such as the multi-commodity flow problem (e.g., a popular approach to solving LPs involves solving  many linear systems).
%\footnote{Popular approaches to
%solving LPs involve many iterations, each of which involves solving a linear system.} 
 





In describing our approach, it is helpful to consider a matrix $M$ that summarizes the reservations. For instance, for the topology in  Fig.~\ref{fig:implementation_example_com}, the reservation matrix $M$ is summarized in Fig.~\ref{reservationMatrixFig}. Each row and column corresponds to a node pair.
%For example, the node pair $(A,B)$ is shown since it has demand, while the node pair $(A,C)$ is shown since it is used as an intermediate segment to carry traffic from $A$ to $B$. 
The diagonal entries indicate the total reservation across all live tunnels and active logical sequences associated with that node pair. A non-diagonal entry in column $i$ and row $j$ indicates 
that the node pair $j$ must carry traffic corresponding to column $i$. For instance, in the third row corresponding to the node pair $(A,D)$, the diagonal entry $a_{l3} + b_{q1}$ is the total reservation associated with that node pair (over tunnel $l3$ and \LS{} $q1$). Further, the entry $-b_{q2}$ reflects that $(A,D)$ is a segment of the \LS{} $q2$ from $A$ to $B$ and must be able to carry the reservation $b_{q2}$ associated with $q2$.


%Next, we will show how to get $r_{lt}$ from the reservations. We will represent the reservation as a matrix and solve linear systems to get $r_{lt}$. In a particular scenario $x$, let $T_x(s,t)$ denote the set of alive tunnels from $s$ to $t$ and $L_x(s,t)$ denote the set of active \LS{}s from $s$ to $t$. Let $P$ be the set of node pairs of interest. We are interested in a node pair $(s,t)$ if either there is demand from $s$ to $t$, or other node pairs with demands can indirectly route by using $(s,t)$ as an intermediate segment.\cj{Is this vague? I need this explained because it will solve the theoretical concern which Mohit raised.} For example, in Figure~\ref{fig:implementation_example}, the node pairs we are interested in are $(A,B)$ which has demand, $(A,C)$, $(C,D)$, $(A,C)$ and $(D,B)$ which be indirectly used for $(A,B)$ traffic through logical sequences. Other node pairs are not relevant to this routing. We can now describe the reservations in a matrix $M \in \mathbb{R}^{P \times P}$. Each row stands for how a node pair $ij$ services all the needs on it. The diagonal of $Mat$ is the sum of available reservations on the pair, i.e. $M_{ij, ij} = \sum_{l \in T_x(i,j)} a_{l} + \sum_{q \in L_x(i,j)}b_{q}$. And other entries of $Mat$ denote how much a node pair needs to carry for other node pairs, i.e. $M_{ij, mn} = -\sum_{q \in Q(i,j) \cap L_x(m,n)} b_{q}$ if $(i,j) \ne (m,n)$. For example, the matrix for the reservation in Figure~\ref{fig:implementation_example} can be written as


\begin{figure}[t]
\begin{align}
\begin{split}
& M_{1} = 
\begin{blockarray}{cccccc}
AC & CD & AD & DB & AB \\
\begin{block}{(ccccc)c}
  a_{l_1} & 0 & -b_{q_1} & 0 & 0 & AC \\
  0 & a_{l_2} & -b_{q_1} & 0 & 0 & CD \\
  0 & 0 & a_{l_3} + b_{q_1} & 0 & -b_{q_2} & AD \\
  0 & 0 & 0 & a_{l_4} & -b_{q_2} & DB \\
  0 & 0 & 0 & 0 & a_{l_5} + b_{q_2} & AB \\
\end{block}
\end{blockarray} \\
%& \quad \quad \quad = \begin{blockarray}{cccccc}
%AC & CD & AD & DB & AB \\
%\begin{block}{(ccccc)c}
%  1 & 0 & -1 & 0 & 0 & AC \\
%  0 & 1 & -1 & 0 & 0 & CD \\
%  0 & 0 & 2 & 0 & -1 & AD \\
%  0 & 0 & 0 & 1 & -1 & DB \\
%  0 & 0 & 0 & 0 & 2 & AB \\
%\end{block}
%\end{blockarray}
\end{split}
\nonumber
\end{align}
\vspace{-0.25in}
\caption{Reservation matrix associated with Fig.~\ref{fig:implementation_example_com}.}
\label{reservationMatrixFig}
\vspace{-0.15in}
\end{figure}

%We will represent the reservation as a matrix and solve linear systems to get $r_{lt}$. In a particular scenario $x$, let $T_x(s,t)$ denote the set of alive tunnels from $s$ to $t$ and $L_x(s,t)$ denote the set of active \LS{}s from $s$ to $t$. 
%A node pair $(s,t)$is only shown if there is demand from $s$ to $t$, or if the pair is used as an intermediate segment by other pairs.

%\cj{This is crucial to our proof. I want to have a formal definition of $P$, but it will be very technical, and I need to bring back $T_x$, $L_x$, etc. } }


A node pair $(s,t)$ is considered to be of interest if it carries positive demand, or if it carries traffic for another node pair of interest.  Let $P$ be the set of node pairs of interest (more  formally defined in the Appendix).
%We don't need to assign routing to tunnels between node pairs which are not included in $P$. \cj{this is to imply $r_{lt} = 0$, if $l\in T(i,j)$ and $(i,j)\ne P$}
%\sgr{See node pair now.}
Constraint \eqref{eq:capconstraint} in our \LS{} model can be equivalently expressed in matrix notation as $M \times \vec{1} \ge_{v} \vec{D}$. Here, $\vec{1}$ and $\vec{D}$ are $P \times 1$ column vectors. All entries of $\vec{1}$ are 1, while the $p^\text{th}$ row of $\vec{D}$ has an entry $z_pd_p$ indicating the total traffic associated with pair $p$ that can be carried. 
%
%Here, $P$ is the set of node pairs of interest, $\vec{D} \in \mathbb{R^*}^{P}$ is the demand vector where $\vec{D}_{ij}$ represents the traffic demand from $i$ to $j$. \sgr{Should we say $z_{st} d_{st}$?}. Further $\vec{1} \in \mathbb{R}^{P}$ is a vector where all entries are 1. 
%Then, our model (\eqref{eq:vs_model}) guarantees that  $M \times \vec{1} \ge_{v} \vec{D}$,
%\cj{Not sure if this is the best way mathematically.} 
%
%
Let $\vec{U}$ be a $P \times 1$ column vector. Then, we have:
%
\begin{proposition}\label{prop:linear_system}
$M$ is an invertible M-matrix\footnote{A matrix $T$ is an invertible M-matrix if $T_{ij}\le 0$ when $i\ne j$ and $Tx\ge 0$ implies that $x\ge 0$.}, and there is a unique solution $\vec{U^*}$ to the linear system $M \times \vec{U} = \vec{D}$, where $\forall (i,j) \in P$, $\vec{U^*}(i,j) \in [0,1]$.
\end{proposition}
%
We defer a proof to the appendix but discuss the implications here.
%First, while the model \eqref{eq:vs_model} precomputes the reservations, 
While \System{}'s models determine the reservations, realizing them
in practice requires determining the fraction of the reservation that is actually used in any given failure scenario. The above result indicates that such a fraction exists and may be obtained as a solution to a linear system of equations. 
While linear systems are already much faster to solve than LPs, the 
result also indicates that the matrix $M$ is of a type for which simple
and memory-efficient iterative algorithms for solving linear systems can be used~\cite{berman1994nonnegative}.

%involving matrix vector multiplications converge to the solution~\cite{berman1994nonnegative}.

%\sgr{complexity/better punchline?}

%Let $\vec{U}$ be a $P \times 1$ column vector with the $p^{th}$ row having an 
%entry $u_p$ that denotes the fraction of the reservation associated with pair $p$ that is used.
%Then, it must be the case that the following linear system of equations is satisfied
%$M \times \vec{U} = \vec{D}$. 


%The above proposition tells us that we can use the reservations proportionally in each node pair. That is, to exactly serve the demand in $\vec{D}$, all the reservations in node pair $(i,j)$ are used by the same fraction $\vec{U^*}(i,j)$. Thus, $\forall l \in T_x(i,j)$, $\vec{U^*}(i,j)a_l$ is the amount of traffic that will be carried by tunnel $l$. Since $\vec{U}(i,j) \in [0,1]$, this usage is clearly valid. Now, to get $r_{lt}$ for each destination $t$, we just need to solve one linear system for each $t$. Let $\vec{D_t}$ be the demand vector for all demands sent to $t$. From the same argument for the above proposition, we know that there is a unique solution $\vec{U_t^*}$ to the linear system $Mat \times \vec{U_t} = \vec{D_t}$ where $\forall (i,j) \in P$, $\vec{U_t^*}(i,j) \in [0,1]$. Then $\forall l \in T_x(i,j)$, $r_{lt} = \vec{U_t^*}(i,j)a_l$. \cj{sum of $u_t$ argument?}

For $t \in V$, let $\vec{D_t}$ be a $P \times 1$ column vector where the $p^{\text{th}}$ row of $\vec{D_t}$ has an entry $z_pd_p$ if $t$ is an end point of $p$, and 
0 otherwise.
%the demand vector for all demands sent to $t$. 
Using the same argument as for Proposition~\ref{prop:linear_system}, there is a unique solution $\vec{U_t^*}$ to the linear system $M \times \vec{U_t} = \vec{D_t}$.
%where $\forall (i,j) \in P$, $\vec{U_t^*}(i,j) \in [0,1]$. 
Then, the following holds:
%
\begin{proposition}\label{prop:valid_routing}
For any live tunnel 
$l$ from $i$ to $j$ and any destination $t$, let $r_{lt}=\vec{U_t^*}(i,j)a_l$ be the total traffic carried to destination $t$ on tunnel $l$. Then $r_{lt}$ represents a valid routing which carries all the traffic with the destination of $t$.
\end{proposition}
%
%To get the routing $r_{lt}$, 
%We already know that $\forall t\in V$, $M \times \vec{U_t} = \vec{D_t}$. So putting the vectors for each destination together, we will have the following linear system
We compute $U_t^*$ for every node $t$ by solving the linear system
$M \times [\vec{U_{t_1}^*},\vec{U_{t_2}^*},...\vec{U_{t_{|V|}}^*}] = [\vec{D_{t_1}},\vec{D_{t_2}},...\vec{D_{t_{|V|}}}]$
, which in turn allows $r_{lt}$ to
be computed. 
%Solving the linear system is fast, since it only requires a matrix inverse and a matrix multiplication. 
As computed, $r_{lt}$ may have cycles that can be eliminated by subtracting flow associated with the cycle. 
%
%\begin{align}
%\begin{split}
%& M \times [U_{t_1}^*,U_{t_2}^*,...U_{t_{|V|}}^*] = [D_{t_1},D_{t_2},...D_{t_{|V|}}]
%\nonumber
%\end{split}\label{eq:matrix}
%\end{align}
%
%Since $M$ is invertible, we only need to get the inverse of $M$, and compute $U_t^*$ as 
%
%\begin{align}
%\begin{split}
%& [U_{t_1}^*,U_{t_2}^*,...U_{t_{|V|}}^*] = M^{-1} \times [D_{t_1},D_{t_2},...D_{t_{|V|}}]
%\end{split}\label{eq:matrix}
%\end{align}
%
Fig.~\ref{fig:implementation_example_com}(b) shows a concrete realization of \System{}'s 
%model determined reservations with just tunnels. 
routing on tunnels for the abstract model shown in Fig.~\ref{fig:implementation_example_com}(a).
Each tunnel is annotated with the fraction of the traffic to destination B carried on that tunnel
%
%Each tunnel is associated with the fraction of the reservation on that tunnel that is used to carry traffic to destination $B$, obtained as above 
-- e.g., $r_{l5,B}=1/4$ indicates that $l5$ carries 1/4 of the traffic to $B$.

%  \begin{figure}[t]
%	\centering
        
%	    \includegraphics[ trim={3.6cm 11.2cm 22.5cm 3.3cm}, clip, width=0.25\textwidth]{figures/implementation_example_r.pdf}
%        \label{fig:implementation_example_r}

%    \caption{\System{}'s realization of the model using only tunnels.}
%
%    \caption{The routing we get from solving the linear system, which tells us that to send 1 unit of traffic from $A$ to $B$, we can send 1/2 on $l5$ directly, and send 1/4 on $l1$, $l2$ and $l3$ so that 1/2 will be sent from $A$ to $D$, then send $1/2$ on $l4$ from $D$ to $B$.
%    }
 %       \label{fig:implementation_example_r}
%\end{figure}

%\sgr{Chuan, please add a figure to replace (or compress) the text below.}

%
%Now, to get $r_{lt}$ for each destination $t$, we just need to solve one linear system for each $t$. Let $\vec{D_t}$ be the demand vector for all demands sent to $t$. From the same argument for the above proposition, we know that there is a unique solution $\vec{U_t^*}$ to the linear system $Mat \times \vec{U_t} = \vec{D_t}$ where $\forall (i,j) \in P$, $\vec{U_t^*}(i,j) \in [0,1]$. Then $\forall l \in T_x(i,j)$, $r_{lt} = \vec{U_t^*}(i,j)a_l$. \cj{sum of $u_t$ argument?} For example in Figure~\ref{fig:implementation_example}, we can write the linear system for destination $B$ as $M_1 \times \vec{U_B} = \vec{D_B}$ where $\vec{D_B}$ has $1$ in the $AB$ entry and $0$ in all other entries. Solving this linear system will give us
%
%\sgr{
%\begin{align}
%\begin{split}
%U_B^* = 
%\begin{blockarray}{cc}
%  \\
%\begin{block}{(c)c}
%  1/4 & AC\\
%  1/4 & CD\\
%  1/4 & AD\\
%  1/2 & DB\\
%  1/2 & AB\\
%\end{block}
%\end{blockarray}
%\end{split}\label{eq:matrix}
%\end{align}
%}



\subsection{Topologically sorted logical sequences}
\label{sec:topsortls}
While the approach in \S\ref{sec:Centralized_LS_scheme} works for \textit{arbitrary} \LS{}s, we next describe an alternate approach that works when \LS{}s are chosen with some restrictions. Given two \LS{}s $(i,j)$, and $(i',j')$, we say that $(i,j) > (i',j')$ if $(i',j')$ is a segment of \LS{} $(i,j)$. Our approach below is applicable if the active \LS{}s under every failure scenario can be topologically sorted with respect to relation '$>$'. For example, in Fig.~\ref{fig:implementation_example_com}, the \LS{}s satisfy a topological ordering with $q2 > q1$ since $(A,B)$ uses the segment $(A,D)$ (but not vice versa). 

When a topological ordering is possible, \System{} implements \LS{}s more directly (Fig.~\ref{fig:implementation_example_com}(c)).
When $A$ sends a packet to $B$, traffic is split across
the tunnel $l5$ and \LS{} $q1$. Traffic to $q1$ involves pushing a label, and looking up the table entry for host $D$. 
This entry indicates traffic is split across tunnel $l1$ and \LS{} $q2$. Traffic to $q2$ involves pushing another label
and looking up the entry for host $C$, which indicates the
traffic is to be forwarded on tunnel $l1$. When a router
receives a packet, it pops labels as needed, and if it is an intermediate point of a \LS{} takes the appropriate action.
For example, when $D$ receives a packet on tunnel $l3$
it pops the outer label $l3$, and based on the inner label $q1$,
looks up the entry for $B$, and forwards to $B$ along tunnel $l4$. 

A key question is to decide how to split the traffic at each hop -- e.g., for traffic from $A$ to $B$, what fraction is sent on each of tunnels $l5$, and \LS{} $q2$. We define \textit{local proportional routing} as a scheme where the traffic associated with each node pair $(i,j)$ is split across all tunnels and \LS{}s from $i$ to $j$ in proportion to the reservations associated with these tunnels and \LS{}s. This is a generalization of \FFC{} which uses a locally proportional scheme but in a context where there are only tunnels. Then, the following holds:
%
%\begin{figure}[t]
%	\centering
%	    \includegraphics[ trim={3.5cm 8.5cm 13.3cm 3cm}, clip, width=0.45\textwidth]{figures/implementation_example_local.pdf}
%        \label{fig:implementation_example_local}
%    \caption{$A$'s routing tables for distributed routing scheme.
%    \sgr{Please see revised text. The figure is repetitive but maybe ok. Should we also show D's table? Also, show packets and labels as they go across the network?}
%    }
%        \label{fig:implementation_example_local}
%\end{figure}
%
%
\begin{proposition}
\label{prop:topological_assumption} 
The \LS{} models can be realized by local proportional routing
when the topological sort property is met.
\end{proposition}

%\input{prop7_proof_old}
\input{prop7_proof_new}

Thus, once the model is solved and the reservations are determined, traffic is forwarded by each router in proportion to the reservations. When a tunnel fails, or a \LS{} is inactive (for \SysLS{}, \LS{}s are always active, while for \SysCLS{}
the \LS{}s are active under a given set of conditions), the weights are re-scaled in proportion to the reservations on the live tunnels and active \LS{}s. 
Our evaluations focus on \LS{}s $q$ between $i$ and $j$ which are only active when the link $i-j$ fails. Then, this failure is locally detected by $i$ which then activates $q$ and follows the standard proportional scheme. We discuss ways to get topologically sorted sequences in \S\ref{sec:evaluation}.

%After the weights are installed, under each scenario, a router will update its table to disable the failed tunnels and inactive \LS{}s, and renormalize the remaining weights. As described in \S\ref{sec:vs_model} and \S\ref{sec:ls_with_hint}, an unconditional  \LS{} is always active and a conditional \LS{} will be inactive when the attached hint is not satisfied under current scenario.  \sgr{Special case where link fails..}


%We find that some simple heuristics to choose \LS{}s can ensure topologically sorted assumption. For example, we can use the shortest path(segment) as the unconditional logical sequence for each source-destination pair. Then the assumption is satisfied under any failure scenario. \cj{do we need argument/proof here?} We will show in \S\ref{sec:evaluation} that using this set of \LS{}s can greatly improve the performance. Another way to ensure the assumption is to start with a more sophisticated set of \LS{}s which may violate the assumption. Then we can prune the set so that the remaining set makes $P$ able to be topologically sorted.

%\subsection{Topologically sorted \LS{}}
%\label{sec:topsortls}

%Based on proposition \ref{prop:linear_system}, we know that all the reservations in the same node pair $(i,j)$ are used by the same fraction. From the view of distributing traffic, this means that the traffic going through $(i,j)$ is assigned to \LS{}s and physical tunnels in proportion to the values of their reservation, which is similar to FFC's routing scheme except that we also have \LS{}s. So we can use the similar distributed scheme by including the information of \LS{}s. 

%\begin{figure}[t]
%	\centering
% 	    \includegraphics[ trim={3.5cm 8.5cm 13.3cm 3cm}, clip, width=0.45\textwidth]{figures/implementation_example_local.pdf}
%        \label{fig:implementation_example_local}
%    \caption{$A$'s routing tables for distributed routing scheme.}
%    \label{fig:implementation_example_local}
%\end{figure}

%Figure~\ref{fig:implementation_example_local} shows how we can use proportional allocation to route the same topology in Figure~\ref{fig:implementation_example}. The figure shows router $A$'s tables in it. When $A$ needs to send traffic to $B$, it will first looks up its table for $B$, which tells it the available paths are a physical tunnel $l_5$ and a \LS{} $q_2$ and it should split traffic equally. If it chooses $l_5$, the traffic will go through tunnel $l_5$ as in FFC. If it chooses $q_2$, the traffic will be sent though segments $AD$ and $DB$. The next hop table will tell that the next hop for $q_2$ is $D$. So it will need to again check the table for $D$, which shows the two ways to go to $D$ are $l_3$ and $q_1$ with equal weights. It will then split traffic between these two choices which will either send the traffic directly through $l_3$ to $D$, or use $q_1$ and eventually send through $l_1$ to $C$, the next hop of $q_1$. When the traffic on $q_2$ goes to $D$, $D$ will know from its table that the next hop of $q_2$ is $B$, and look up paths to route to $B$. Just like in FFC's implementation, the installed weights of tunnels and \LS{}s are normalized values of reservations($a_l$ and $b_q$). If we use this scheme to route, how the traffic is sent through physical tunnels will be exactly the same as that achieved from linear systems.

%Note that, just as we model the \LS{}, we allow a logical sequence to use other logical sequences to route for its segments. So in this example, $q_1$ can be used to route $AD$ segment in $q_2$. As a result, even though we never provide a physical tunnel or a \LS{} as $A-C-D-B$, such routing can be achieved in our implementation. After the weights are installed, under each scenario, a router will update its table to disable the failed tunnels and inactive \LS{}s, and renormalize the remaining weights. As described in \S\ref{sec:vs_model} and \S\ref{sec:ls_with_hint}, an unconditional  \LS{} is always active and a conditional \LS{} will be inactive when the attached hint is not satisfied under current scenario.

%The above routing scheme of proportional distribution will not add much extra complexity in implementation other than what is already in FFC's implementation. However, for some choices of \LS{}s, it may cause recursion in routing. Suppose we have an additional \LS{} $q_3$ from $D$ to $B$ which goes through segments $DA$ and $AB$. Routing from $A$ to $B$ may use $q_2$ and the traffic will go through segment $DB$. When $D$ tries to route to $B$, it may choose $q_3$. However, if $q_3$ is chosen, it will again need to go through segment $AB$ and cause recursion.

%Whether this routing scheme will run into recursion clearly depends on how we choose \LS{}s. We find that under some assumptions of \LS{}s, we can ensure this distributed routing scheme works. We define a relation '$>$' on $\langle P, P \rangle$. If when routing from $i$ to $j$, it's possible to use a \LS{} which passes through segment $i'j'$, we say that $(i,j) > (i', j')$. More formally, if $L(i,j)\cap Q(i'j)' \ne \emptyset$, we define that $(i,j) > (i',j')$. Now we claim that if \LS{}s are chosen in a way that $P$ can be topologically sorted on the '$>$' relation at each failure scenario, then the routing scheme described above can be deployed without recursion.

%\begin{proposition}\label{prop:topological_assumption} Under the topologically sorted assumption, a local proportionally
%distributed routing scheme similar to FFC scheme works for \LS{} model. 
%\end{proposition}
%{\bf Proof.} 
%We will formally define the proportional rules and show that by doing so, we will get the solution to the linear system $M \times \vec{U} = \vec{D}$. We define $U_{a_l}$ as the amount of traffic on tunnel $l$ and $U_{b_q}$ as the amount of traffic on physical sequence $q$. Then we assign the value to $U_{a_l}$ and $U_{b_q}$ in the topological order of node pairs. We assign the value as below using the proportional rules:

%\begin{align}
%\begin{split}
%& u_{ij} = \frac{\vec{D}(i,j) + \sum_{(m,n) \in P,q\in Q(i,j)\cap L_x(m,n)}U_{b_q}}{\sum_{l\in T_x(i,j)}a_l + \sum_{q\in L_x(i,j)}b_q} \quad \forall (i,j) \in P \\
%& U_{a_{l'}} = u_{ij}a_{l'} \quad \forall (i,j) \in P, l' \in T_x(i,j)\\
%& U_{b_{q'}} = u_{ij}b_{q'} \quad \forall (i,j) \in P, q' \in L_x(i,j)\\
%\end{split}
%\end{align}

%Since the values are assigned in the topological order, so $\forall q \in Q(i,j)$, $U_{b_q}$ is assigned before $(i,j)$. So this strategy is well-defined.

%Now for any $(i,j) \in P$, if we sum $U_{a_{l}}$ and $U_{b_{q}}$ over all $l \in T_x(i,j)$ and $q \in L_x(i,j)$, we get

%\begin{align}
%\begin{split}
%& \vec{D}(i,j) + \sum_{(m,n) \in P,q\in Q(i,j)\cap L_x(m,n)}u_{mn}b_{q} \\
%& = \sum_{l\in T_x(i,j)}u_{ij}a_{l} + \sum_{q\in L_x(i,j)}u_{ij}b_{q} \\
%\end{split}
%\end{align}

%Then the above equation becomes exactly the linear system we need to solve where  $\vec{U^*}$ is the solution if $\vec{U^*}(i,j) = u_{ij}$ for all $(i,j) \in P$.
%$\square$

%We find that some simple heuristics to choose \LS{}s can ensure topologically sorted assumption. For example, we can use the shortest path(segment) as the unconditional logical sequence for each source-destination pair. Then the assumption is satisfied under any failure scenario. \cj{do we need argument/proof here?} We will show in \S\ref{sec:evaluation} that using this set of \LS{}s can greatly improve the performance. Another way to ensure the assumption is to start with a more sophisticated set of \LS{}s which may violate the assumption. Then we can prune the set so that the remaining set makes $P$ able to be topologically sorted.





==> design_bak.tex <==
\section{design}

Suppose we have a set of applications $A$ where each application in $A$ has SLO requirement to sustain desirable performance with probability of $\beta$. Based on the definition of \AppOptLoss{}, we know that all applications will have no more than loss of \AppOptLoss{} with probability of $\beta$. For example, if $\beta$ is $0.99$ and we have a routing which provides \AppOptLoss{} of $10\%$, then this routing ensures that any application will see no more than $10\%$ loss with probability of $0.99$. So we want to design routing for each failure scenario so that \AppOptLoss{} is minimized. Next, we illustrate our key notations and how we model this problem.

%-For each flow, flow-loss is weighted sum of loss across scenarios, with the weight corresponding to how likely that scenario is bad.
%Pick the best routing.
% $min x$
%-Take a weighted sum of the flow-loss across all the flows with the weight being how likely that flow is a bottleneck flow. Pick the best weights for which scenario is bad for each flow.
%  $max_w min_x$
%-Optimize this across all the possible weights for the bottleneck flow.
%  $max_\lambda max_w min_x$
  
%Write applications with multiple flows, start with single target. Then present multiple targets as a separate thing.

\begin{table}[t]
  %\small
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|| c || p{6cm}||} 
    \hline
      notation  & meaning\\
    \hline\hline
$Q$ & Set of all scenarios \\
$A$ & Set of applications \\
$P$ & Set of source-destination pairs\\
$R(i)$ & Set of tunnels for pair $i$\\
$E$ & Set of edges\\
$d_{ai}$ & Traffic demand of pair $i$ in application $a$\\
$\beta$ & Target availability\\
$p_q$ & probability of scenario q\\
$y_{lq}$ & 1 if tunnel $l$ is alive in scenario $q$, 0 otherwise\\
$x_{lq}$ & allocated bandwidth on tunnel $l$ in scenario $q$(routing variable)\\
$t_{qa}$ & loss of application $a$ in scenario $q$\\
$w_{qa}$ & the contribution of scenario $q$ to worst scenarios for application $a$ \\
$\theta$ & worst cvar across applications\\
$\theta_a$ & cvar of application $a$\\
$\alpha_a$ & dual variable, can be interpreted as 'threshold' loss between good and bad scenarios\\
$s_{qa}$ & dual variable, can be interpreted as the loss exceeding the threshold\\
$Z_{ak}$ & Bound on sum of probabilities of scenarios in group $k$ that are excluded for application $a$(later it gets scaled by $\gamma_a$) \\
$z_{aq}$ & $w_{qa}$ scales by $\gamma_a$(the weight of application $a$)\\
$\gamma_a$ & importance of application $a$, can be interpreted as the probability of application $a$ being the bottleneck. \\
    \hline    
    \end{tabular}
    }
    \caption{Notation}
    \label{tab:notations}
    \vspace{-0.3in}
\end{table}

\subsection{Notation and preliminaries}


Consider a network topology, represented as a graph $G= \langle V, E 
\rangle $. Each link $e \in E$ is associated with a link capacity $c_e$. 
$P$ to represent the set of source-destination pairs. Each pair $i$ can use a set of tunnels $R(i)$ to route the traffic. Each application $a \in A$ requires bandwidth to send traffic for multiple source-destination pairs. We are given the traffic demand $d_{ai}$ for pair $i$ in application $a$. With each application requiring bandwidth for multiple source-destination pairs, we now define the loss of an application $a$ in a failure scenario $q$ $loss(a,q)$ as its max loss across pairs. For example, if an application $a$ has $10\%$ loss in a scenario, then at least one of its source-destination pairs $i$ only has $0.9d_{ai}$ bandwidth, and no pair will see a loss more than $10\%$.

$Q$ represents the set of failure scenarios. For each scenario $q \in Q$, $p_q$ represents the probability of $q$. And $y_{lq}$ represents whether a tunnel $l$ is alive in scenario $q$. We use $x_{lq}$ to denote the bandwidth assigned to tunnel $l$ in scenario $q$, i.e., our designed routing. 

 \cj{need to talk about SLO, var, cvar} Below, we present a formulation to design routing for a target availability $\beta$

\begin{align}
\mbox{($W$)} \ 
& \min_{x,t} \max_{w,a\in A} \quad \sum_{q \in Q} t_{qa}w_{qa} \nonumber \\ 
\mbox{s.t.} 
& \sum_{q\in Q} w_{qa} \le 1-\beta \quad \forall a \in A\\
& 0 \le w_{qa} \le p_q \quad \forall a \in A, q \in Q \\
& \sum_{l \in R(i)} x_{lq}y_{lq} \ge \sum_{a \in A}(1 - t_{qa})d_{ai} \quad \forall i \in P, q \in Q \label{eq:demand} \\
& \sum_{e \in l} x_{lq} \le c_e \quad \forall e \in E,q \in Q  \label{eq:capacity}
\end{align}

Here, $x_{lq}$ represents the bandwidth we allocate to tunnel $l$ in scenario $q$. $t_{qa}$ represents the loss of application $a$ in scenario $q$, which means that for each flow $i$, at least $(1-t_{qa})d_{ai}$ traffic should be transferred in scenario $q$. The value of $w_{qa}$ represents a selection of scenarios for application $a$. The inner max over $w$ is to find scenarios with most loss for each application and compute the average loss, and max over $a \in A$ is to find the application with worst average loss. Since every application has its own $w$  variable, the selection of worst $1-\beta$ scenarios can be different for each application, unlike Teavar. In other words, different applications can achieve their target availability through different set of scenarios, which allows more flexibility in coordinating traffic across applications to achieve SLO. For example, in the scenario shown in Fig.\ref{fig:flow_example_1}, the above model allows the network to ignore application 2(AD flow) so that application 1(AC flow) gets all the bandwidth, while Teavar forces the two applications to share bandwidth and raises the loss.

\subsection{decomposition}
optimization problem can be converted into an LP. Note that we need to enumerate scenarios and design routing for each scenario. As a result, it will not scale well for large topologies and large set of scenarios. We will show how to decompose this problem into iteratively solving several sub-problems. 


We make two modifications to the above formulation. 1. We split scenarios into $|G|$ groups. $Z_{ik}$ can be seen as the budget of scenarios we assign to group $k$ for flow $i$. For each flow in each group $k$, we are looking for the worst $Z_{ik}$ scenarios. 2. we rewrite the most inner max(max flow cvar) as a convex combination of flow cvar. We can prove that the optimal objective will not change(example? lemma?).

\begin{align}
& \min_{x} \max_{w,Z,\gamma}  \quad \sum_{a \in A} \gamma_a(\sum_{k,q\in Q_k} t_{qa}w_{qa}) \nonumber \\ 
\mbox{s.t.} 
& \sum_{a \in A}\gamma_{A} = 1\\
& \gamma_{a} \ge 0 \quad \forall a \in A\\
& \sum_{k\in G} Z_{ak} \le 1-\beta \quad \forall a \in A\\
& \sum_{q\in Q_k} w_{qa} \le Z_{ak} \quad \forall a \in A, k \in G\\
& 0 \le w_{qa} \le p_q \quad \forall a \in A, q \in Q \\
& \eqref{eq:demand}, \eqref{eq:capacity} \nonumber
\end{align}

To eliminate the non-linear terms in the objective, let $z_{iq} = \gamma_i w_{qi}$, and we also scale $Z_{ik}$ by $\gamma_i$. The formulation can be rewritten as

\begin{align}
& \mbox{($W''$)} \max_{Z,\gamma} \min_{x} \max_{z}  \quad \sum_{a \in A} (\sum_{k,q\in Q_k} t_{qa}z_{aq}) \nonumber \\ 
\mbox{s.t.} 
& \sum_{a \in A}\gamma_{a} = 1\\
& \gamma_{a} \ge 0 \quad \forall a \in A\\
& \sum_{k\in G} Z_{ak} \le (1-\beta)\gamma_a \quad \forall a \in A\\
& \sum_{q\in Q_k} z_{aq} \le Z_{ak} \quad \forall a \in A, k \in G\\
& 0 \le z_{aq} \le p_q \gamma_a \quad \forall a \in A, q \in Q \\
& \eqref{eq:demand}, \eqref{eq:capacity} \nonumber
\end{align}

Note that we interchange min and max in the problem.

Take the dual of inner max of (W''), we can get

\begin{align}
& \mbox{($H$)}  \max_{Z,\gamma} \min_{x,\alpha, s}  \quad \sum_{a \in A} \sum_{k \in G} (\alpha_a Z_{ak} + \sum_{q\in Q_k} p_q s_{qa} \gamma_a) \nonumber \\ 
\mbox{s.t.} 
& \sum_{a \in A}\gamma_{a} = 1\\
& \sum_{k\in G} Z_{ak} \le (1-\beta)\gamma_a \quad \forall a \in A\\
& \alpha_{a} + s_{qa} \ge t_{qa}   \quad \forall a \in A, q \in Q \\
& s_{qa} \ge 0   \quad \forall a \in A, q \in Q \\
& \eqref{eq:demand}, \eqref{eq:capacity} \nonumber
\end{align}

We use Bender's decomposition to iteratively solve the problem. The inner min problem can be decomposed into $|G|$ sub-problems, one per group.

\begin{align}
& \mbox{($Sub_k$)}  \min_{x,\alpha, s}  \quad \sum_{a \in A} (\alpha_{ak} Z_{ak} + \sum_{q\in Q_k} p_q s_{qak} \gamma_a) \nonumber \\ 
\mbox{s.t.} \quad & \alpha_{ak} + s_{qak} \ge t_{qa}   \quad \forall a \in A, q \in Q_k \\
& s_{qak} \ge 0   \quad \forall a \in A, q \in Q_k \\
&   \sum_{l \in R(i)} x_{lq}y_{lq} \ge \sum_{a \in A}(1 - t_{qa})d_{ai} \quad \forall i \in P, q \in Q_k  \\
& \sum_{e \in l} x_{lq} \le c_e \quad \forall e \in E,q \in Q_k 
\end{align}

The outer max problem will be the master problem of Bender's which aggregates the sub-problems:

\begin{align}
\begin{split}
& \mbox{($Master$)} \max_{Z,\gamma}   \quad \sum_{k \in G} f_k  \\ 
\mbox{s.t.} \quad
& \sum_{a \in A}\gamma_{a} = 1\\
& \sum_{k\in G} Z_{ak} \le (1-\beta)\gamma_a \quad \forall a \in A\\
& f_k \le \sum_{a \in A} (\alpha^*_{ak} Z_{ak} + \sum_{q\in Q_k} p_q s^*_{qak} \gamma_a) \quad \forall k \in G\\
\end{split}
\end{align}

%%Notes
\textbf{Why partition not feasible in one formulation but feasible in another.}

Original formulation: 
-For each flow, each partition, compute the loss.
-Compute sum across partitions for each flow.
-Then compute max across flows.

New formulation:
 -Each partition, compute weighted sum of loss across flows in that partition
 -Sum over partitions.
 
\textbf{Heuristics: Finding reasonable initial parameters($\gamma$ and $Z$) for Bender's.} General idea: $\gamma_i$ can be interpreted as the probability that flow $i$ is the bottleneck flow, and $Z_{ik}$ is the budgets on scenarios that can be excluded for group $k$ and flow $i$, scaled by $\gamma_i$. We solve SMORE for each scenario, and achieve the information of how each flow performs in each scenario($\lambda_i$), and then aggregate this information in the worst $1-\beta$ scenarios.

-Model that ensures the worst-case loss across all flows is as small is possible for each scenario. Lets refer to this as ScenarioOptimalLoss model (right now, call this SMORE, but revisit later).

-What we want is to optimize the loss of flows across scenarios, rather than be optimal for any given scenario. That is we are willing to tolerate some extra loss for some flows in some scenarios than the above strategy, if those flows can already meet their overall requirements through other scenarios.

The reason why this is a heuristic. SMORE is assuming the worst scenarios are the same for all flows. But, really the worst scenarios could be different across the flows.


1. Solve SMORE for each scenario, and get $\lambda_i$(dual variable of $\theta \ge t_i$). This can be interpreted as the probability of $i$ being the bottleneck flow in this scenario.

2. Let $Q'$ be the set of scenarios with worst $(1-\beta) \%$ loss obtained by SMORE(not specific to any flow). So $\sum_{q \in Q'} p_q = 1-\beta$.

3. $\gamma_i = \frac{\sum_{q \in Q'} \lambda_i p_q}{1-\beta} $. Note that $\sum_{q \in Q'} p_q = 1-\beta$. So as a heuristic, we initialize $\gamma_i$ to be the weighted average of $\lambda_i$ in $Q'$, and captures the probability that flow $i$ is the bottleneck in $Q'$, i.e., the worst scenarios in SMORE. 

4. $Z_{ik} = \sum_{q\in Q_k}\lambda_i p_q $. As a heuristic, we set $Z_{ik}$ to be the probability that flow $i$ is the bottleneck for scenarios in partition $Q_k$.

(If we do this for the whole set:

1. Solve SMORE for each scenario, and get $\lambda_i$.

2. $\gamma_i = \sum_{q \in Q} \lambda_i p_q$. Note that $\sum_{q \in Q} p_q = 1$. So $\gamma_i$ is the weighted average of $\lambda_i$ over the whole set.

3. $Z_{ik} = \frac{1}{1-\beta}\sum_{q\in Q_k}\lambda_i p_q $
)





==> ffcMonotonocity.tex <==
\section{\System{} overview}
\label{sec:system}
\System{}'s primary goal is to bridge the gap between existing congestion-free routing mechanisms, and intrinsic network capability. \System{} tackles the issues raised in \S\ref{sec:motivation} by better modeling, and adopting more flexible response strategies.

Unfortunately, not all routing strategies are amenable to formal guarantees on worst-case performance under 
failures. For instance, when the network responds with an optimal multi-commodity flow (the most flexible response), the problem of determining the worst-case performance under failures is intractable~\cite{lancet:sigmetrics20}. Thus, a central challenge that \System{} tackles is one of carefully crafting response strategies that are (i) amenable to formal worst-case guarantees; and yet (ii) perform closer to the network's intrinsic capability. \sgr{Deployability?}

\System{} achieves the above by (i) developing tractable optimization formulations that are inspired by practical response mechanisms in networking and conservatively estimate network capability; and (ii) providing explicit response mechanisms that achieve the estimated capability. Moreover, \System{} allows the network architect to incrementally dial-in additional flexibility in response as desired.

%\System{} achieves the above by (i) developing tractable optimization formulations that provide conservative estimates of the network's intrinsic capability. These tractable formulations are loosely inspired by variants of practical mechanisms using in networking; and (ii) designing response mechanisms with provable guarantees by considering the mechanisms implicit in these tractable models. 
%
%In practice, it may be desirable to restrict response mechanisms Thus, rather than present a single "point" mechanism, as part of \System{}, we have developed a family of mechanisms, that represent different trade-offs between efficiency and the complexity of deployment. In particular,
%

\textbf{Roadmap.} We introduce notation (\S\ref{sec:notation}), and present \FFCimp{} (\S\ref{sec:monotonicity}), 
which uses \FFC{}'s response mechanism
but better models network structure. We show that \FFCimp{} out-performs \FFC{}, and achieves better performance with more tunnels. Despite these benefits, we show that \FFCimp{} (like \FFC{}) can perform arbitrarily worse than optimal. We introduce a more flexible approach based on  the logical sequence abstraction, and formally show the performance benefits over \FFCimp{} (\S\ref{sec:vs_model}). We present further generalizations in \S\ref{sec:ls_with_hint}, and show how to practically realize the schemes (\S\ref{sec:practical}). 

%$\bullet$ On the other hand, we also present a mechanism that performs close to optimal, while being significantly more deployable than optimal.



\subsection{Notation and preliminaries}
\label{sec:notation}

%FFC~\cite{ffc_sigcomm14} is a path-based routing scheme which can compute the bandwidth allocated to each tunnel in order to optimize the performance on the network under $k_e$ simultaneous link failures and $k_v$ simultaneous node failures. Note that in this work, we only focus on link failures, but we can easily add node failures following the same idea. 

Consider a network topology, represented as a graph $G= \langle V, E 
\rangle $. Each link $e \in E$ is associated with a link capacity $c_e$. For each node pair $(s,t)$ on the graph, we are given a traffic demand $d_{st}$, and a set of tunnels $T(s,t)$ to route the traffic. Each tunnel $l$ consists of a set of links $\tau_l \subseteq E$. Below, we present a formulation for bandwidth allocation with tunnels,
%
\begin{align}
\mbox{($P1$)} \ 
& \max_{z,a} \quad \Theta(z) \nonumber \\
\mbox{s.t.} \quad & 
\sum_{l \in T(s,t)} a_{l}(1 - y_{l}) \ge z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y \label{eq:tunnel_serve_demand} \\ 
& a_{l} \ge 0 \quad \forall s,t \in V, l \in T(s,t) \label{eq:al_1} \\ 
& \sum_{l;\forall s,t \in V, l \in T(s,t)} a_{l} \delta(e \in \tau_{l}) \le c_e \quad \forall e \in E \label{eq:al_2}
\end{align}
%
Here, $\delta(e \in \tau_{l})=1$ if $e \in \tau_{l}$ and 0 otherwise. The formulation determines $a_l$ and $z_{st}$, where $a_l$ represents the amount of reservation on tunnel $l$, and variable $z_{st}$ represents the fraction of traffic from $s$ to $t$ that can be satisfied. $Y$ stands for the set of tunnel failure scenarios of interest, and $y_l$ indicates whether tunnel $l$ fails or not in a failure scenario (we later discuss how $Y$ is modeled).
$\Theta(z)$ is the metric function we want to optimize. For tractability, we assume $\Theta(z)$ is a concave function, and note that this model covers common metrics such as overall throughput and maximum link utilization. For example, $\Theta(z) = \sum_{s,t} \min\{1,z_{st}\}d_{st}$ models overall throughput. Alternately, when $\Theta(z) = \min\limits_{s,t}\{z_{st}\}$, and the optimal value is $\Theta^*$, the model guarantees that $\Theta^*$ fraction of each flow can be sent in every failure scenario. The inverse of this $\Theta^*$ is the utilization of the most congested link, also known as the Maximum Link Utilization (MLU). \sgr{Cite references to indicate these metrics are used in traffic engineering.} Thus, $\Theta(z) = \min\limits_{s,t}\{z_{st}\}$ minimizes the MLU.




%We define monotonicity as a property on models. We say a model is monotonic on tunnels, if when more tunnels are added, the performance doesn't get worse. From the example above, FFC is clearly not monotonic on tunnels.

%Without the last tunnel carrying $0.5$ unit of traffic, the first 3 tunnels can only carry 2.5 when there is no failure. For the same reason, under single link failure, only 1.5 traffic can be guaranteed. And only 0.5 traffic can be guaranteed under 2 link failures.

%Table~\ref{tab:ffc_example} shows the throughput guarantee given by FFC under two tunnel options and the optimal result. FFC can not reach optimal under failures in either of these two tunnel options. The first tunnel option is always 0.5 less than the optimal because it doesn't have the fourth tunnel to use. But providing the fourth tunnel to FFC even impairs the throughput guarantee under failures, which means FFC model is not monotonic on tunnels.

%\subsection{Better failure model}\label{sec:analysisffc}

\subsection{Modeling network structure}
\label{sec:monotonicity}
We now discuss how to model the set of failure scenarios $Y$. If at most $p_{st}$ tunnels between $s$ and $t$ share a common link, \FFC{} assumes that upto $fp_{st}$ tunnels can fail under 
$f$ link failures, and plans for \textit{all possible combinations} of $fp_{st}$ tunnel failures. As discussed in \S\ref{sec:motivation}, this is conservative -- e.g., for the network shown in Fig.~\ref{fig:ffc_example}, FFC considers the simultaneous failure of $l1$ and $l2$ even though this is impossible under single link failure. To address this, \System{} more accurately models $Y$ by better relating link and tunnel failures. Let $x_e$ indicate if link $e$ fails. Then, \System{} models $Y$ as:
%
\begin{align}
\begin{split}
& \sum_{e \in E} x_e \le f \\
& x_e - y_l \le 0 \quad \forall l, e \in \tau_{l} \\
& y_l - \sum_{e \in \tau_{l}} x_e \le 0 \quad \forall l  \\
& 0 \le x_{e} \le 1 \quad \forall e\in E\\
& 0 \le y_{l} \le 1 \quad \forall l\\
\end{split}\label{eq:tunnel_model}
\end{align}
%
The first constraint bounds the maximum number of simultaneous link failures. The second ensures that the failure of an underlying link will cause the tunnel to fail. The third ensures that a tunnel only fails when at least one underlying link fails. \sgr{Discuss binary/relaxation?}
%If $x$ are binary, these constraints model the exact relationship between link failures and tunnel failures, and $Y$ is the set of tunnel failure scenarios under $f$ link failures. 
%\sgr{But x is not binary.. is some explanation needed?} 
We denote (P1) with $Y$ modeled by \eqref{eq:tunnel_model} as \FFCimp{}. Next, we prove that (i) \FFCimp{} performs at least as well as \FFC{}; and (ii) unlike \FFC{}, the performance of \FFCimp{} does not degrade as more tunnels are added.

\begin{proposition}\label{prop:ffcim_beats_ffc}
The feasible region of FFC is contained in the feasible region of \FFCimp{}, so \FFCimp{} performs at least as well as FFC for any metric. 
\end{proposition}
\textbf{Proof.} \FFC{} models $Y$ as
%
\begin{align}
\begin{split}
& \sum_{l \in T(s,t)}y_{l} \le fp_{st} \quad \forall s,t \in V\\
& 0 \le y_{l} \le 1 \quad \forall l\\
\end{split} \label{eq:ffc_failure}
\end{align}
% 
Let $Y_0$ be the set of tunnel failure scenarios considered by FFC (constrained by \eqref{eq:ffc_failure}) and let $Y_1$ be the set of tunnel failure scenarios considered 
by \FFCimp{} (constrained by \eqref{eq:tunnel_model}). We show that $Y_1 \in Y_0$. 
For any $s,t\in V$, we sum the third constraint in \eqref{eq:tunnel_model} over all $l \in T(s,t)$ to get $\sum_{l\in T(s,t)} (y_l - \sum_{e \in \tau_{l}} x_e ) \le 0$.
%
%\begin{align}
%\begin{split}
%& \quad \sum_{l\in T_{st}}\Big(y_l - \sum_{e \in \tau_{l}^E} x_e \Big) \le 0 \quad \forall s,t \in V
%\end{split}
%\end{align}
%
Then,
\begin{align}
\begin{split}
& \quad \sum_{l\in T(s,t)}y_l \le \sum_{l\in T(s,t)}\sum_{e \in \tau_{l}} x_e  = \sum_{l\in T(s,t)}\sum_{e \in E} x_e\delta(e \in \tau_{l}) \\
& = \sum_{e \in E} x_e\sum_{l\in T(s,t)}\delta(e \in \tau_{l})  \le fp_{st},
\end{split} 
\nonumber
\end{align}
%
%\begin{align}
%\begin{split}
%& \quad \sum_{l\in T_{st}}y_l \\
%& \le \sum_{l\in T_{st}}\sum_{e \in \tau_{l}^E} x_e  = \sum_{l\in T_{st}}\sum_{e \in E} x_e\delta(e \in \tau_{l}^E) \\
%& = \sum_{e \in E} x_e\sum_{l\in T_{st}}\delta(e \in \tau_{l}^E)  \le k_ep_{st},
%\end{split} 
%\end{align}
%
which shows that any scenario in $Y_1$ also satisfies \eqref{eq:ffc_failure}. Since FFC imposes (1) for each $y\in Y_0$ while \FFCimp{} imposes (1) for each $y\in Y_1$, \FFCimp{} is less constrained than FFC. \sgr{Discuss: does FFC relax integrality of y?}
$\square$

The above proof does not depend on the objective function in the optimization problem, which means that the proposition holds for any metric. We next show that unlike \FFC{}, \FFCimp{}'s performance does not degrade
with more tunnels.

\begin{proposition}\label{prop:ffcim_beats_ffc}
As we provide more tunnels, \FFCimp{}'s performance can not decrease.
\end{proposition}
\textbf{Proof.} 
Let $\{T_0(s,t) \mid \forall s,t \in V\}$ and $\{T_1(s,t) \mid \forall s,t \in V\}$ be two sets of tunnels, and $T_0(s,t) \subseteq T_1(s,t)$ for all $s,t \in V$. Then, we show that the optimal value for (P1) with $T = T_1$ will not be worse than the optimal solution to (P1) with $T = T_0$.
\sgr{Added we show that. Resolve if it looks ok}
Let $(a^*, z^*)$ be the optimal solution to (P1) with $T = T_0$. We construct $(a', z')$ in the following way,
%
\begin{align}
\begin{split}
& a'_l = a^*_l \quad \forall s,t \in V, l \in T_0(s,t)\\
& a'_l = 0 \quad \forall s,t \in V, l \in T_1(s,t) - T_0(s,t)\\
& z'_{st} = z^*_{st} \quad \forall s,t \in V
\end{split}
\end{align}
%
Let $Y_0$ denote \eqref{eq:tunnel_model} with $T=T_0$ and $Y_1$ denote \eqref{eq:tunnel_model} with $T=T_1$. It is easy to see that projection of $Y_1$ onto the space of variables $\{x_e\}_{e\in E}$ and $\{y_l\}_{l \in T_0}$ is contained in $Y_0$, since all the constraints in $Y_0$ are present in $Y_1$. Now for each $y \in Y_1$,
%
\begin{align}
\begin{split}
&  \sum_{l \in T_1(s,t)} a'_{l}(1 - y_{l}) = \sum_{l \in T_0(s,t)} a^*_{l}(1 - y_{l}) \le z^*_{st}d_{st} = z_{st}d_{st}, 
\end{split}
\nonumber
\end{align}
%
where the first equality is because $a'_l = 0$ for $l \notin T_0(s,t)$, the first inequality is because $(a^*,z^*)$ is feasible for $T=T_0$ and the projection of $Y_1$ is contained in $Y_0$ and the last equality is by construction. 
%
Since $z$ is not altered, the objective value remains the same. $\square$


%Based on the above propositions, using failure model in \eqref{eq:tunnel_model} can solve non-monotonicity issue of the conservative way to model failures. And using \eqref{eq:tunnel_model} will be at least as good as the original failure model. 

We later show in \S\ref{sec:evaluation} that
\FFCimp{} 
%using \eqref{eq:tunnel_model} instead of \eqref{eq:ffc_failure} 
performs much better than \FFC{} for real networks.
Like with \FFC{}, the failure set $Y$ may involve too many scenarios to enumerate. Instead, the model \FFCimp{} (and all other models presented in this paper) can be solved using dualization to ensure the number of constraints is polynomial in the size of the network, a technique that has been widely used in prior networking papers~\cite{r3:sigcomm10,ffc_sigcomm14,nsdiValidation17}.
More details are presented in the Appendix.






==> fig_bak.tex <==

\begin{figure*}[t]

\begin{minipage}[t]{0.45\textwidth}
	    \includegraphics[ trim={7.8cm 10.5cm 7.7cm 6.1cm}, clip, width=\textwidth]{figures/problem_scenario.pdf}
        \label{fig:flow_example_1}

    \vspace{-0.25in}
    \caption{How traffic is routed by SMORE and Teavar when link AD fails.}
        \label{fig:flow_example_1}
\end{minipage}\hspace{0.1in}
%
\begin{minipage}[t]{0.45\textwidth}
\includegraphics[trim={6.5cm 9cm 4.3cm 5cm}, clip, width=\textwidth]{figures/smore_table.pdf}
        \label{fig:smore_table}
\vspace{-0.25in}
    \caption{Loss incurred with SMORE and Teavar.}
        \label{fig:smore_table}
\end{minipage}\hspace{0.1in}
%
\vspace{-0.15in}
\end{figure*}



\begin{figure}[t]
	\centering
        \includegraphics[ trim={7.8cm 10.5cm 7.7cm 6.1cm}, clip, width=0.48\textwidth]{figures/problem_scenario.pdf}
        \label{fig:flow_example_1}

    \vspace{-0.25in}
    \caption{How traffic is routed by SMORE and Teavar when link AD fails.}
        \label{fig:flow_example_1}
        \vspace{-0.1in}
\end{figure}

\begin{figure}[t]
	\centering
 \includegraphics[trim={6.5cm 9cm 4.3cm 5cm}, clip, width=0.48\textwidth]{figures/smore_table.pdf}
        \label{fig:smore_table}
\vspace{-0.25in}
    \caption{Loss incurred with SMORE and Teavar.}
        \label{fig:smore_table}
        \vspace{-0.1in}
\end{figure}





\begin{figure}[t]
	\centering
    	   \includegraphics[trim={7cm 9cm 7.6cm 6.5cm}, clip, width=0.48\textwidth]{figures/flow_example.pdf}
        \label{fig:flow_example}

    \vspace{-0.25in}
    \caption{Illustrating \System{}’s potential
    %\sgr{Replace Application 1 by Flow f1, Application 2 by Flow f2. Also, can you show f1 and f2 in the picture how they should be routed to meet the requirements?}
    }
        \label{fig:flow_example}
        \vspace{-0.1in}
\end{figure}

\begin{figure}[t]
	\centering
    	  \includegraphics[trim={6.7cm 9cm 4.3cm 5cm}, clip, width=0.48\textwidth]{figures/optimal_table.pdf}
        \label{fig:optimal_table}
\vspace{-0.4in}
    \caption{The loss achieved for routing scheme in Fig.~\ref{fig:flow_example}. The ovals show that each flow can
   be sent with 99\%ile loss of 0. The last column's values are not relevant.
    }
        \label{fig:optimal_table}
        \vspace{-0.2in}
\end{figure}



==> overview_bak.tex <==
\section{\System{} overview}



\subsection{Notation and preliminaries}
\label{sec:notation}

%FFC~\cite{ffc_sigcomm14} is a path-based routing scheme which can compute the bandwidth allocated to each tunnel in order to optimize the performance on the network under $k_e$ simultaneous link failures and $k_v$ simultaneous node failures. Note that in this work, we only focus on link failures, but we can easily add node failures following the same idea. 

Consider a network toplogy, represented as a graph $G= \langle V, E 
\rangle $. Each link $e \in E$ is associated with a link capacity $C_e$. For each node pair $(s,t)$ on the graph, we are given a traffic demand $d_{st}$, and a set of tunnels $T_{st}$ to route the traffic. Each tunnel $l$ consists of a set of links $\tau_l^{E} \subseteq E$. Below, we present a formulation corresponding to classic tunnel-based fowarding used in \FFC{}. 

\begin{align}
\begin{split}
& \max_{z,a} \quad \Theta(z) \\
\mbox{s.t.} \quad & 
\sum_{l \in T_{st}} a_{l}(1 - y_{l}) \ge z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y\\
& a_{l} \ge 0 \quad \forall s,t \in V, l \in T(s,t)\\
& \sum_{l;\forall s,t \in V, l \in T_{st}} a_{l} \delta(e \in \tau_{l}^E) \le c_e \quad \forall e \in E\\
\end{split}\label{eq:tp_model}
\end{align}


The formulation seeks to determine $a_l$ and $z_{st}$ where $a_l$ represents the amount of reservation on tunnel $l$, and variable $z_{st}$ represents the fraction of traffic from $s$ to $t$ that can be satisfied. $Y$ stands for the set of tunnel failure scenarios of interest, and $y_l$ indicates whether $l$ fails or not in a failure scenario (we later discuss how $Y$ is modeled).
$\Theta(z)$ is the metric function we want to optimize. Note that $\Theta(z)$ can be any concave function, and this model covers common metrics such as overall throughput and link utilization. For example, $\Theta(z) = \sum_{s,t} min(1,z_{st})d_{st}$ maximizes overall throughput. Alternately, we could use $\Theta(z) = min(z_{st})$. Doing so maximizes the factor $z$ such that all flows can be guaranteed an allocation $z$ times their demand under all failure scenarios in $Y$. Further, with this model, the inverse of the objective
minimizes the maximum link utilization (or the utilization of the most congested link).

 


%We define monotonicity as a property on models. We say a model is monotonic on tunnels, if when more tunnels are added, the performance doesn't get worse. From the example above, FFC is clearly not monotonic on tunnels.

%Without the last tunnel carrying $0.5$ unit of traffic, the first 3 tunnels can only carry 2.5 when there is no failure. For the same reason, under single link failure, only 1.5 traffic can be guaranteed. And only 0.5 traffic can be guaranteed under 2 link failures.

%Table~\ref{tab:ffc_example} shows the throughput guarantee given by FFC under two tunnel options and the optimal result. FFC can not reach optimal under failures in either of these two tunnel options. The first tunnel option is always 0.5 less than the optimal because it doesn't have the fourth tunnel to use. But providing the fourth tunnel to FFC even impairs the throughput guarantee under failures, which means FFC model is not monotonic on tunnels.

%\subsection{Better failure model}\label{sec:analysisffc}

\subsection{Accurately modeling failures}
\label{sec:monotonicity}
A key question with Eq (\ref{eq:tp_model}) above is how to model the set of failure scenarios $Y$. \FFC{}'s approach is to determine the parameter $p_{st}$ such that at most $p_{st}$ tunnels between $s$ and $t$ share a common link.
Then, \FFC{} assumes that upto $k_ep_{st}$ tunnels could fail under 
$k_e$ link failures, and plans for \textit{all possible combinations}
of $k_ep_{st}$ tunnel failures. 



As discussed in \S\ref{}, this is unduly conservative. For example, in
Fig.\ref{}, under single link failures, only tunnels $T3$ and $T4$ fail
together, and other two tunnel failure combinations need not be considered.
To address this, \System{} more accurately models the failure set $Y$ 
to only capture those combinations of tunnel failures that actually
need be considered. Let $x_e$ indicates if link $e$ fails.
Then, \System{} models $Y$ as 

\begin{align}
\begin{split}
& \sum_{e \in E} x_e \le k_e \\
& x_e - y_l \le 0 \quad \forall l, e \in \tau_{l}^E \\
& y_l - \sum_{e \in \tau_{l}^E} x_e \le 0 \quad \forall l  \\
& 0 \le x_{e} \le 1 \quad \forall e\in E\\
& 0 \le y_{l} \le 1 \quad \forall l\\
\end{split}\label{eq:tunnel_model}
\end{align}

The first constraint bounds the maximum number of simultaneous link failures. The second ensures that any failed underlying link of a tunnel will cause the tunnel to fail. The third ensures that a tunnel only fails when at least one underlying link fails. This set of constraints depict the exact connection between link failures and tunnel failures, and $Y$ will be exactly the set of tunnel failure scenarios under $k_e$ link failures. 
%Thus it will eliminate the gap caused by conservative estimation of tunnel failures in \FFC{}. 
We denote the optimization problem \eqref{eq:tp_model} with $Y$ modeled by \eqref{eq:tunnel_model} as \FFCimp{}. Next, we prove that (i) \FFCimp{} 
performs at least as well as \FFC{}; and (ii) unlike \FFC{}, the performance 
of \FFCimp{} does not degrade as more tunnels are added.

\begin{proposition}\label{prop:ffcim_beats_ffc}
The feasible region of FFC is contained in the feasible region of \FFCimp{}, so \FFCimp{} performs at least as well as FFC for any metric.
\end{proposition}
\textbf{Proof.} \FFC{} models $Y$ as

\begin{align}
\begin{split}
& \sum_{l \in T_{s,t}}y_{l} \le k_ep_{st} \quad \forall s,t \in V\\
& 0 \le y_{l} \le 1 \quad \forall l\\
\end{split} \label{eq:ffc_failure}
\end{align}
 
Let $Y_0$ be the set of all tunnel failure scenarios considered by FFC(constrained by \eqref{eq:ffc_failure})
and let $Y_1$ be the set of all tunnel failure scenarios considered by \FFCimp{}(constrained by \eqref{eq:tunnel_model}). For any $s,t\in V$ we sum the last constraint in \eqref{eq:tunnel_model} over all $l \in T_{st}$ to get

\begin{align}
\begin{split}
& \quad \sum_{l\in T_{st}}(y_l - \sum_{e \in \tau_{l}^E} x_e ) \le 0 \quad \forall s,t \in V
\end{split}
\end{align}

Thus

\begin{align}
\begin{split}
& \quad \sum_{l\in T_{st}}y_l \\
& \le \sum_{l\in T_{st})}\sum_{e \in \tau_{l}^E} x_e  = \sum_{l\in T_{st}}\sum_{e \in E} x_e\delta(e \in \tau_{l}^E) \\
& = \sum_{e \in E} x_e\sum_{l\in T_{st}}\delta(e \in \tau_{l}^E)  \le k_ep_{st}
\end{split} 
\end{align}

which shows that any scenario in $Y_1$ also satisfies \eqref{eq:ffc_failure}. So $Y_1 \subseteq Y_0$. Then \FFCimp{}'s constraints are contained in \FFC{}'s constraints. And \FFC{}'s feasible region is contained in \FFCimp{}'s.
$\square$

Note that the above proof doesn't depend on the objective function in the optimization problem, which means that the proposition holds for any metric. Then, we will also show that \eqref{eq:tp_model} with $Y$ modeled by \eqref{eq:tunnel_model} is monotonic on tunnels. 

\begin{proposition}\label{prop:ffcim_beats_ffc}
As we provide more tunnels, \FFCimp{}'s performance will not decrease.
\end{proposition}
\textbf{Proof.} 
\cj{proof needs some modification}
Let $\{T_0(s,t)|\forall s,t \in V\}$ and $\{T_1(s,t)|\forall s,t \in V\}$ be two sets of tunnels, and $T_0(s,t) \subseteq T_1(s,t)$ for all $s,t \in V$. Then the optimal solution to \eqref{eq:tp_model} with $T = T_1$ will not be worse than the optimal solution to \eqref{eq:tp_model} with $T = T_0$.
Let $(a^*, b^*)$ be the optimal solution to \eqref{eq:tp_model} with $T = T_0$. We construct $(a', b')$ in the following way,

\begin{align}
\begin{split}
& a'_l = a^*_l \quad \forall s,t \in V, l \in T_0(s,t)\\
& a'_l = 0 \quad \forall s,t \in V, l \in T_1(s,t) - T_0(s,t)\\
& b'_{st} = b^*_{st} \quad \forall s,t \in V\\
\end{split}
\end{align}

It is easy to see that $(a', b')$ is a solution to \eqref{eq:tp_model} with $T = T_1$. Since $b'=b^*$ and the objective is the sum over all $b$, the objective of $(a', b')$ is the same as the objective of $(a*, b*)$. So the optimal solution with $T = T_1$ is at least as good as the optimal solution with $T = T_0$.
$\square$

%Based on the above propositions, using failure model in \eqref{eq:tunnel_model} can solve non-monotonicity issue of the conservative way to model failures. And using \eqref{eq:tunnel_model} will be at least as good as the original failure model. 

We later show in \S\ref{sec:evaluation} that \eqref{eq:tunnel_model} provides significantly better performance than \FFC{} in real networks.
Like with \FFC{}, the failure set $Y$ may involve too many scenarios to enumerate. The model \FFCimp{} (and all other models presented in this paper) may be solved using dualization to ensure the number of constraints is polynomial in the size of the network, a technique that has been widely used in prior networking papers~\cite{r3:sigcomm10,ffc_sigcomm14,nsdiValidation17}.
More details are presented in the Appendix. \sgr{Chuan: please remember to add this.}






==> prop7_proof_new.tex <==
{\bf Proof.} For a particular failure scenario $x$, let $T_x(s,t)$ denote the set of live tunnels from $s$ to $t$, $L_x(s,t)$ denote the set of active \LS{}s from $s$ to $t$ and $Q_x(s,t)$ denote the active \LS{}s which go through segment $(s,t)$. We show by induction along the topological sort order that locally proportional routing services the demand. Our induction hypothesis is that the pair $(i,j)$ needs to route $\Tilde{D_{ij}}$ where,
%
\begin{align}
\begin{split}
\Tilde{D_{ij}} = \vec{D}(i,j) + \sum_{(m,n) \in P, q\in Q_x(i,j)\cap L_x(m,n)}u_{mn}b_q, 
\label{eq:hypothesis_equality}
\end{split}
\end{align}
if every router distribute $\Tilde{D_{ij}}$ among the tunnels ($l \in T_x(i,j)$) and \LS{}s ($q \in L_x(i,j)$) in the proportion of their reservations, i.e., there is a constant $u_{ij}$ such that traffic along $l$ is $u_{ij}a_l$ and that along \LS{} q is $u_{ij}b_q$ where 
%
\begin{align}
\begin{split}
u_{ij} = \frac{\Tilde{D_{ij}}}{\sum_{l\in T_x(i,j)}a_l + \sum_{q\in L_x(i,j)}b_q}. \nonumber
\end{split}
\end{align}
%
For the base case, observe that for the topologically largest pair $p_1=(i_1,j_1)$, the demand received is $\vec{D}(i_1,j_1)$. And the hypothesis is trivially true because $Q(i_1,j_1)=\emptyset$. For the induction step, we assume that the hypothesis is true for pairs $p_1,p_2,...,p_n$ in topological sort order and show it holds for $p_{n+1} = (i,j)$. Observe that for any $q \in Q_x(i,j) \cap L_x(m,n)$, the traffic sent to $b_q$ is, by the induction hypothesis, $u_{mn}b_q$ because $Q_x(i,j) \cap L_x(m,n) = \emptyset$ implies $(m,n) > (i,j)$. Then,
%
\eqref{eq:hypothesis_equality} holds for $(i,j)$, and
it follows easily that if $(i,j)$ routes $u_{ij}b_q$ along each $q \in L_x(i,j)$ and $u_{ij}a_l$ along each $l \in T_x(i,j)$ that $\sum_{l \in T_x(i,j)} u_{ij}a_l + \sum_{q \in L_x(i,j)} u_{ij}b_q = \Tilde{D_{ij}}$.
%
Since it follows easily from above that 
%
\begin{align}
\begin{split}
u_{ij}(\sum_{l \in T_x(i,j)} a_l + \sum_{q \in L_x(i,j)} b_q) = \\
\vec{D}(i,j) + \sum_{(m,n) \in P, q\in Q_x(i,j)\cap L_x(m,n)}u_{mn}b_q, \nonumber
\end{split}
\end{align}
%
it follows that $(u_{ij})_{(i,j)\in P}$ solves $M \times \vec{U} = \vec{D}$. Therefore, by proposition \ref{prop:linear_system}, $0 \le u_{ij} \le 1$. This implies that the routing is feasible since none of the reservations are exceeded. $\square$

==> prop7_proof_old.tex <==
{\bf Proof.} 
For a particular failure scenario $x$, let $T_x(s,t)$ denote the set of alive tunnels from $s$ to $t$, $L_x(s,t)$ denote the set of active \LS{}s from $s$ to $t$. Recall (\S\ref{sec:vs_model}) that $Q(s,t)$ denotes the set of \LS{}s which go through segment $(s,t)$.  We formally define the proportional rules and show that the result is a solution to the linear system $M \times \vec{U} = \vec{D}$. Let $U_{a_l}$ 
and $U_{b_q}$ respectively denote the traffic on tunnel $l$ and \LS{} $q$. Then, we assign values to $U_{a_l}$ and $U_{b_q}$ using the proportional rules below:
%
\begin{align}
\begin{split}
& u_{ij} = \frac{\vec{D}(i,j) + \sum_{(m,n) \in P,q\in Q(i,j)\cap L_x(m,n)}U_{b_q}}{\sum_{l\in T_x(i,j)}a_l + \sum_{q\in L_x(i,j)}b_q} \quad \forall (i,j) \in P \\
& U_{a_{l}} = u_{ij}a_{l} \quad \forall (i,j) \in P, l \in T_x(i,j)\\
& U_{b_{q}} = u_{ij}b_{q} \quad \forall (i,j) \in P, q \in L_x(i,j)
\end{split}
\nonumber
\end{align}
%
We assign values in the topological order of node pairs. Hence, $\forall q \in Q(i,j)$, $U_{b_q}$ is assigned before $u_{ij}$, and the strategy is well-defined.
%
Now for any $(i,j) \in P$, we have
%
\begin{align}
\begin{split}
& \sum_{l\in T_x(i,j)}u_{ij}a_{l} + \sum_{q\in L_x(i,j)}u_{ij}b_{q} \\
& = 
\vec{D}(i,j) + \sum_{(m,n) \in P,q\in Q(i,j)\cap L_x(m,n)}u_{mn}b_{q}
\end{split}
\nonumber
\end{align}

Then $\vec{U}$ where $\forall (i,j) \in P: \vec{U}(i,j) = u_{ij}$ is the solution to the linear system $M \times \vec{U}= \vec{D}$.
$\square$

==> topological_sort_proof.tex <==

\subsection{proof}

\cj{a few notations may be a bit confusing and conflicting the previous sections because sec 4 and 5 are not written yet.}

We define a graph $G=\langle V, E \rangle$ where $V$ is the set of nodes and $E$ is the set of edges. Each edge $e \in E$ is associated with an edge capacity $C_e$. For each node pair $(s,t)$ on the graph, we are given a traffic demand $d_{st}$, and a set of physical tunnels $T_a(s,t)$ and a set of logical sequences $T_b(s,t)$ we can use to route traffic. If a physical tunnel $l$ consists of an edge $e$, then $e \in L_a(l)$. If a logical sequence $q$ uses node pair $(i,j)$, then $q \in L_b(i,j)$.

We also define a relation 'cover' on $\langle V^2, V^2 \rangle$. If $T_b(i,j) \cap L_b(i',j') \neq \emptyset$, we define that $(i,j)$ covers $(i',j')$.

We solve the virtual network model to get a set of variables $b(q)$ on all logical sequences and $a(l)$ on all physical tunnels which satisfies the following constraints:

\begin{align}
\begin{split}
& d_{i,j} + \sum_{q \in L_b(i,j)} b_q \le \sum_{l \in T_a(i,j)} a_l + \sum_{q \in T_b(i,j)} b_q \quad \forall i, j \in V \\
& \sum_{l \in L_a(i,j)} a_l \le c_{i,j} \quad \forall \langle i, j \rangle \in E \\
\end{split}
\end{align}

We define $sd(q) = (i,j)$ if $q \in T_b(i,j)$, then a routing can be found by solving the following linear system 

\begin{align}
\begin{split}
& d_{i,j} + \sum_{q\in L_b(i,j)}Z(sd(q))b(q) = Z(i,j)(\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)) \\
\end{split}\label{eq:linear_system}
\end{align}

To write as matrix, we are solving $Z$ for $AZ=D$, where $A_{(i,j),(i,j)} = \sum_{l \in T_a(i,j)} a_l + \sum_{q \in T_b(i,j)} b_q$, $A_{(i,j),(i',j')} = -\sum_{q \in L_b(i,j) \cap T_b(i',j')} b_q$, $D_{(i,j)} = d_{i,j}$.

\begin{proposition}\label{prop:linear_system}
A valid routing always exists from the virtual network model. More formally, there always exists a solution to \eqref{eq:linear_system} in $[0,1]^{|V^2|}$. 
\end{proposition}

{\bf Proof.} 
We use fixed-point theorem to prove this. Let $f(Z)$ be a function with mapping from $[0,1]^{|V^2|}$ to $\mathbb{R}^{|V^2|}$. And we define $f(Z)$ as

\begin{align}
\begin{split}
& f(Z)_{i,j} = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z(sd(q))b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \\
\end{split}
\end{align}

It is easy to see that $Z_0$ is a solution to \eqref{eq:linear_system} if $f(Z_0) = Z_0$. With $Z \in [0,1]^{|V^2|}$, we have 

\begin{align}
\begin{split}
& f(Z)_{i,j} \ge \frac{d_{i,j}}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \ge 0 \\
\end{split}
\end{align}

and 

\begin{align}
\begin{split}
& f(Z)_{i,j} \le \frac{d_{i,j} + \sum_{q\in L_b(i,j)}b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \le 1 \\
\end{split}
\end{align}

Since $f$ is a continuous function mapping from from $[0,1]^{|V^2|}$ to $[0,1]^{|V^2|}$, and $[0,1]^{|V^2|}$ is a compact convex set, based on fixed-point theorem, we know that there is at least one point $Z_0$ so that $f(Z_0) = Z_0$.
$\square$

Now assume all node pairs can be topologically sorted based on the cover relation, we claim that we can route the demand in this strategy: Distribute traffic for node pairs in the topological order. And for each node pair $(i,j)$, distribute the demand and the flow from $L_b(i,j)$ to the physical tunnels $T_a(i,j)$ and $T_b(i,j)$ proportionally based on $a(l)$ and $b(q)$. 

\begin{proposition}\label{prop:topological_sort}
If all node pairs can be topologically sorted based on the cover relation, then assigning traffic proportionally will be a valid routing.
\end{proposition}

{\bf Proof.} 
We will formally define the proportional rules and show that by doing so, we will get a valid solution to \eqref{eq:linear_system}. We define $Z_a(l)$ as the amount of traffic on tunnel $l$ and $Z_b(q)$ as the amount of traffic on physical sequence $q$. Then we assign the value to $Z_a(l)$ and $Z_b(q)$ in the topological order of node pairs. We assign the value as below using the proportional rules:

\begin{align}
\begin{split}
& Z_a(l') = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)}a(l') \quad \forall l' \in T_a(i,j)\\
& Z_b(q') = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)}b(q') \quad \forall q' \in T_b(i,j)\\
\end{split}
\end{align}

Since the values are assigned in the topological order, so $\forall q \in L_b(i,j)$, $Z_b(q)$ is assigned before $(i,j)$. So this strategy is well-defined.

Now for any $(i,j)$, if we sum $Z_a(l)$ and $Z_b(q)$ over all $l \in T_a(i,j)$ and $q \in T_b(i,j)$, we get

\begin{align}
\begin{split}
& d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q) = \sum_{l\in T_a(i,j)}Z_a(l) + \sum_{q\in T_b(i,j)}Z_b(q) \\
\end{split}
\end{align}

Let $Z(i,j) = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)}$. Then the above equation becomes exactly the linear system we need to solve. So $Z(i,j)$ is a solution.

We then show by induction that $Z(i,j) \in [0,1]$ for all node pairs $(i,j)$. Suppose $(i_0,j_0)$ is the first node pair in the topological order. Then we have $L_b(i_0,j_0) = \emptyset$. So $Z(i_0,j_0) = \frac{d_{i_0,j_0}}{\sum_{l\in T_a(i_0,j_0)}a(l) + \sum_{q\in T_b(i_0,j_0)}b(q)} \in [0,1]$. 
Now for node pair $(i,j)$ which is not the first in the topological order, suppose for every node pair $(i',j')$ previous to $(i,j)$  in the order, we have $Z(i',j') \in [0,1]$. Then

\begin{align}
\begin{split}
& Z(i,j) = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \\
& \quad \quad \quad  =\frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z(sd(q))b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \\
& \quad \quad \quad \le \frac{d_{i,j} + \sum_{q\in L_b(i,j)}b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \le 1
\end{split}
\end{align}

Similarly, we can show that $Z(i,j) \ge 0$. So by induction, $Z(i,j) \in [0,1]$ for all node pairs $(i,j)$. 
$\square$

Some simple heuristics can be used to find a set of \LS{}s which satisfy the topologically sorted assumption. In fact, using shortest path(segments) as the unconditional \LS{}s for all pairs can ensure the assumption. \cj{do we need to prove this?}In \S\ref{sec:evaluation}, we will show that this set of \LS{}s can significantly improve the performance. Another way to satisfy the assumption is to find a more sophisticated set of \LS{}s first, which may violate the assumption. Then we can prune the set so that the remaining set works. 

==> vnGeneralized.tex <==
\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={9cm 9.3cm 7cm 10cm}, clip, width=0.48\textwidth]{figures/vnhintexample.pdf}
        \label{fig:vn_hint_example}
\vspace{-0.25in}
    \caption{Illustrating conditional logical sequences}
        \label{fig:vn_hint_example}
\vspace{-0.05in}
\end{figure}


\begin{table}[t]
  \small
    \centering
    \begin{tabular}{||c c c c c c||} 
    \hline
     Optimal & FFC & \FFCimp{} & \SysLS{} & \SysCLS{} & R3 \\
    \hline\hline
    1 & 0 & 2/3 & 4/5 & 1 & 0 \\ 
    \hline
    \end{tabular}
    \caption{Throughput of different schemes for the topology in Fig~\ref{fig:vn_hint_example} under 2 simultaneous link failures.}
    %with 6 tunnels. We provide a \LS{} $S4T$ for \SysLS{} and \SysCLS{}. In \SysLS{}-1 and \SysCLS{}, we provide tunnels $S-4$ and 3 tunnels from $4$ to $T$. In addition to this, we provide $S-1-4$, $S-2-4$ and $S-3-4$ for \SysLS{}-2. \cj{Is this too long?..}}
    \label{tab:toy_result}
    \vspace{-0.2in}
\end{table}

\subsection{Conditional Logical Sequences}
\label{sec:ls_with_hint}
As described in \S\ref{sec:vs_model}, each segment in a \LS{} must guarantee the reservation 
associated with the \LS{} over the entire set of failures. We next consider a generalization, that we call conditional \LS{}s which only guarantee the reservation over a subset of failure scenarios. A conditional \LS{} $q$ is associated with a condition $h_q$, and a reservation $b_q$. The reservation $b_q$ must be guaranteed over each segment of $q$ for all scenarios where the condition $h_q$ is met. An example condition is a given set of links being alive or dead. 

\textbf{Illustrating benefits of conditional \LS{}s}. We illustrate by considering Fig.~\ref{fig:vn_hint_example}. Table~\ref{tab:toy_result} shows the traffic guaranteed by different schemes for traffic from source $s$ to destination $t$ under single and two link failures. The table shows both \FFC{} and \FFCimp{} (both schemes use all 6 tunnels from $s$ to $t$) are sub-optimal (for the same reasons as (\S\ref{sec:monotonicity}, \S\ref{sec:vs_model})).

Consider now that a \LS{} $(s,4,t)$ is added with logical segments $s4$ (with the tunnel $s-4$), and $4t$ (with multiple tunnels from $4$ to $t$ including $4-1-5-t$, $4-2-6-t$, and $4-3-7-t$). Further, the \LS{} is associated with a condition that the reservation is only needed when the link $s-4$ is alive. 
Table~\ref{tab:toy_result} shows the optimal is achieved with this conditional \LS{} (\SysCLS{}). Consider two link failure case. When $s-4$ is dead, at most one of the tunnels $s-1-5-t$, $s-2-6-t$, $s-3-7-t$ are dead and the remaining can carry 1 unit of flow. When $s-4$ is alive, at most 2 of these tunnels are dead. Therefore, they can cary 0.5 units of flow. Finally, \LS{} $(s,4,t)$ can carry 0.5 units of flow since $s4$ is alive and at most 2 of the tunnels $4-1-5-t$ , $4-2-6-t$ and $4-3-7-t$ are dead.
%To explain why, consider the single link failure case. When $s4$ is dead, all the tunnels $s15t$, $s26t$ and $s37t$ are alive (since we are designing for single link failures), and can together carry $3/2$ units of traffic. When $s4$ is alive, at most one of these tunnels can fail with single link failures, and the remaining tunnels can carry a traffic of $0.5$. Further, the LS{} $s4t$ may carry a reservation of $0.5$ which can be guaranteed in all scenarios where $s4$ is alive, and at most one other link fails. 

Note that when the same \LS{} is added but without the attached condition, the objective is 
not optimal. This is because, the logical segment $s4$ cannot guarantee any reservation over single link failures when only the tunnel $s-4$ is used. It is possible to add more tunnels between $s$ and $4$ (e.g., $s-1-4$, $s-2-4$, $s-3-4$), which allows the \LS{} $(s,4,t)$ to be more resilient to failures (\SysLS{}). However, this is at the cost of reservations on the tunnels from $s$ to $t$, and consequently the objective is increased but still does not achieve the optimal.
\sgr{May need to readd text to say which scheme is what, but my concern is about naming scheme.}






%\begin{figure}[t]
%	\centering
%        \includegraphics[trim={0 4cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/r3_example_1.png}
%        \label{fig:r3_example_1}
%    \caption{Limitation of R3~\cite{r3:sigcomm10}.
%    \sgr{Please replace this fig as discussed.}
%        }
%    \label{fig:r3_example}
%\end{figure}




%\begin{figure}[t]
%	\centering
%	    \includegraphics[ trim={0.5cm 0.5cm 0.8cm 0.5cm}, clip, width=0.48\textwidth]{figures/vnhint_example_result.pdf}
%        \label{fig:vn_hint_example_result}
%    \caption{Throughput guarantee achieved by \VS{} model with and without using \LS{} comparing to the optimal.
%    \sgr{Include R3, and hints. Also, internally do various other configurations to decide how to show.}
%    }
%     \label{fig:vn_hint_example_result}
%\end{figure}




%\textbf{Old possibly useful text: Conditional reservation}
%Unfortunately, isolating shared part in tunnels is not enough to handle the example in Figure~\ref{fig:ffc_example}. The main reason is that under 2 simultaneous link failures, we can't guarantee capacity from $S$ to $7$ with only one path to send the traffic. Thus, we are not able to utilize the new tunneling. However, the capacity from $S$ to $7$ is not always needed. As in the policy mentioned in  \S\ref{sec:analysisffc}, if $S-7$ dies, the 3 tunnels without involving $7$ can handle the traffic. We only need the other 3 tunnels when $S-7$ is alive. In other words, we only need to send traffic from $S$ to $7$ when $S-7$ is alive. To achieve this, we are introducing conditional reservation which provides richer flexibility in routing. A conditional reservation means we require a certain amount of capacity only when the associated condition is satisfied. And we also only use it when the same condition is true. In the example in Figure~\ref{fig:ffc_example}, we can make conditional reservation from $S$ to $7$ with the condition being that $S-7$ is alive. Similarly, we can make a conditional reservation from $7$ to $T$ with the same condition. With the associated condition being satisfied, enough capacity can be reserved so that the throughput on the network will met the optimal.

\textbf{Modeling conditional \LS{}s.} 
We next discuss how conditional \LS{}s are modeled. Under any given failure scenario, let $h_q$ indicate whether \LS{} $q$ is active or not. Like before, let $y_l$ indicate whether tunnel $l$ fails or not. Let $(y,h)$ denote all $y_l$ and $h_q$ variables, and let $YH$ denote all possible combinations of $(y,h)$ under all scenarios involving the simultaneous failure of $f$ links. To incorporate these conditions, we replace constraint \eqref{eq:capconstraint} in (P2) with the constraint below,
and refer to the resulting model as \textbf{\SysCLS{}}.
%
\begin{align}
& \sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + \sum_{q \in L(s,t)} b_{q} h_{q} \nonumber \\
& \ge \sum_{q' \in Q(s,t)} b_{q'} h_{q'} + z_{st}d_{st} \quad \forall s,t \in V, \forall (y,h) \in YH \nonumber
%\label{eq:vs_model}
\end{align}
%
In \S\ref{sec:evaluation}, we show that \LS{}s activated under a simple condition (a single link being dead) is sufficient to get good performance. To handle this, we model $YH$ by adding constraints $h_q = x_{e_q}$ 
for each \LS{} $q$ to \eqref{eq:tunnel_model}, where $e_q$ is the link whose failure activates \LS{} $q$. In the Appendix, we model a more general condition, where all links in a set $\eta_q$ are alive and all links in a 
set $\xi_q$ are dead, which helps generalize \System{} to richer failures (e.g., node failures) (\S\ref{sec:generalizations}).

%\System{} is general, and \LS{}s may be associated with a wide range of conditions on \LS{}s that indicate under which scenarios the reservation is activated. In practice, we find a simple condition  is sufficient to get good performance (\S\ref{sec:evaluation}). Here, we can model $YH$ by adding $h_q = x_{e_q}$ to \eqref{eq:tunnel_model} for each sequence $q$, where $e_q$ is the link associated with the condition condition. \cj{Please check this para where I only talk about the most simple condition 2020.2.6}

%As an example, if the condition for \LS{} $q$ is all links in $\eta_q$ are alive and all links in $\xi_q$ are dead, then we model $YH$ by adding the following constraints to \eqref{eq:tunnel_model}:
%
%$H(f)$ denotes the set of all possible hinting scenarios under $f$ simultaneous link failures. $h_q$ denotes whether the hint of $q$ is true in the hinting scenario $h$. Note that in the most general form, a hint essentially describes an arbitrary subset of all link failure scenarios. But we find that in many cases, a simple hint such as a link being alive or a link being dead is sufficient to greatly improve the performance as in the example above. This also makes the model more tractable. Suppose the hint for \LS{} $q$ is all links in $\eta_q$ are alive and all links in $\xi_q$ are dead, then similar to \eqref{eq:tunnel_model}, we can model $H(f)$ as
%
%\begin{align}
%\begin{split}
%& (h_q - 1) + x_e \le 0 \quad \forall q, e \in \eta_{q} \\
%& h_q - x_e \le 0 \quad \forall q, e \in \xi_{q} \\
%& (1 - h_q) - \sum_{e \in \eta_{q}} x_e - \sum_{e \in \xi_{q}} (1 - x_e) \le 0 \quad \forall q  \\
%& 0 \le h_{q} \le 1 \quad \forall q\\
%\end{split}\label{eq:hint_model}
%\end{align}
%

%greatly improve the performance. \cj{simple hint in appendix}\sgr{Revisit the above text. Do we need the model here? Should we present a simpler case for single link failure if we do and say it can be more general?}

\subsection{\System{} generalizations}
\label{sec:generalizations}
In this section, we discuss generalizations of \System{}, and its 
relationship with R3~\cite{r3:sigcomm10}, another congestion-free mechanism. 

\textbf{Heuristics for selecting \LS{}s.}
We present a heuristic for selecting \LS{}s that works well empirically (\S\ref{sec:evaluation}). Our approach involves considering a more 
general model based on flows and decomposing the results of that model into \LS{}s. 

We begin by introducing \textit{logical flows}, which are a generalization
of \LS{}s in that traffic is no longer constrained to visiting a sequence of hops. A logical flow $w$ from $s$ to $t$ is captured by the flow balance constraints below:
%
\begin{equation}
\begin{split}
& b_{w} \ge 0 \quad \forall s,t \in V, \forall w \in W(s,t)\\
& \sum_{j} p_{w}(ij) - \sum_{j} p_{w}(ji) = 
\begin{cases}
b_{w}  \quad \forall s, t, i = s, w \in W(s,t) \\
0  \quad \forall s, t, i \ne s, i \ne t, w \in W(s,t) \\
-b_{w}  \quad \forall s, t, i = t, w \in W(s,t)
\end{cases} 
%\nonumber
\end{split}\label{eq:logflow}
\end{equation}
%
Here, $b_w$ is the reservation associated with the logical flow, and $p_{w}(ij)$ is
the amount of this reservation that must be supported on logical segment $ij$. 
%The constraints capture that the total reservation on all logical segments 
%outgoing from $s$ (and incoming to $t$) is $b_w$, while at all other nodes
%the reservation on segments coming into the node is the same as the reservation
%on segments going out of that node.
Each logical flow $w$ may itself be associated with a condition $h_w$, which indicates 
the reservation associated with $w$ is only guaranteed when $h_w$ is satisfied. 
%
Let $W(s,t)$ be the set of all logical flows for traffic from $s$ to $t$. Then,
relative to (P2), the logical flow model involves adding
\eqref{eq:logflow}, and changing \eqref{eq:capconstraint} to
%
\begin{align}
\begin{split}
& \sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + \sum_{w \in W(s,t)}b_{w}h_w  \\
& \ge \sum_{s',t' \in V,w' \in W(s',t')} p_{w'}(st)h_{w'} + z_{st}d_{st} \\
& \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \forall s,t \in V, \forall (y,h) \in YH\\
\end{split}
%\label{eq:vn_capacity_constraint}
\nonumber
\end{align}
%
The first term on the RHS captures the reservation that must be supported on 
$(s,t)$ for any logical flow $w'$ from $s'$ to $t'$.

To obtain \LS{}s, we decompose the flow into sequences~\cite{nsdiValidation17,semi_oblivious_nsdi18}. For each flow $w\in W(s,t)$, this approach generates a derived graph with the same
nodes as the original topology. 
%Or, more generally, a subset if some flexibility is undesirable. 
For each node pair $(i,j)$, if $p_w(ij) > 0$, we add an edge from $i$ to $j$ with the weight being $p_w(ij)$. Then, we search for the widest path from $s$ to $t$ on this graph, and use the sequence of hops in this widest path as a \LS{} with condition $h_w$. 

%\cj{decomposition algorithm. 2020.2.4}


%This more sophisticated routing can provide us a better understanding of the network's intrinsic capability and how to use the capacity to get a better performance, which can be used to generate \LS{}s to improve the performance of \VS{} model. For example, from $p_{st}(ij)$ we can find paths which take more capacity. Then these paths will be good candidates for \LS{}s to be used in \VS{} model.


\textbf{Relationship to link bypass.}
While we have focused on tunnel based mechanisms so far~\cite{ffc_sigcomm14}, we next discuss the relationship of our work to R3~\cite{r3:sigcomm10}, another congestion-free routing scheme.
Instead of tunnels, R3~\cite{r3:sigcomm10} focuses on a link bypass mechanism, where traffic on a link $e=\langle i,j \rangle$ is re-routed upon its failure, along a pre-computed flow from $i$ to $j$ and this flow does not use $e$. 

We first illustrate using Fig.~\ref{fig:vn_hint_example} that our models can out-perform R3. \sgr{2 failure, not single} As Table~\ref{tab:toy_result} shows, when R3 is applied to Fig.~\ref{fig:vn_hint_example}, no traffic can be carried from $s$ to $t$ if two link failures must be tolerated. To understand why, consider a scenario where links $1-5$, and $5-t$ fail. Since a link bypass for $1-5$ must start at $1$ and end at $5$, and a link bypass for $5-t$ must start at $5$ and end at $t$, no viable bypass paths exist for either link. Instead, an obvious feasible strategy is to route the traffic along the path $s-2-6-t$, an option that is not considered by R3 because $s$ is not an end point of either $1-5$ or $5-t$. 

We now state a more formal result:
%
\begin{proposition}
\label{prop:r3_bad}
A special case of \System{}'s logical flow model where 
conditions are restricted to the no failure or single link failure
scenarios, and links are tunnels, dominates R3.
\end{proposition}
%
\textbf{Proof.}
To see this, consider the logical flow model under the conditions above. More specifically, for each node pair $(s,t)$, we have a flow $w$ with the condition being no failure and we constrain the flow to exactly serve the demand, i.e., $b_w = z_{st} d_{st}$. For node pair $(i,j)$ which has an edge, we have a flow $w$ with the condition being the link $(i,j)$ being dead. This model is exactly the Generalized-R3 model presented in ~\cite{lancet:sigmetrics20} which has been shown to dominate R3. $\square$ 


%\textbf{Proof.}
%To see this, consider the logical flow model under the conditions above, but by adding $b_w = z_st d_st$ when $h_w=0$. This model is exactly the Generalized-R3 model presented in ~\cite{Lancet:Sigmetrics21} which has been shown to dominate R3.$\square$ \sgr{Chuan, please take a pass on the proposition.}



%The essential idea of R3 is to build a bypass for each link which will be used when that link fails. The way it models this, is to have a base routing to specify how the network routes the traffic under no failures, and to have a protection routing to reserve some bypass capacity for each link. When a link fails, the bypass for the failed link will be triggered to take over the traffic. If we look at R3 in our framework, links can be seen as tunnels in our model, base routing is reservation without hint and protection for link $i-j$ can be seen as reservation with hint of $i-j$ being dead. So R3 is a special case of our \VN{} framework where \VN{} with hint is adopted.


\textbf{Shared risk links groups (SRLGs) and node failures}
While we have focused on link failures, a few modifications allow for the treatment of shared risk link groups (SRLGs), and node failures. An SRLG captures that a group of links may fail together (e.g., owing to failure of an underlying optical element)~\cite{Sprint}. Each SRLG is modeled by a condition $h_q$ which indicates
all links in that SRLG fail. Observe that the first constraint in \eqref{eq:tunnel_model} is imposed on $x$ variables that capture link failures. Instead, the constraint can be imposed on conditions dependent on the $x$ variables. For example, a requirement that at most $f$ SRLGs fail is modeled by requiring that $\sum_{q \in Q} h_q \leq f$, where $Q$ is the set of SRLGs. Similarly, the failure of each node is modeled by a condition that all links incident on that router fail. 
%where $G$ is a set of SRLGs, and $x^{g}$ is the condition that the set of links in $G$ fail together. 
%Similarly, node failures may be modeled by having $G$ be the set of routers, and $x^{g}$ denoting that the links incident on the router fail together. 
%\LS{}s could be associated with these conditions that capture SRLG and node failure to allow re-routing
%traffic in these conditions.
%
%Any \LS{} that is used is associated with the condition that all nodes on that sequence must be alive. 
Our discussion and results in \S\ref{sec:monotonicity} holds for node failures as well - i.e., relative to \FFC{}, \FFCimp{} performs better, and \FFCimp{}'s performance does not degrade with tunnels.
Further, our models do not suffer from the weaknesses of link bypass mechanisms including R3~\cite{r3:sigcomm10}, that cannot deal with node failures (since no viable bypass paths for link $\langle i,j \rangle$ from $i$ to $j$ exist when node $j$ itself fails).


%Suppose $G$ is a set of shared risk links groups, and for $g\in G$, let $E_g$ represent the set of links in group $g$. To ensure congestion-free routing under at most $f$ group failures, 
%\System{} models the failure set $Y$ as shown below. 
%
%\begin{align}
%\begin{split}
%& \sum_{g \in G} x_g \le f \\
%& x_g - y_l \le 0 \quad \forall l, g: \tau_{l} \cap E_g \ne \emptyset\\
%& y_l - \sum_{g: \tau_{l} \cap E_g \ne \emptyset} x_g \le 0 \quad \forall l  \\
%& 0 \le x_{g} \le 1 \quad \forall g\in G, 0 \le y_{l} \le 1 \quad \forall l 
%\end{split} 
%\nonumber
%\end{align}
%
%The constraints capture that if a group $g$ fails ($x_g$ indicates if $g$ fails), then all tunnels using any link in $g$ fail. Further, a tunnel fails only if a group containing one of its links fail.


%The idea is that we draw connection between group failures and tunnel failures instead of between link failures and tunnel failures as in \eqref{eq:tunnel_model}. 
%As for \SysCLS{}, similarly, we can draw connection between group failures and hints.\cj{Do I need the hint failure model?} 

%Node failures may be modeled as an SRLG where each group is associated with all the links connected to a particular router. 





% However, for the same reason illustrated in \S\ref{sec:motivation}, it can be overly conservative and may provide worse performance guarantee if we provide more tunnels. Our schemes can also be used for node failures and SRLG, but with better performance guarantee. 

==> vnNoHintModel.tex <==
\subsection{Modeling more flexible response}
\label{sec:vs_model}
While \FFCimp{} is guaranteed to out-perform \FFC{}, we begin by presenting a theoretical result that shows the performance of \FFCimp{} can still be arbitrarily worse than optimal
because of the inflexibility of tunnel-based reservations.
We then discuss \System{}'s more flexible approach.

\begin{figure}[t]
	\centering
        
    	    \includegraphics[trim={6cm 14cm 8.3cm 8cm}, clip, width=0.48\textwidth]{figures/parallel_example_g.pdf}
        \label{fig:parallel_example_g}
\vspace{-0.25in}
    \caption{A topology with $m$ nodes generalized from the previous example.}
        \label{fig:parallel_example_g}
\end{figure}

\begin{proposition}
\label{prop:ffcimp_bad}
The throughput guaranteed by \FFCimp{} (and hence that guaranteed by \FFC{}) can be arbitrarily worse than the optimal even with exponentially many tunnels.\cj{without arbitrary metric function $\Theta$}
\end{proposition}
\textbf{Proof.} Consider the topology in Fig.~\ref{fig:parallel_example_g}
(the example in Fig.~\ref{fig:parallel_example} is a special case where $p = 3$, $n = 2$ and $m = 2$).
%
Under any failure involving $n-1$ links, the
network can carry $1 - \frac{n-1}{p}$ units of traffic if it responded optimally. This is because under any such failure, the network can carry (i) at least 1 unit of traffic between $s_i$ and $s_{i+1}, i > 0$; and (ii) at least $1 - \frac{n-1}{p}$ units of traffic between $s_0$ and $s_1$. Moreover, if $n-1$ of the links between between $s_0$ and $s_1$ fail simultaneously, the traffic is no more than $1 - \frac{n-1}{p}$.

Next, consider \FFCimp{}, and assume that all possible tunnels between $s$ and $t$ are used. There are $pn^{m-1}$ possible tunnels. We will show that \FFCimp{} can only guarantee traffic of $1/n$ units from $s_0$ to $s_m$ under $n-1$ simultaneous link failures. To see this, observe that the reservation across all tunnels between $s$ and $t$ is at most 1 (constrained by the capacity of all links between $s_0$ and $s_1$). Let $r_i$ denote the reservation on all tunnels that use the $i^{th}$ link between $s_1$ and $s_2$. Then, $\sum_{i=1}^{n} r_i \leq 1$, and there must exist at least one link $j$ between $s_1$ and $s_2$ such that $r_j \leq 1/n$. Consider a failure scenario where all links between $s_1$ and $s_2$ except $j$ fail. Under this scenario, \FFCimp{} can guarantee at most $1/n$ units of traffic from $s_0$ to $s_m$.

Note that $1 - \frac{n-1}{p} - \frac{1}{n} = \frac{(p-n)(n-1)}{pn}> 0$ whenever $p > n > 1$. Consider the case where $p = n^2$. Then, as $n$ gets larger, the amount of traffic carried in the optimal solution converges to 1, while  \FFCimp{} converges to 0. 
%It's reasonable to assume that $\Theta(z)$ is continuous at $0$ and $\Theta(0) = 0$, which is to say that sending small amounts of traffic should not cause a step jump in the performance, and that when no traffic is sent, the performance metric is zero. We can also assume that $\lim_{z \to 1} \Theta(z)$ is a constant number. Thus, the performance guaranteed by \FFCimp{} can be arbitrarily bad for any metric. 
$\square$



%\begin{itemize}
%\item parallel links example
% The number of tunnels can be exponential with long sequence

%\item Theoretical result:
%Theorem:  FFC-improved result can be arbitrarily bad

%\item Virtual network modeling
%A reservation builds a virtual network
%introduce logical sequence reservation b, b will need to be supported by its underlying hops
%\item ab no hinting model
%\end{itemize}


%\textbf{Old possibly useful text.}
%One of the reasons why FFC is not able to handle the example in Figure~\ref{fig:ffc_example} is that FFC can not distinguish the shared part among tunnels. Hence when it is doing reservation, it has to reserve the shared part multiple times in order to allocate to different tunnels, leading to a capacity bottleneck. For example, in Figure~\ref{fig:ffc_example}, link $S-7$ is a shared link for 3 tunnels. In FFC model, all these three tunnels are competing the capacity in $S-7$, resulting in a lower utilization. Our solution for this issue is to split the tunnels. More specifically in this example, we can split the 3 tunnels into a short tunnel from $S$ to $7$, and 3 tunnels from $7$ to $T$. In this way, tunnels will not compete for capacity in link $S-7$ anymore. If there is any traffic going from $S$ to $7$, $7$ will decide which tunnels to use instead of letting $S$ decide. Note that comparing to FFC, this is not simply changing the provided tunnels. It is fundamentally different from FFC because FFC only allows tunnels from the source of a flow to the destination of flow. Here, we will not pose any limitation on how the tunnels will be used.
%
%Though Proposition \ref{prop:ffcimp_bad} considers throughput, the same result can be proved for any metric $\Theta$ that satisfies some mild conditions as shown in the Appendix. 
As discussed in \S\ref{sec:motivation}, these issues with \FFC{} and \FFCimp{} stem from the fact that reservations are made over entire tunnels, are tightly coupled to a particular network path, and are pre-allocated independent of any specific failure scenario. When a link in the tunnel fails, the corresponding capacity is unavailable in other links along the tunnel. 

\textbf{Logical sequences.}
Instead, \System{} considers more flexible network response by introducing the notion of a \textit{logical sequence (\LS{})}. A \LS{} $q$ from $s$ to $t$ consists of a series of logical hops $s, v_1,...,v_m, t$. Consecutive logical hops in a \LS{} need not have a direct link between them, and in fact any pair of routers in the network could be consecutive logical hops. Traffic from $s$ to $t$ is required to traverse the logical hops $v_1, v_2, \dots ,v_m,t$, with 
significant flexibility in terms of how traffic is carried between two consecutive logical hops. In particular, traffic may be
carried over physical tunnels (like \FFC{}), or other \LS{}s. Each \LS{} $q$ is associated with a reservation $b_q$, which indicates that every segment of $q$ ($sv_1$, $v_1v_2$, \dots, $v_mt$) is guaranteed to carry $b_q$ traffic under all failure scenarios that \System{} is designed for. 
%\cj{picture needed?} \sgr{not sure, lets discuss later}.

We next illustrate the potential benefits of \LS{}s using  Fig.~\ref{fig:parallel_example_g}. Consider the \LS{} $q$ which traverses the logical hops $s_0,s_1,...,s_m$. Let each link be a tunnel. Traffic between consecutive logical hops is carried by the tunnels (links) connecting those hops. For example, traffic between $s_1$ and $s_2$ is carried on the $n$ tunnels (links) connecting the nodes. 
When any link fails, only the reservation in the relevant segment of $q$ is impacted
-- e.g., if a link between $s_1$ and $s_2$ fails, there is no impact on the reservation on the segment between $s_0$ and $s_1$. This is unlike \FFC{} and \FFCimp{} where such a failure would cause part of the capacity on other links to be unavailable. 
%
%Consequently, a reservation of $2/3$ can be guaranteed on the segment $su$ under any single link failure. Likewise, a reservation of $1$ can be guaranteed from $ut$ under any single link failure. Hence, a reservation of $2/3$ units can be guaranteed from $s$ to $t$.
%
The corollary to Proposition~\ref{prop:ffcimp_bad} below captures the resulting  benefits.
%
\begin{corollary}
For the topology in Fig.~\ref{fig:parallel_example_g},
\System{}'s performance with a single \LS{} and polynomially many tunnels can be arbitrarily better than \FFCimp{} and \FFC{} with exponentially many tunnels. 
\label{cor:ls_reaches_optimal}
\end{corollary}
%
{\bf Proof.} 
We have already shown that \FFC{} and \FFCimp{} can be arbitrarily worse than optimal. Consider \System{} where \LS{} $q$ corresponding to $s_0,s_1,...,s_m$ is used, with each link being a tunnel. There are $p+n(m-1)$ tunnels in total. Under any scenario involving $n-1$ simultaneous link failures, the first segment ($s_0s_1$) has a capacity of at least $1 - \frac{n-1}{p}$  available. All other segments have at least capacity $1$ available on any $n-1$ failure scenario. Thus, $q$ can carry at least $1 - \frac{n-1}{p}$ traffic, which meets the optimal throughput. $\square$

We note that using the \LS{} has at least two sources of flexibility beyond classic tunneling. First, in classic tunneling, 
traffic on each tunnel only carries traffic corresponding
to the end points of the tunnel. Second, when there is a failure,
only the source node of a tunnel may respond. In contrast,
with a \LS{}, each segment may carry traffic corresponding to
different sources and destinations - for instance, 
in Fig.~\ref{fig:parallel_example_g}, the segment 
(and hence tunnel) between $s_1$ and $s_2$ may carry traffic between
$s_0$ and $s_m$. Further, if the link between $s_1$ and $s_2$ fails,
$s_1$ may redistribute the traffic that arrives at $s_1$ onto the 
tunnels between $s_1$ and $s_2$.

\noindent
\textbf{Bandwidth allocation with \LS{}s.}
We next show that bandwidth allocation with \LS{}s can be tractably formulated. For each pair with source $s$ and destination
$d$, let $L(s,t)$ denote the set of \LS{}s from $s$ to $t$
(with $T(s,t)$ denoting the set of tunnels as before). Note that
each source destination pair is associated with zero or more \LS{}s, and zero or more tunnels. Then, the model seeks to reserve $b_q$ on each \LS{}, and reserve $a_l$ on each tunnel $l$ as discussed below:
%
\begin{align}
\mbox{($P2$)} \ 
& \max_{z,a,b} \quad \Theta(z) \nonumber\\
\mbox{s.t.} \quad & 
\sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + \sum_{q \in L(s,t)} b_{q} \nonumber\\
& \ge \sum_{q' \in Q(s,t)} b_{q'} + z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y \label{eq:capconstraint}\\
& b_{q} \ge 0 \quad \forall s,t \in V, q \in L(s,t) \nonumber\\
& \mbox{Constraints} \  \eqref{eq:al_1}, \eqref{eq:al_2} \nonumber
%\label{eq:vs_model}
\end{align}
%
The most significant change relative to \eqref{eq:tunnel_model} pertains to the capacity constraint (first constraint). The LHS of this constraint captures that traffic from $s$ to $t$ could use both the reservations ($a_l$) on the physical tunnels  between $s$ and $t$, and the reservations ($b_q$) on the \LS{}s between $s$ and $t$. While the capacity on tunnel $l$ is only available when all links on the tunnel are alive ($y_l=0$), the reservation on the \LS{} $q$ is always available (though we relax this requirement in \S\ref{sec:ls_with_hint}). The RHS of this constraint corresponds to the total traffic that must be carried from $s$ to $t$. 
With \FFC{}, this corresponds entirely to the bandwidth allocated to traffic
that originates at $s$, and terminates at $t$. However, in \System{}, it is possible that $st$ is a segment of a \LS{} $q'$ (between a source $s'$ and destination $t'$). Let $Q(s,t)$ denote the set of all such \LS{}s. Then, 
the RHS also accounts for reservations on all such $q' \in Q(s,t)$. We refer to
(P2) as the \textbf{\SysLS{}} model. Note that the reservation on a \LS{} is supported by the reservations on physical tunnels and other \LS{}s. The reservations on physical tunnels themselves are supported by the capacity of underlying physical links. 
%We remark that, as in corollary \ref{cor:ls_reaches_optimal}, \System{} achieves the optimal throughput for the network in Figure \ref{fig:parallel_example_g} when $b_q=z_{st} = 1- \frac{n-1}{p}$ for the \LS{} $(s_0,s_1,...,s_m)$.



%We will discuss in \S\ref{sec:practical} how the scheme may be practically realized. In \S\ref{sec:evaluation} we will show the benefits of \System{} empirically,
%and show that simple heuristics to pick \LS{}s are effective.


%that a routing scheme with a centralized controller can be easily derived from \eqref{eq:vn_model}'s solution. Furthermore, with additional assumption on the choice of logical sequences, a distributed routing scheme similar to FFC can be easily implemented.


%We call \eqref{eq:vn_model} the virtual network model \sgr{Check model name later.} We introduce a new variable $b_q$ which represents the amount of reservation we make on the logical sequence $q$. Similar to physical tunnels, we make sure the reservation on the logical sequence should always be non-negative. On the capacity constraint(first constraint), for each node pair $(s,t)$, now we can use both the reservation on physical tunnels($a_l$) and the reservation on logical sequences($b_q$) to route traffic. And if $s-t$ is a segment of a logical sequence, then $s-t$ should also carry traffic for this logical sequence, other than the original demand from $s$ to $t$. Other constraints are exactly the same as in \eqref{eq:vn_model}. Note that in the model, reservation on a physical tunnel is supported by the capacity of underlying physical links. The reservation on a logical sequence is supported by the capacity of both the physical tunnels and logical sequence in the underlying hops. We will show in \S\ref{sec:practical} that a routing scheme with a centralized controller can be easily derived from \eqref{eq:vn_model}'s solution. Furthermore, with additional assumption on the choice of logical sequences, a distributed routing scheme similar to FFC can be easily implemented.



%By decomposing the path from $s_0$ to $s_m$ into segments, using a logical sequence can achieve optimal performance with polynomially many tunnels in Figure \ref{fig:parallel_example_g}.






==> wbackground.tex <==
\section{Motivation}
\sgr{We may revert to doing System-TF first, then logical sequence etc.. To Be decided}.

In recent years, researchers have investigated ways to design networks to 
proactively ensure that it is congestion-free over a desired set of failures~\cite{r3:sigcomm10,ffc_sigcomm14,DRCN14}. A common practice is to 
design networks for $f$ \sgr{Can we go with $f$?} simultaneous link failures.

To illustrate these schemes, consider \FFC{}~\cite{\FFC_sigcomm14}, a recent and representative approach set in the context of tunnel-based forwarding. Consider a network where each pair of nodes $(s,t)$ is associated with a traffic demand $d_{st}$, and a set of tunnels $T_{st}$ to route the traffic. \FFC{} seeks to assign a bandwidth $b_{st}$ to each node pair such that this bandwidth \sgr{Check notation} can be guaranteed under all possible $f$ simultaneous link failures. To achieve this, \FFC{} reserves bandwidth on each tunnel, and ensures that the total reservation on all tunnels in $T_{st}$ exceeds $b_{st}$ under every failure scenario of interest. 

%Two points must be emphasized. First, techniques for congestion-free routing ~\cite{r3:sigcomm10,ffc_sigcomm14,DRCN14} are designed for specific ways
%in which networks respond to failures. For instance, with FFC, when any link
%fails, the source node $s$ of an affected tunnel that has been set up from
%$s$ to $t$ can redirect traffic on other live tunnels in the set $T_{st}$.
%These techniques focus on (i) a specific manner in which the network
%responds to failures; and (ii) must apriori decide how to route traffic
%when any 

In the rest of this section, we present examples to illustrate that \FFC{}
can be overly conservative in practice. The insights gained from these
examples motivate our approach.

%As part of \System{}, we have developed a family of techniques that robustly guarantee that the network is congestion-free under $f$ failures, while bridging the gap between \FFC{}, and the optimal response from the network. 


\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={6cm 4.9cm 8cm 7cm}, clip, width=0.48\textwidth]{figures/monotonicity.pdf}
        \label{fig:ffc_example}

    \caption{A simple network with 4 tunnels $T_1$, $T_2$, $T_3$ and $T_4$ from $s$ to $t$. $T_1$ and $T_2$ can carry 1 unit of traffic respectively. $T_3$ and $T_4$ can carry 0.5 unit of traffic respectively. }
        \label{fig:ffc_example}
\end{figure}

\begin{figure}[t]
	\centering
        
	    \includegraphics[ trim={0.5cm 1.5cm 0.5cm 0.5cm}, clip, width=0.48\textwidth]{figures/ffcexampleresult.pdf}
        \label{fig:ffc_example_result}

    \caption{Throughput guarantee ahieved by \FFC{} with different tunnel choices comparing to the optimal}
        \label{fig:ffc_example_result}
\end{figure}




\subsection{Overly conservative failure modeling}
\label{sec:issue_of_non_monotonicity}




%\begin{table}[t]
%  \small
%    \centering
%    \begin{tabular}{||c c c c||} 
%    \hline
%    $k_e$ & Tunnel 1-3 & Tunnel 1-4 & Optimal\\
%    \hline\hline
%    0 & 2.5 & 3 & 3\\  
%    1 & 1.5 & 1 & 2\\ 
%    2 & 0.5 & 0 & 1\\  
%    \hline
%    \end{tabular}
%    \caption{Comparison between the optimal and using FFC with different tunnel options on Fig~\ref{fig:ffc_example} based on throughput matric.}
%    \label{tab:ffc_example}
%    \vspace{-0.4in}
%\end{table}
%\cj{graph annotated with traffic}

Consider Fig.~\ref{fig:ffc_example} where the goal is to carry the maximum amount
of traffic possible from $s$ to $t$, while tolerating any possible single link failure. If the network could respond optimally for each failure scenario (by running an optimal multi-commodity flow for that scenario), it is easy to verify that the network is intrinsically capable of carrying 2 units of flow from $s$ to $t$ under all possible single link failures. When \FFC{} is used, the results
depend on the set of tunnels considered. We start by considering the case where all 4 tunnels $T1$ to $T4$ are used, which we denote as \FFC{}-4. Fig.~\ref{fig:ffc_example_result} shows that only 1 unit of traffic can be carried with \FFC{}-4, much lower than optimal.

\textbf{Why is \FFC{} conservative?}
%We now discuss why \FFC{}'s results are so conservative. 
\FFC{} uses a parameter $p_{st}$ which denotes the maximum number of tunnels between $s$ and $t$ that share
a common link. When designing to tolerate $f$ link failures, \FFC{} conservatively
assumes that upto $f p_{st}$ tunnels may fail, and plans a reservation that
can tolerate all possible failures of $f p_{st}$ tunnels. In the figure,
when \FFC{} uses all 4 tunnels, $p_{st}$ is 2. Hence when designing for single link failures, \FFC{}-4 plans for all possible combinations of two tunnel failures.
This is overly conservative because tunnels $T1$ and $T2$ do not fail together under single link failures.

Interestingly, \FFC{} can perform better when fewer tunnels are used. To illustrate this, we consider a scheme \FFC{}-3, where only tunnels $T1$, $T2$, and $T3$ are used.
Fig.~\ref{fig:ffc_example_result} shows that \FFC{}-3 performs better than \FFC{}-4, but worse than optimal. This is because with \FFC{}-3, all tunnels are disjoint, and $p_{st}=1$. Hence, \FFC{}-3 only needs to be consider single tunnel failures.
However, unlike the optimal scheme, \FFC{}-3 cannot tap into the capacity of 
links $s-4$ and $4-3$. Note that \FFC{} cannot perform better with another choice of 3 (or fewer) tunnels.

Fig.~\ref{fig:ffc_example_result} also shows that if all two link failures
must be tolerated, the optimal is 1, while \FFC{}-3 is 0.5, and \FFC{}-4 is 0.
The reasons are similar to the above -- here, \FFC{}-4 can only service traffic that can survive $p_{st}f = 2 \times 2 = 4$ tunnel failures, and consequently cannot carry any traffic, while \FFC{}-3 only needs to consider all 2 tunnel failure scenarios. 
Overall, these results show that \FFC{} is not only \textit{conservative}, but also its performance may \textit{degrade} with \textit {an increase in the number of tunnels}.




\subsection{Failures lead to unutilized reservations}
\label{sec:issue_of_capacity_competing}

\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={6.5cm 12.2cm 8.5cm 6.5cm}, clip, width=0.48\textwidth]{figures/parallel.pdf}
        \label{fig:parallel_example}

    \caption{A simple topology with 3 nodes and 5 links. We denote a tunnel going through $e_i$ and $e_j$ as $T_{ij}$. There are 6 tunnels $T_{14}$, $T_{15}$, $T_{24}$, $T_{25}$, $T_{34}$ and $T_{35}$ in the topolgy.}
        \label{fig:parallel_example}
\end{figure}
A second issue with \FFC{} is that it is inherently limited by the fact that reservations are made at the granularity of entire tunnels. To illustrate this, consider the topology in Fig.~\ref{fig:parallel_example}. It is easy to verify that if the network responds optimally, it can carry 2/3 units of traffic from $s$ to $t$ under any single link failure. Unfortunately, \FFC{} can only achieve an optimal of 1/2. In \S\ref{}, we will further generalize this example to show that \FFC{} can see arbitrarily poor performance relative to optimal. 

\textbf{Why is \FFC{} conservative?}
The key reason why tunnel-based allocation does not perform as well as optimal is because reservations are made on all links of a tunnel, and when a link fails, the reservations on other links of that tunnel go unutilized. For example, consider a tunnel $l$ that traverses links $e_1$ and $e_4$. When $e_4$ (and hence the tunnel $l$) fails, \FFC{} only uses the reservations on the remaining tunnels, and the reservation on $e_1$ for the failed tunnel $l$ goes unutilized. In contrast, the optimal approach is able to use all capacity on all the non-failed links. 

In the figure above, let $T_4$ and $T_5$ respectively denote the set of tunnels from $s$ to $t$ that use $e_4$ and $e_5$. Let $r_4$ and $r_5$ denote the
amount of reservation that \FFC{} makes on each of these sets of tunnels.
When $e_4$ fails, \FFC{} can carry at most $r_5$ units of traffic, and when
$e_5$ fails, \FFC{} can carry at most $r_4$ units of traffic. Thus, \FFC{} can guarantee at most $\min(r_4,r_5)$ traffic from $s$ to $t$ over all single link
failures. However, $\min \{r4,r5\} \times 2 \leq r4+r5 \leq 1$, where the second inequality is because tunnels in $T4$ and 
$T5$ must reserve capacity in one of the links $e1$, $e2$, or $e3$, whose combined capacity is 1 unit. Hence, \FFC{} can carry at most 0.5 units of traffic from $s$ to $t$.



%To explain this, we present an argument to show that \FFC{} can carry at most $0.5$ units of traffic from $s$ to $t$, regardless of how tunnels are
%chosen. Let $T_4$ and $T_5$ respectively denote the set of tunnels 
%from $s$ to $t$ that use $e_4$ and $e_5$. If \FFC{} could guarantee 
%that more than $0.5$ units of traffic, then the tunnels in $T_4$ should have a reservation that exceeds $0.5$ to handle the failure of link $e_5$. Similarly, tunnels in the set $T_5$ should also have a reservation that exceeds $0.5$ to handle the failure of $e_4$. Then the set of tunnels in $T_4$ and $T_5$ combined must have a reservation that exceeds $1$, which is not possible (since each of these tunnels must reserve capacity in one of the links $e1$, $e2$, or $e3$, whose combined capacity is 1 unit). 



\begin{figure}[t]
	\centering
	    \includegraphics[trim={6.5cm 13.7cm 10.5cm 3cm}, clip, width=0.48\textwidth]{figures/logical_sequence.pdf}
        \label{fig:logical_sequence}

    \caption{An example of a logical sequence and its underlying support.}
        \label{fig:logical_sequence}
\end{figure}




\subsection{\System{}'s approach}
To tackle the issues raised in \S\ref{sec:issue_of_non_monotonicity},
\System{} better models the set of failures over which reservations must be met. \System{} does so while retaining the exact mechanism that \FFC{} employs
to respond to failures (i.e., when a tunnel fails, the source of each tunnel responds by redirecting traffic to other tunnels). We formally show the
resulting approach (which we term \FFCimp{}) is already
(i) guaranteed to out-perform \FFC{}; and (ii) to monotonically improve with the number of tunnels.

%For instance, in  Fig.~\ref{fig:ffc_example}, when all 4 tunnels are used, \System{} captures that the only two tunnel failure that arises from a
%single link failure is the failure of $T4$ and $T3$. Thus, it is 
%sufficient that any reservation be upheld when a single tunnel fails, 
%or when both $T3$ and $T4$ fail, rather than all combinations of two tunnel 
%failures.

To tackle the issues raised in \S\ref{sec:issue_of_capacity_competing}, 
\System{} considers more flexible response strategies. Specifically, \System{} 
abstracts the task of going from source $s$ to destination $t$ into one that involves traversing a series of segments, and ensures that sufficient reservation is made 
on each segment. Fig.~\ref{fig:logical_sequence} illustrates the ideas for the 
above example. Traffic is abstracted as being sent from $s$ to $u$, 
followed by $u$ to $t$, with reservations on each of the segments $su$, and 
$ut$. The failure of links $e_4$ and $e_5$ have no impact on the segment 
$su$. Consequently, a reservation of $2/3$ can be guaranteed on the segment 
$su$ under any single link failure. Likewise, a reservation of $1$ can be guaranteed from $ut$ under any single link failure. Hence, a reservation
of $2/3$ units can be guaranteed from $s$ to $t$.

More generally, \System{} views each pair $s$ to $t$ as comprising of a
one or more series of logical segments. The end points of a logical segment need not be physically adjacent in the underlying topology. The reservations on each logical segment could be made using tunnels, or other logical segments.


%There are 3 tunnels from $s$ to $u$, each comprising a single link, which together must carry the reservation from $s$ to $u$. Similarly, there are 2 tunnels from $u$ to $t$ (each comprising a single link) which together must carry the reservation from $u$  to $t$. To handle single link failure, sufficient capacity is reserved on each of the segments,
%(rather than across all the tunnels from $s$ to $t$). 



%Second, in \FFCimp{}, only the source node of a tunnel can respond to the failure. In contrast, \System{} allows other nodes to respond. For example, if $e_1$ fails, $s$ can respond by redistributing to $T_2$ and $T_3$. If $e_4$ fails, $u$ can respond by redistributing the received traffic to $T_5$. Under any single link failure, at least 2 links between $s$ and $u$ will be alive leaving at least $2/3$ capacity. And at least 1 link between $u$ and $t$ will be alive leaving at least $1$ capacity. So 2/3 unit of traffic can be guaranteed under any single link failure.

%However, in the new scheme, the intermediate nodes can also respond. Third, a tunnel from $s$ to $t$ can only be used to send traffic from $s$ to $t$. In the new scheme, we are now allowing the tunnels to be used for other sources and destinations, providing much more flexibility in routing.


%\sgr{Need to bring out this is more general so people do not view this as too simplistic..lots of logical sequences.. nodes in the sequence need 
%not be physically connected, can be tunnels/sequences etc.}


%We start in \S\ref{} with an approach that we call \FFCimp{} that models the failure scenarios of interest more accurately than
%\FFC{}. In \S\ref{}, we present 







==> ychuan-vnGeneralized.tex <==
\section{\System{} generalizations}
\sgr{PLEASE DO NOT EDIT THIS FILE. TO BE PHASED OUT.}


We introduced in \S\ref{sec:vs_model} the concept of logical sequence and how we use it to design routing with better performance. In this section, we will illustrate the limitation of logical sequence in an example where the virtual network model can not meet the optimal. And we will generalize the idea of logical sequence to provide more flexibility.

\subsection{Limitation of logical sequence}
\label{sec:ls_without_hint}

\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={6cm 4.9cm 8cm 7cm}, clip, width=0.48\textwidth]{figures/vnhintexample.pdf}
        \label{fig:vn_hint_example}

    \caption{A simple network with 6 tunnels from $s$ to $t$. We denote these tunnels as $T_1$, $T_2$, $T_3$, $T_{41}$, $T_{42}$ and $T_{43}$ based on the intermediate hops.}
        \label{fig:vn_hint_example}
\end{figure}

 The main idea of using a logical sequence $q$ is to reserve capacity $b_q$ on given series of hops in $\tau_q$. As shown in the first constraint in \eqref{eq:vs_model}, the usage of logical sequence is not attached to any condition. So the reservation on the logical sequence is always available to be used, which means that we need to make sure the reservation is viable under any failure scenario. If under some failure scenario, it is not possible to make such reservation, then the logical sequence will not be able to help.

Consider the topology in Figure~\ref{fig:vn_hint_example}. Using our model with all 6 tunnels while without any \LS{}, at most $4/3$ unit of traffic can be guaranteed from $s$ to $t$ under single link failure, and at most $2/3$ can be guaranteed under 2 link failures. But the optimal routing can guarantee $3/2$ unit of traffic under any single link failure and $1$ unit of traffic under any two simultaneous link failures. This gap comes from the same issue introduced in \S\ref{sec:issue_of_capacity_competing}. In order to reduce the gap, we can add a logical sequence $s4,4t$ with 1 tunnel from $s$ to $t$ and 3 tunnels from $4$ to $t$ by decomposing tunnels traversing node $4$. But as shown in Fig.~\ref{fig:vn_hint_example_result}, the gap between \VS{} model and the optimal persists. Note that the first hop $(s4)$ relies on single tunnel, hence under the failure of link $s-4$, the logical sequence $s4,4t$ can not carry any traffic. We are not able to guarantee the reservation under one failure scenario. So we can not make any reservation, and logical sequence will not help in this scenario. For the same reason, decomposing other tunnels into \LS{} won't help. For example, if we decompose tunnels traversing node $1$ into \LS{} $s1,1t$, on the failure of $1-t$, the sequence can not carry traffic.

\subsection{Logical sequence with hint}
\label{sec:ls_with_hint}

We look into the optimal routing in Figure~\ref{fig:vn_hint_example} under single link failure. If $s-4$ is the failed link, $s$ can use $T_1$, $T_2$ and $T_3$ to route 1.5 unit of traffic. If $s-4$ is alive, $s$ can use $T_1$, $T_2$ and $T_3$ to route 1 unit of traffic, and route 0.5 unit of traffic through $4$. So $T_{41}$, $T_{42}$ and $T_{43}$ are only needed when link $s-4$ is alive. And the main reason why logical sequence can not help in this scenarios is that we are giving too much 'responsibility' to the logical sequence. We require it to be helpful under all failure scenarios, which is not possible and more importantly, not necessary. In this example, However, if we can add a hint to say we only need \LS{} $s4,4t$ when link $s-4$ is alive, it is possible to reserve 0.5 along the sequence. And we can achieve the optimal routing.

More generally, we introduce logical sequence with hint. A hint can be seen as a condition attached to the logical sequence $q$. We only make reservation on $q$ for those failure scenarios where the hint is true. And we are only able to use $q$ for these failure scenarios. A hint can be a link being alive, a link being dead, or combined conditions among several links. In the example above, the hint for the logical sequence $s4,4t$ is $s-4$ being alive.

To model hints in the optimization, we only need to make small changes in \eqref{eq:vs_model}. Before, we reserve $b_q$ on logical sequence $q$, and don't attach any condition to it so that it will be reserved and available under any failure scenario. Now we only need to attach the hint to it by modifying the first constraint as \cj{model notation}

\begin{align}
\begin{split}
& 
\sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + \sum_{q \in L(s,t)} b_{q} h_{q} \\
& \ge \sum_{q' \in \tau_{st}} b_{q'} h_{q'} + z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y(f), \forall h \in H(f)\\
\end{split}\label{eq:hint_constraint}
\end{align}

$H(f)$ denotes the set of all possible hinting scenarios under $f$ simultaneous link failures. $h_q$ denotes whether the hint of $q$ is true in the hinting scenario $h$. Note that in the most general form, a hint essentially describes an arbitrary subset of all link failure scenarios. But we find that in many cases, a simple hint such as a link being alive or a link being dead is sufficient to greatly improve the performance as in the example above. This also makes the model more tractable. Suppose the hint for \LS{} $q$ is all links in $\eta_q$ are alive and all links in $\xi_q$ are dead, then similar to \eqref{eq:tunnel_model}, we can model $H(f)$ as

\begin{align}
\begin{split}
& \sum_{e \in E} x_e \le k_e \\
& (h_q - 1) + x_e \le 0 \quad \forall q, e \in \eta_{q} \\
& h_q - x_e \le 0 \quad \forall q, e \in \xi_{q} \\
& (1 - h_q) - \sum_{e \in \eta_{q}} x_e - \sum_{e \in \xi_{q}} (1 - x_e) \le 0 \quad \forall q  \\
& 0 \le x_{e} \le 1 \quad \forall e\in E\\
& 0 \le h_{q} \le 1 \quad \forall q\\
\end{split}\label{eq:hint_model}
\end{align}

\subsection{Virtual network}

%The choice of logical sequences apparently will have a great impact on the performance. We want to use a small set of logical sequences to get a good performance improvement. In order to select a good set of logical sequences, we want to further generalize \VS{} model.

As introduced in \S\ref{sec:vs_model}, a logical sequence $q$ from $s$ to $t$ stands for a sequence of hops to guide the traffic from $s$ to $t$. The traffic in each hop will eventually be supported by the underlying tunnels. So if we see a tunnel as a virtual link from the source to the destination, a logical sequence can be seen as a path on the virtual graph constructed by these virtual links. Now, to fully utilize the capacity on the virtual graph, we should route on the whole network instead of being constrained by a given set of paths. Driven by this idea, \VS{} model in \eqref{eq:vs_model} can be further generalized to \VN{} model as 

\begin{align}
\begin{split}
& \max_{z,a,b,p} \quad \Theta(z) \\
\mbox{s.t.} \quad & 
\sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + b_{st}  \\
& \ge \sum_{s',t' \in V} p_{s't'}(st) + z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y(f)\\
& a_{l} \ge 0 \quad \forall s,t \in V, l \in T(s,t)\\
& b_{st} \ge 0 \quad \forall s,t \in V\\
& \sum_{l;\forall s,t \in V, l \in T(s,t)} a_{l} \delta(e \in \tau_{l}^E) \le c_e \quad \forall e \in E\\
& \sum_{j} p_{st}(ij) - \sum_{j} p_{st}(ji) = 
\begin{cases}
b_{st}  \quad \forall s, t, i = s \\
0  \quad \forall s, t, i \ne s, i \ne t \\
-b_{st}  \quad \forall s, t, i = t 
\end{cases} 
\end{split}\label{eq:vn_model}
\end{align}

$b_{st}$ represents the amount of capacity we reserve on the virtual network which can be used to route from $s$ to $t$. $p_{st}(ij)$ stands for the amount of reservation on hop $ij$ in order to build $b_{st}$. The last flow constraint describes how $p_{st}(ij)$ builds $b_{st}$. And $s-t$ also needs to account for its reservation on building for other pairs, so on RHS of the first constraint, we need to add $\sum_{s',t' \in V} p_{s't'}(st)$.

\VN{} model in \eqref{eq:vn_model} provides more flexibility than \VS{} model in \eqref{eq:vs_model} because we can now reserve on the whole network instead of some given set of sequences. This more sophisticated routing can provide us a better understanding of the network's intrinsic capability and how to use the capacity to get a better performance, which can be used to generate \LS{}s to improve the performance of \VS{} model. For example, from $p_{st}(ij)$ we can find paths which take more capacity. Then these paths will be good candidates for \LS{}s to be used in \VS{} model.

\subsection{Virtual network with hint and R3}

Like the logical sequence in \eqref{eq:vs_model}, the reservation $b_{st}$ in \eqref{eq:vn_model} is not attached with any condition. So following the idea introduced in \S\ref{sec:ls_with_hint}, we can further provide flexibility to \VN{} model by associating the reservation with a hint. We denote $W(s,t)$ as the set of all reservation we can use for traffic from $s$ to $t$. Then we associate reservation $w \in W(s,t)$ with a hint $h_w$.  We only need to make such reservation when hint $h_w$ is true, and we can only use it when $h_w$ is true. Then the capacity constraint will be changed to

\begin{align}
\begin{split}
& \sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + \sum_{w \in W(s,t)}b_{w}h_w  \\
& \ge \sum_{s',t' \in V,w' \in W(s',t')} p_{w'}(st)h_{w'} + z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y(f)\\
\end{split}\label{eq:vn_capacity_constraint}
\end{align}

We also need to slightly change the flow balance constraint as below so that we can make multiple reservations for one source-destination pair

\begin{align}
\begin{split}
& b_{w} \ge 0 \quad \forall s,t \in V, \forall w \in W(s,t)\\
& \sum_{j} p_{w}(ij) - \sum_{j} p_{w}(ji) = 
\begin{cases}
b_{w}  \quad \forall s, t, i = s, w \in W(s,t) \\
0  \quad \forall s, t, i \ne s, i \ne t, w \in W(s,t) \\
-b_{w}  \quad \forall s, t, i = t, w \in W(s,t)
\end{cases} 
\end{split}\label{eq:vn_model}
\end{align}

Using hint in virtual network provides additional flexibility in handling failures. \cj{how to go from here to r3?} This model can be seen as a framework which can design a routing based on different levels of flexibility(using \LS{}, using \VN{}, using hint, etc.) In fact, we find that R3, a former work of link-based routing scheme, also lies in this framework.

R3~\cite{r3:sigcomm10} also considers networks under $f$ simultaneous failures. But instead of using tunnels, it attempts to produce a link-based protection mechanism to ensure that the network is congestion-free under all such failures. The essential idea of R3 is to build a bypass for each link which will be used when that link fails. The way it models this, is to have a base routing to specify how the network routes the traffic under no failures, and to have a protection routing to reserve some bypass capacity for each link. When a link fails, the bypass for the failed link will be triggered to take over the traffic. If we look at R3 in our framework, links can be seen as tunnels in our model, base routing is reservation without hint and protection for link $i-j$ can be seen as reservation with hint of $i-j$ being dead. So R3 is a special case of our \VN{} framework where \VN{} with hint is adopted.

\begin{figure}[t]
	\centering
        \includegraphics[trim={0 4cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/r3_example_1.png}
        \label{fig:r3_example_1}

    \caption{Limitation of R3~\cite{r3:sigcomm10}.
        }
    \label{fig:r3_example}
\end{figure}

Unfortunately, R3 is unable to handle various commonly occurring failure scenarios. The key limitation of R3 is that only the end point of a failed link can reroute traffic. And the rerouted traffic has to go to the other end point of the failed link. In the topology shown in Figure~\ref{fig:r3_example}, if any two links fail, it is feasible to route the traffic from the source $s$ to the destination $t$ without exceeding any link capacities. Nevertheless, under such failures, R3 fails to deliver the $s-t$ traffic. More specifically, R3 is unable to protect against the simultaneous failures of links $l_1$ and $l_2$ since, when these links fail, there are no viable bypass paths for either of the links. Because a bypass for $l_1$ has to start at $s$ and end at $5$, and a bypass for $l_2$ has to start at $5$ and end at $6$. Instead, an obvious feasible strategy is to route the traffic along the path $s-3-4-t$, an option that is not considered by R3 because $t$ is not an end point of either $l_1$ or $l_2$.

%\begin{itemize}
%\item Generalizations: Adding hints, and why.
%\item Practical problem: How to find good hints and good virtual network sequences?
%Generalize above model to routing: logical routing vs. logical sequence
%How to find b sequences: decomposition of generalized routing model
%\item Relationship to R3. Background on R3. R3 may be seen as a special case of 
%the above, where hints correspond only to individual links failing, and when a link <i,j> fails, 
%only node i can react. R3 does not work well.
%\end{itemize}



%With the logical sequence introduced in \S\ref{sec:vn_model}, we provide more flexibility in routing comparing to use physical tunnels

%\textbf{Old possibly useful text: Conditional reservation}
%Unfortunately, isolating shared part in tunnels is not enough to handle the example in Figure~\ref{fig:ffc_example}. The main reason is that under 2 simultaneous link failures, we can't guarantee capacity from $S$ to $7$ with only one path to send the traffic. Thus, we are not able to utilize the new tunneling. However, the capacity from $S$ to $7$ is not always needed. As in the policy mentioned in  \S\ref{sec:analysisffc}, if $S-7$ dies, the 3 tunnels without involving $7$ can handle the traffic. We only need the other 3 tunnels when $S-7$ is alive. In other words, we only need to send traffic from $S$ to $7$ when $S-7$ is alive. To achieve this, we are introducing conditional reservation which provides richer flexibility in routing. A conditional reservation means we require a certain amount of capacity only when the associated condition is satisfied. And we also only use it when the same condition is true. In the example in Figure~\ref{fig:ffc_example}, we can make conditional reservation from $S$ to $7$ with the condition being that $S-7$ is alive. Similarly, we can make a conditional reservation from $7$ to $T$ with the same condition. With the associated condition being satisfied, enough capacity can be reserved so that the throughput on the network will met the optimal.




       

==> ychuan_ffcMonotonocity.tex <==
\section{FFC: Monotonicity and Fix}
\label{sec:monotonicity}

\subsection{FFC model}
FFC~\cite{ffc_sigcomm14} is a path-based routing scheme which can compute the bandwidth allocated to each tunnel in order to optimize the performance on the network under $k_e$ simultaneous link failures and $k_v$ simultaneous node failures. Note that in this work, we only focus on link failures, but we can easily add node failures following the same idea. We define a graph $G= \langle V, E 
\rangle $. Each link $e \in E$ is associated with a link capacity $C_e$. For each node pair $(s,t)$ on the graph, we are given a traffic demand $d_{st}$, and a set of tunnels $T_{st}$ to route the traffic. Each tunnel $l$ consists of a set of links $\tau_l^{E} \subseteq E$. Now, the formulation below describes how we can model path-based bandwidth allocation under failures, which is used in FFC. 

\begin{align}
\begin{split}
& \max_{z,a} \quad \Theta(z) \\
\mbox{s.t.} \quad & 
\sum_{l \in T_{st}} a_{l}(1 - y_{l}) \ge z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y\\
& a_{l} \ge 0 \quad \forall s,t \in V, l \in T(s,t)\\
& \sum_{l;\forall s,t \in V, l \in T_{st}} a_{l} \delta(e \in \tau_{l}^E) \le c_e \quad \forall e \in E\\
\end{split}\label{eq:tp_model}
\end{align}


The formulation seeks to determine $a_l$ and $z_{st}$ where $a_l$ represents the amount of reservation on tunnel $l$, and variable $z_{st}$ represents the fraction of traffic from $s$ to $t$ that can be satisfied. $Y$ stands for the set of tunnel failure scenarios of interest, and $y_l$ indicates whether $l$ fails or not in a failure scenario. The key question here is how to model the failure set $Y$. We will discuss how FFC models it and some of its limitation in \S\ref{sec:issue_of_non_monotonicity}.  $\Theta(z)$ is the metric function we want to optimize. Note that $\Theta(z)$ can be any concave function, and this model covers common metrics such as overall throughput and link utilization. For example, we can use $\Theta(z) = \sum_{s,t} min(1,z_{st})d_{st}$ to maximize overall throughput. And we can use $\Theta(z) = min(z_{st})$ and take the inverse of the objective to minimize the link utilization. The idea of this model is to find the valid routing with the maximum performance, that is, to find a valid bandwidth allocation $a$ and scale factors $z$ for the demands so that the performance is optimal and the traffic scaled by $z$ can always be satisfied by the reservation of the residual tunnels under any failure scenario in $Y$.

Clearly, the feasible region, i.e., the set of valid routing, depends on the failure set $Y$. Since we are interested in a routing robust to any $k_e$ simultaneous link failures, we need to know the corresponding tunnel failure scenarios. However, FFC doesn't directly infer tunnel failures from link failures. Instead, FFC estimates the maximum number of tunnel failures, and prepare for the worst-case among all tunnel failure combinations. Suppose in all tunnels between $s$ and $t$, at most $p_{st}$ tunnels share a common link. Then FFC will plan for $k_ep_{st}$ tunnel failures for traffic from $s$ to $t$ under $k_e$ link failures. More formally, FFC models $Y$ as

\begin{align}
\begin{split}
& \sum_{l \in T_{s,t}}y_{l} \le k_ep_{st} \quad \forall s,t \in V\\
& 0 \le y_{l} \le 1 \quad \forall l\\
\end{split} \label{eq:ffc_failure}
\end{align}

The failure set described above may be combinatorially large. Thus, we can use dualization to compress the constraints so that the number of constraint will be polynomial to the size of the network. More detailed formulation can be found in appendix. 

\subsection{Issue of non-monotonicity}
\label{sec:issue_of_non_monotonicity}

Though the failure model in \eqref{eq:ffc_failure} is simple and covers all failure scenarios of interests, it clearly over-estimates the set. In other words, $Y$ may contain tunnel failure scenarios which will never occur under $k_e$ link failures. An over-estimated failure set will result in a more constrained feasible region which can not capture all valid routing upon failures and the performance guarantee may also be conservative. 

%In fact, $k_e$ link failures may not even cause $k_ep_{st}$ tunnel failures, which will be shown in an example next.We will later show in the evaluation section that FFC's modeling of tunnel failures can lead to significantly conservative performance guarantee.

We find that besides giving conservative results, another issue of FFC's modeling of failures is that it is not monotonic on tunnels. \cj{Is this enough for definition?}That is, providing more resource(edges and tunnels) can impair the performance of the model. This will bring difficulties in the network design, especially in the tunnel selection.

\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={6cm 4.9cm 8cm 7cm}, clip, width=0.48\textwidth]{figures/monotonicity.pdf}
        \label{fig:ffc_example}

    \caption{A simple network with 4 tunnels $T_1$, $T_2$, $T_3$ and $T_4$ from $s$ to $t$. $T_1$ and $T_2$ can carry 1 unit of traffic respectively. $T_3$ and $T_4$ can carry 0.5 unit of traffic respectively. }
        \label{fig:ffc_example}
\end{figure}

\begin{figure}[t]
	\centering
        
	    \includegraphics[ trim={0.5cm 1.5cm 0.5cm 0.5cm}, clip, width=0.48\textwidth]{figures/ffcexampleresult.pdf}
        \label{fig:ffc_example_result}

    \caption{Throughput guarantee ahieved by FFC with different tunnel choices comparing to the optimal}
        \label{fig:ffc_example_result}
\end{figure}

%\begin{table}[t]
%  \small
%    \centering
%    \begin{tabular}{||c c c c||} 
%    \hline
%    $k_e$ & Tunnel 1-3 & Tunnel 1-4 & Optimal\\
%    \hline\hline
%    0 & 2.5 & 3 & 3\\  
%    1 & 1.5 & 1 & 2\\ 
%    2 & 0.5 & 0 & 1\\  
%    \hline
%    \end{tabular}
%    \caption{Comparison between the optimal and using FFC with different tunnel options on Fig~\ref{fig:ffc_example} based on throughput matric.}
%    \label{tab:ffc_example}
%    \vspace{-0.4in}
%\end{table}
%\cj{graph annotated with traffic}

\cj{Is it Ok I just dive into throughput matric here?}
\cj{highlight 0 throughput}

Fig.~\ref{fig:ffc_example} shows a simple network in which FFC is not monotonic due to its failure modeling. We consider using 3 tunnels and using 4 tunnels in this network. Fig.~\ref{fig:ffc_example_result} shows how FFC performs with different tunnel choices comparing to the optimal. We consider two tunnel choices. One is to use $T1$, $T2$ an $T3$, which is the best option in using 3 tunnels. The other is to use all 4 tunnels. We obtain the optimal result by enumerating all failure scenarios and running the multicommodity flow model. From the figure, we make the following observation, 1) there is significant gap between FFC and the optimal and 2) as more tunnels are added to FFC, the performance gets worse. Next, we will seek to understand why such issues exist in the FFC model.

The key parameter in FFC is $p_{st}$ which denotes the maximum number of tunnels sharing a common link. The higher the value of $p_{st}$ is, the more conservative the solution will be. When FFC only uses $T1$, $T2$ and $T3$, since these 3 tunnels are disjoint, $p_{st}$ will be $1$ under this option. Without $T4$ carrying 0.5 traffic, it will always be 0.5 less than the optimal. But when $T4$ is added, $T3$ and $T4$ are sharing a common link, making $p_{st}=2$ in this option. Now to plan for single link failure, FFC will plan for all combinations of $k_ep_{st}=2$ tunnel failures. And the worst case happens when $T1$ and $T2$ fail at the same time. Even though this scenario will never happen under single link failure, FFC will include this scenario into $Y$, the failure set of interest, and give the result to only guarantee 1 unit of traffic. To plan for two link failures, FFC will plan for $k_ep_{st}=4$ tunnel failures, which means that all tunnels are not available. Hence it simply can not allocate bandwidth to give any traffic guarantee. But note that 2 simultaneous link failures will not cause all tunnels to fail in this topology, which means that the failure set $Y$ is again over-estimated. Thus, it leaves no valid routing in the feasible region and achieves 0 throughput guarantee.

%We define monotonicity as a property on models. We say a model is monotonic on tunnels, if when more tunnels are added, the performance doesn't get worse. From the example above, FFC is clearly not monotonic on tunnels.

%Without the last tunnel carrying $0.5$ unit of traffic, the first 3 tunnels can only carry 2.5 when there is no failure. For the same reason, under single link failure, only 1.5 traffic can be guaranteed. And only 0.5 traffic can be guaranteed under 2 link failures.

%Table~\ref{tab:ffc_example} shows the throughput guarantee given by FFC under two tunnel options and the optimal result. FFC can not reach optimal under failures in either of these two tunnel options. The first tunnel option is always 0.5 less than the optimal because it doesn't have the fourth tunnel to use. But providing the fourth tunnel to FFC even impairs the throughput guarantee under failures, which means FFC model is not monotonic on tunnels.

\subsection{Better failure model}\label{sec:analysisffc}

Based on the issues in FFC, We want to design a better model which 1) ensures the gap between FFC and the optimal is reduced and 2) the model is monotonic on tunnels. To do this, we need to more accurately model the failure set so that only those tunnel failure scenarios caused by $k_e$ link failures will be captured. So we use a better model for tunnel failures and draw the connection between link failures and tunnel failures directly. Suppose $x_e$ indicates if link $e$ fails, we model $Y$ as 

\begin{align}
\begin{split}
& \sum_{e \in E} x_e \le k_e \\
& x_e - y_l \le 0 \quad \forall l, e \in \tau_{l}^E \\
& y_l - \sum_{e \in \tau_{l}^E} x_e \le 0 \quad \forall l  \\
& 0 \le x_{e} \le 1 \quad \forall e\in E\\
& 0 \le y_{l} \le 1 \quad \forall l\\
\end{split}\label{eq:tunnel_model}
\end{align}

The first constraint bounds the maximum number of simultaneous link failures. The second ensures that any failed underlying link of a tunnel will cause the tunnel to fail. The third ensures that a tunnel only fails when at least one underlying link fails. This set of constraints depict the exact connection between link failures and tunnel failures, and $Y$ will be exactly the set of tunnel failure scenarios under $k_e$ link failures. Thus it will eliminate the gap caused by conservative estimation of tunnel failures in \FFC{}. We denote the optimization problem \eqref{eq:tp_model} with $Y$ modeled by \eqref{eq:tunnel_model} as \FFCimp{}. Next, we will show that \FFCimp{}'s performance will not be worse than \FFC{}'s.

\begin{proposition}\label{prop:ffcim_beats_ffc}
The feasible region of FFC is contained in the feasible region of \FFCimp{}, so \FFCimp{} performs at least as well as FFC for any metric.
\end{proposition}
{\bf Proof.} 
 
Let $Y_0$ be the set of all tunnel failure scenarios considered by FFC(constrained by \eqref{eq:ffc_failure})
and let $Y_1$ be the set of all tunnel failure scenarios considered by \FFCimp{}(constrained by \eqref{eq:tunnel_model}). For any $s,t\in V$ we sum the last constraint in \eqref{eq:tunnel_model} over all $l \in T_{st}$ to get

\begin{align}
\begin{split}
& \quad \sum_{l\in T_{st}}(y_l - \sum_{e \in \tau_{l}^E} x_e ) \le 0 \quad \forall s,t \in V
\end{split}
\end{align}

Thus

\begin{align}
\begin{split}
& \quad \sum_{l\in T_{st}}y_l \\
& \le \sum_{l\in T_{st})}\sum_{e \in \tau_{l}^E} x_e  = \sum_{l\in T_{st}}\sum_{e \in E} x_e\delta(e \in \tau_{l}^E) \\
& = \sum_{e \in E} x_e\sum_{l\in T_{st}}\delta(e \in \tau_{l}^E)  \le k_ep_{st}
\end{split} 
\end{align}

which shows that any scenario in $Y_1$ also satisfies \eqref{eq:ffc_failure}. So $Y_1 \subseteq Y_0$. Then \FFCimp{}'s constraints are contained in \FFC{}'s constraints. And \FFC{}'s feasible region is contained in \FFCimp{}'s.
$\square$

Note that the above proof doesn't depend on the objective function in the optimization problem, which means that the proposition holds for any metric. Then, we will also show that \eqref{eq:tp_model} with $Y$ modeled by \eqref{eq:tunnel_model} is monotonic on tunnels. 

\begin{proposition}\label{prop:ffcim_beats_ffc}
As we provide more tunnels, \FFCimp{}'s performance will not decrease.
\end{proposition}
\cj{proof needs some modification}
{\bf Proof.} 


Let $\{T_0(s,t)|\forall s,t \in V\}$ and $\{T_1(s,t)|\forall s,t \in V\}$ be two sets of tunnels, and $T_0(s,t) \subseteq T_1(s,t)$ for all $s,t \in V$. Then the optimal solution to \eqref{eq:tp_model} with $T = T_1$ will not be worse than the optimal solution to \eqref{eq:tp_model} with $T = T_0$.
Let $(a^*, b^*)$ be the optimal solution to \eqref{eq:tp_model} with $T = T_0$. We construct $(a', b')$ in the following way,

\begin{align}
\begin{split}
& a'_l = a^*_l \quad \forall s,t \in V, l \in T_0(s,t)\\
& a'_l = 0 \quad \forall s,t \in V, l \in T_1(s,t) - T_0(s,t)\\
& b'_{st} = b^*_{st} \quad \forall s,t \in V\\
\end{split}
\end{align}

It is easy to see that $(a', b')$ is a solution to \eqref{eq:tp_model} with $T = T_1$. Since $b'=b^*$ and the objective is the sum over all $b$, the objective of $(a', b')$ is the same as the objective of $(a*, b*)$. So the optimal solution with $T = T_1$ is at least as good as the optimal solution with $T = T_0$.
$\square$

Based on the above propositions, using failure model in \eqref{eq:tunnel_model} can solve non-monotonicity issue of the conservative way to model failures. And using \eqref{eq:tunnel_model} will be at least as good as the original failure model. We will later show in \S\ref{sec:evaluation} that \eqref{eq:tunnel_model} provides significantly better performance in real networks.





==> ychuan_practical.tex <==
\section{Deriving practical routing schemes}\label{sec:practical}

In \S\ref{sec:system}, we introduced our \System{} and how we can generalize the model to provide more flexibility in routing hence to give better performance guarantee. Next, we will illustrate two ways to practically implement routing schemes obtained from our model. We claim that (i) with help of a controller, our generalized model can be implemented as a centralized routing scheme which only needs to solve a linear system upon any link failure; (ii) with an additional assumption on the choice of \LS{}s, our \LS{} model can be implemented as a distributed routing scheme which does proportional assigning traffic just as FFC does.  

%\begin{itemize}
%    \item Proposition: Solving the general case involves solving a linear system globally
%and reinstall the rules.
%    \item Theorem: (Harder): Need to show that the solution of the linear system is between 0 and 1.
%    \item Centralized, but linear system is quick to solve Discuss results below that show distributed possible.
%\end{itemize}

\subsection{Centralized routing by solving linear systems}

In this centralized scheme, upon the update on the failure scenario(initialization, link failure, link recovery), we need a controller to recompute the weights and reinstall the weights in the routers. We claim that the recomputation only requires solving $|V|^2$ linear systems with $|V|^2$ variables and $|V|^2$ equations. A linear system only contains equations, which is usually much less complicated to solve than an LP with similar size. Thus, the update of routing weight can be much faster comparing to update by solving an LP.

Upon failure scenario $x$, let $T_x(s,t)$ denote the set of alive tunnels from $s$ to $t$, $W_x(s,t)$ denote the set of active virtual flow from $s$ to $t$ and $R_x(s,t)$ denote the amount of capacity available to transmit traffic from $s$ to $t$. Then we have $R(s,t) = \sum_{l \in T_x(s,t)} a_{l} + \sum_{w \in W_x(s,t)}b_{w}$. Suppose $\forall s,t \in V$, we actually use $u(s,t)$ fraction of $R(s,t)$ for routing. Then to make the used capacity match the traffic going through, we will have $u(s,t)R(s,t) = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(st)u(s',t') + z_{st}d_{st}$. Thus, we can write a linear system as
\begin{align}
\begin{split}
& \quad u(s,t)\big(\sum_{l \in T_x(s,t)} a_{l} + \sum_{w \in W_x(s,t)}b_{w} \big) \\
& = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(st)u(s',t') + z_{st}d_{st} \quad \forall s,t \in V
\end{split}\label{eq:linear_system_vf}
\end{align}
where $u(s,t)$ are the variables.

If there exists a solution $u^*(s,t)$ to this linear system and $\forall s,t \in V, u^*(s,t) \in [0,1]$, then $\forall l \in T_x(s,t)$, $u^*(s,t)a_l$ is the amount of traffic that will be carried by tunnel $l$. And we can prove that with the capacity constraint \eqref{eq:vn_capacity_constraint} being satisfied, such solution always exists.

\begin{proposition}\label{prop:linear_system}
There always exists a solution $u^*(s,t)$ to the linear system in \eqref{eq:linear_system_vf} such that $\forall s,t \in V, u^*(s,t) \in [0,1]$.
\end{proposition} \cj{proof needed here}

In \System{}, a tunnel from $s$ to $t$ can be used to route traffic for other source-destination pairs. So we solve similar linear systems, one for each demand entry $d_{\bar{s}\bar{t}}$. That is, $\forall \bar{s}, \bar{t} \in V$, we solve a linear system which only accounts for the demand from $\bar{s}$ to $\bar{t}$. And the linear system is
\begin{align}
\begin{split}
& \quad u_{\bar{s}\bar{t}}(\bar{s},\bar{t})\big(\sum_{l \in T_x(\bar{s},\bar{t})} a_{l} + \sum_{w \in W_x(\bar{s},\bar{t})}b_{w} \big) \\
& = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(\bar{s}\bar{t})u_{\bar{s}\bar{t}}(s',t') + z_{\bar{s}\bar{t}}d_{\bar{s}\bar{t}} \\ 
& \quad u_{\bar{s}\bar{t}}(s,t)\big(\sum_{l \in T_x(s,t)} a_{l} + \sum_{w \in W_x(s,t)}b_{w} \big) \\
& = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(st)u_{\bar{s}\bar{t}}(s',t')  \quad \forall s,t \in V, (s, t) \ne (\bar{s}, \bar{t})
\end{split}\label{eq:linear_system_vf_single}
\end{align}

$\forall l \in T_x(s,t)$, $u^*_{\bar{s}\bar{t}}(s,t)a_l$ is the amount of traffic from $\bar{s}$ to $\bar{t}$ that will be carried by tunnel $l$, which is the weight needed to be installed in router $s$. Based on the same argument for above proposition, there always exists a solution $u^*_{\bar{s}\bar{t}}(s,t)$ to the linear system in \eqref{eq:linear_system_vf_single} such that $\forall s,t \in V, u^*_{\bar{s}\bar{t}}(s,t) \in [0,1]$. And it is obvious that $u^*(s,t) = \sum\limits_{\forall \bar{s},\bar{t} \in V} u^*_{\bar{s}\bar{t}}(s,t)$ is a solution to \eqref{eq:linear_system_vf}. So this routing is valid. 

\subsection{Distributed routing by proportionally assigning traffic}

FFC uses a distributed routing scheme. It installs the value of tunnel reservation($a_l$) as the weight in the source nodes of tunnels. On each scenario, FFC distributes traffic to the alive tunnels proportionally to the weights. It doesn't require help of a centralized controller. After the tunnel weights are installed, routers can adapt to failures by themselves. Our \FFCimp{}, which improves the failure model of FFC, clearly can use the same distributed routing strategy. Next, we will show that even our \System{}, under some assumption on the provided \LS{}s, can also use a similar distributed routing scheme. In this routing strategy, we need to install both the tunnel reservation($a_l$) and \LS{} reservation($b_q$) as the weight in the source nodes. Routers will then distribute traffic to the alive tunnels and alive \LS{} proportionally to the weights. \cj{not sure how to talk about it here...use an example? Do I say using labels?}

This routing strategy doesn't work for all \LS{} choices. Because we allow a \LS{} can use another \LS{} and hence the traffic might be distributed recursively. For example, suppose a \LS{} $q_1$ from $i_1$ to $j_1$ has a segment $i_2j_2$ in it, while a \LS{} $q_2$ from $i_2$ to $j_2$ has a segment $i_1j_1$ in it. Then traffic from $i_1$ to $j_1$ might be distributed to $q_1$, which will need to go through segment $i_2j_2$. When going from $i_2$ to $j_2$, $q_2$ might be chosen to be used, which will need to go through $i_1j_1$ and cause recursion. In order to make proportionally distributing scheme work, we need to choose \LS{}s so that such recursion will never occur.



\subsection{Topological sorting and benefits}
\textbf{Definition:}
b with node pairs being topologically sorted(if a logical sequence of node pair (i,j) involves another node pair (i1, j1), then no logical sequence of node pair (i1, j1) can involve node pair (i, j): 

\textbf{Theorem:} Under the topologically sorted assumption, a local proportionally
distributed routing policy works. This is similar to ffc policy.

\textbf{Implications:}
\begin{itemize}
    \item Send to active b and live tunnels, rescaling to maintain proportion
    \item Active b: hint says it is active [no hint model: always active]
    \item Failure propagation to check which a are alive: Exactly FFC
    \item Hint propagation to check which b are active: New. [No-hint model: not
 needed].
    \item As of now, hint propagation centralized. TBD: is distributed possible under
 some cases?
 \end{itemize}

\subsection{General case}
Not sure to cover in paper: General case: Diagonally dominant LS; Can be partitioned into many 
strictly diagonally dominant LS. This is amenable to distributed implementation (or very fast 
centralized implementation).
	
\subsection{proof}

\cj{a few notations may be a bit confusing and conflicting the previous sections because sec 4 and 5 are not written yet.}

We define a graph $G=\langle V, E \rangle$ where $V$ is the set of nodes and $E$ is the set of edges. Each edge $e \in E$ is associated with an edge capacity $C_e$. For each node pair $(s,t)$ on the graph, we are given a traffic demand $d_{st}$, and a set of physical tunnels $T_a(s,t)$ and a set of logical sequences $T_b(s,t)$ we can use to route traffic. If a physical tunnel $l$ consists of an edge $e$, then $e \in L_a(l)$. If a logical sequence $q$ uses node pair $(i,j)$, then $q \in L_b(i,j)$.

We also define a relation 'cover' on $\langle V^2, V^2 \rangle$. If $T_b(i,j) \cap L_b(i',j') \neq \emptyset$, we define that $(i,j)$ covers $(i',j')$.

We solve the virtual network model to get a set of variables $b(q)$ on all logical sequences and $a(l)$ on all physical tunnels which satisfies the following constraints:

\begin{align}
\begin{split}
& d_{i,j} + \sum_{q \in L_b(i,j)} b_q \le \sum_{l \in T_a(i,j)} a_l + \sum_{q \in T_b(i,j)} b_q \quad \forall i, j \in V \\
& \sum_{l \in L_a(i,j)} a_l \le c_{i,j} \quad \forall \langle i, j \rangle \in E \\
\end{split}
\end{align}

We define $sd(q) = (i,j)$ if $q \in T_b(i,j)$, then a routing can be found by solving the following linear system 

\begin{align}
\begin{split}
& d_{i,j} + \sum_{q\in L_b(i,j)}Z(sd(q))b(q) = Z(i,j)(\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)) \\
\end{split}\label{eq:linear_system}
\end{align}

To write as matrix, we are solving $Z$ for $AZ=D$, where $A_{(i,j),(i,j)} = \sum_{l \in T_a(i,j)} a_l + \sum_{q \in T_b(i,j)} b_q$, $A_{(i,j),(i',j')} = -\sum_{q \in L_b(i,j) \cap T_b(i',j')} b_q$, $D_{(i,j)} = d_{i,j}$.

\begin{proposition}\label{prop:linear_system}
A valid routing always exists from the virtual network model. More formally, there always exists a solution to \eqref{eq:linear_system} in $[0,1]^{|V^2|}$. 
\end{proposition}

{\bf Proof.} 
We use fixed-point theorem to prove this. Let $f(Z)$ be a function with mapping from $[0,1]^{|V^2|}$ to $\mathbb{R}^{|V^2|}$. And we define $f(Z)$ as

\begin{align}
\begin{split}
& f(Z)_{i,j} = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z(sd(q))b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \\
\end{split}
\end{align}

It is easy to see that $Z_0$ is a solution to \eqref{eq:linear_system} if $f(Z_0) = Z_0$. With $Z \in [0,1]^{|V^2|}$, we have 

\begin{align}
\begin{split}
& f(Z)_{i,j} \ge \frac{d_{i,j}}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \ge 0 \\
\end{split}
\end{align}

and 

\begin{align}
\begin{split}
& f(Z)_{i,j} \le \frac{d_{i,j} + \sum_{q\in L_b(i,j)}b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \le 1 \\
\end{split}
\end{align}

Since $f$ is a continuous function mapping from from $[0,1]^{|V^2|}$ to $[0,1]^{|V^2|}$, and $[0,1]^{|V^2|}$ is a compact convex set, based on fixed-point theorem, we know that there is at least one point $Z_0$ so that $f(Z_0) = Z_0$.
$\square$

Now assume all node pairs can be topologically sorted based on the cover relation, we claim that we can route the demand in this strategy: Distribute traffic for node pairs in the topological order. And for each node pair $(i,j)$, distribute the demand and the flow from $L_b(i,j)$ to the physical tunnels $T_a(i,j)$ and $T_b(i,j)$ proportionally based on $a(l)$ and $b(q)$. 

\begin{proposition}\label{prop:topological_sort}
If all node pairs can be topologically sorted based on the cover relation, then assigning traffic proportionally will be a valid routing.
\end{proposition}

{\bf Proof.} 
We will formally define the proportional rules and show that by doing so, we will get a valid solution to \eqref{eq:linear_system}. We define $Z_a(l)$ as the amount of traffic on tunnel $l$ and $Z_b(q)$ as the amount of traffic on physical sequence $q$. Then we assign the value to $Z_a(l)$ and $Z_b(q)$ in the topological order of node pairs. We assign the value as below using the proportional rules:

\begin{align}
\begin{split}
& Z_a(l') = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)}a(l') \quad \forall l' \in T_a(i,j)\\
& Z_b(q') = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)}b(q') \quad \forall q' \in T_b(i,j)\\
\end{split}
\end{align}

Since the values are assigned in the topological order, so $\forall q \in L_b(i,j)$, $Z_b(q)$ is assigned before $(i,j)$. So this strategy is well-defined.

Now for any $(i,j)$, if we sum $Z_a(l)$ and $Z_b(q)$ over all $l \in T_a(i,j)$ and $q \in T_b(i,j)$, we get

\begin{align}
\begin{split}
& d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q) = \sum_{l\in T_a(i,j)}Z_a(l) + \sum_{q\in T_b(i,j)}Z_b(q) \\
\end{split}
\end{align}

Let $Z(i,j) = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)}$. Then the above equation becomes exactly the linear system we need to solve. So $Z(i,j)$ is a solution.

We then show by induction that $Z(i,j) \in [0,1]$ for all node pairs $(i,j)$. Suppose $(i_0,j_0)$ is the first node pair in the topological order. Then we have $L_b(i_0,j_0) = \emptyset$. So $Z(i_0,j_0) = \frac{d_{i_0,j_0}}{\sum_{l\in T_a(i_0,j_0)}a(l) + \sum_{q\in T_b(i_0,j_0)}b(q)} \in [0,1]$. 
Now for node pair $(i,j)$ which is not the first in the topological order, suppose for every node pair $(i',j')$ previous to $(i,j)$  in the order, we have $Z(i',j') \in [0,1]$. Then

\begin{align}
\begin{split}
& Z(i,j) = \frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z_b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \\
& \quad \quad \quad  =\frac{d_{i,j} + \sum_{q\in L_b(i,j)}Z(sd(q))b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \\
& \quad \quad \quad \le \frac{d_{i,j} + \sum_{q\in L_b(i,j)}b(q)}{\sum_{l\in T_a(i,j)}a(l) + \sum_{q\in T_b(i,j)}b(q)} \le 1
\end{split}
\end{align}

Similarly, we can show that $Z(i,j) \ge 0$. So by induction, $Z(i,j) \in [0,1]$ for all node pairs $(i,j)$. 
$\square$








==> ychuan_vnNoHintModel.tex <==
\section{Virtual Network Model}

\label{sec:vn_model}
In \S\ref{sec:monotonicity}, we use a better way to describe tunnel failures which gives us a monotonic model and can improve throughput guarantee significantly. But even with the better failure model, we find that \eqref{eq:tp_model} is still not desirable in many scenarios with enough or even all possible tunnels. In this section, we will illustrate the issue and introduce our solution.  

\subsection{Issue of capacity competing}
\label{sec:issue_of_capacity_competing}

\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={6.5cm 12.2cm 8.5cm 6.5cm}, clip, width=0.48\textwidth]{figures/parallel.pdf}
        \label{fig:parallel_example}

    \caption{A simple topology with 3 nodes and 5 links. We denote a tunnel going through $e_i$ and $e_j$ as $T_{ij}$. There are 6 tunnels $T_{14}$, $T_{15}$, $T_{24}$, $T_{25}$, $T_{34}$ and $T_{35}$ in the topolgy.}
        \label{fig:parallel_example}
\end{figure}

Consider the topology in Figure~\ref{fig:parallel_example}. In the optimal routing, 2/3 unit of traffic can always be guaranteed from $s$ to $t$ under any single link failure. However, \FFCimp{} can guarantee no more than 1/2 unit of traffic. 

Suppose using the model in \eqref{eq:tp_model} can guarantee more than $1/2$ throughput under single failure. Then the model has to allocate more than $1/2$ unit of bandwidth to $T_{14}$, $T_{24}$ and $T_{34}$ in order to handle failure of link $e_5$. Similarly, $T_{15}$, $T_{25}$ and $T_{35}$ also need to be allocated with more than $1/2$ unit of bandwidth in case $e_4$ fails. Then all six tunnels will be allocated with more than of 1 unit of bandwidth, which is not possible in this topology.

The reason why tunnel-based allocation as \eqref{eq:tp_model} can not handle such topology is that tunnels are competing on the shared links. And since the allocation is apriori, once the capacity is allocated, there is no way for tunnels to adjust according to failures. For example, suppose $a'$ amount of capacity is allocated to the tunnel constructed by $e_1$ and $e_4$. When $e_1$ fails, this tunnel can not be used. Not only $e_1$ is not used, $a'$ capacity in link $e_4$ is also wasted in this scenario, because it is assigned apriori and can not be reallocated to the tunnel from $e_2$ or $e_3$. And due to the waste of capacity upon failures, \eqref{eq:tp_model} can never reach the optimal in such topologies. 

Note that we already exploit all viable paths in the topology. But \FFCimp{} still can not meet the optimal. And this result can be generalized to larger topologies. In larger topologies, there can be exponentially many paths on such parallel sequences. It is not even possible to establish tunnels for all paths in order to exploit the network capacity. In fact, we can show that in the similar structure, the throughput guarantee given by \FFCimp{} can be arbitrarily worse, even when we provide all possible tunnels. 

\cj{TODO: includes $\Theta$}
\begin{figure}[t]
	\centering
        
    	    \includegraphics[trim={5.5cm 11.7cm 7.5cm 8cm}, clip, width=0.48\textwidth]{figures/parallel_example_g.pdf}
        \label{fig:parallel_example_g}

    \caption{A topology with $m$ nodes generalized from the previous example.}
        \label{fig:parallel_example_g}
\end{figure}


\begin{proposition}\label{prop:ffcim_beats_ffc}
\FFCimp{}'s performance can be arbitrarily worse than the optimal even with exponentially many tunnels.
\end{proposition}
{\bf Proof.} 


Consider the topology in Figure~\ref{fig:parallel_example_g}. There are totally $n^{m+1}$ tunnels. We will show that \FFCimp{} can not guarantee traffic larger than $1/n$ from $s_0$ to $s_m$ under $n-1$ simultaneous link failure while the network can always serve $1 - \frac{n-1}{p}$ in the optimal solution.

The total traffic going from $s_0$ to $s_1$ can not exceed 1, constrained by the total link capacity between $s_0$ and $s_1$. So at least one link between $s_1$ and $s_2$ will be assigned with 1/n or less bandwidth in \FFCimp{}'s apriori allocation. Thus, failing all other $n-1$ links between $s_1$ and $s_2$ will leave no more than $1/n$ capacity.

It is easy to see that under any $n-1$ failures, $s_0-s_1$ will have at least $p -(n-1)$ links alive and have total capacity of $1 - \frac{n-1}{p}$. And for all $i>1$, at least 1 link is alive between $s_i-s_{i+1}$ with capacity of 1. So capacity of $1 - \frac{n-1}{p}$ is always available.

Note that $1 - \frac{n-1}{p} > 1/n$ for all $p > n$. The example in Figure \ref{fig:parallel_example} is a special case when $p = 3$, $n = 2$ and $m = 2$. Consider further the case where $p = n^2$. In this case, it can be verified that as $n$ is getting larger, the amount of traffic carried in the optimal solution will be closer to 1. In contrast, \FFCimp{} will converge to 0.
$\square$



%\begin{itemize}
%\item parallel links example
% The number of tunnels can be exponential with long sequence

%\item Theoretical result:
%Theorem:  FFC-improved result can be arbitrarily bad

%\item Virtual network modeling
%A reservation builds a virtual network
%introduce logical sequence reservation b, b will need to be supported by its underlying hops
%\item ab no hinting model
%\end{itemize}


%\textbf{Old possibly useful text.}
%One of the reasons why FFC is not able to handle the example in Figure~\ref{fig:ffc_example} is that FFC can not distinguish the shared part among tunnels. Hence when it is doing reservation, it has to reserve the shared part multiple times in order to allocate to different tunnels, leading to a capacity bottleneck. For example, in Figure~\ref{fig:ffc_example}, link $S-7$ is a shared link for 3 tunnels. In FFC model, all these three tunnels are competing the capacity in $S-7$, resulting in a lower utilization. Our solution for this issue is to split the tunnels. More specifically in this example, we can split the 3 tunnels into a short tunnel from $S$ to $7$, and 3 tunnels from $7$ to $T$. In this way, tunnels will not compete for capacity in link $S-7$ anymore. If there is any traffic going from $S$ to $7$, $7$ will decide which tunnels to use instead of letting $S$ decide. Note that comparing to FFC, this is not simply changing the provided tunnels. It is fundamentally different from FFC because FFC only allows tunnels from the source of a flow to the destination of flow. Here, we will not pose any limitation on how the tunnels will be used.

\subsection{Logical sequence and virtual network}

We first illustrate our solution in Figure \ref{fig:logical_sequence}. We break down the path from $s$ to $t$ into two segments $s-u$ and $u-t$. There are 3 tunnels from $s$ to $u$, each comprising a single link. Similarly, there are 2 tunnels from $u$ to $t$, each comprising a single link. We then decompose the task of sending traffic from $s$ to $t$ into series of sub-tasks. We send traffic from $s$ to $u$ first, then send from $u$ to $t$. If a link fails, traffic can be redistributed among tunnels in each affected segment. For example, if $e_1$ fails, $s$ can respond by redistributing to $T_2$ and $T_3$. If $e_4$ fails, $u$ can respond by redistributing the received traffic to $T_5$. Under any single link failure, at least 2 links between $s$ and $u$ will be alive leaving at least $2/3$ capacity. And at least 1 link between $u$ and $t$ will be alive leaving at least $1$ capacity. So 2/3 unit of traffic can be guaranteed under any single link failure.

The key reasons why this strategy will give better performance than \FFCimp{} are following. First, in \FFCimp{}, when link $e_1$ fails, the capacity reserved by $T_{14}$ and $T_{15}$ is gone, wasting some capacity on $e_4$ and $e_5$. In contrast, with the new approach, since we decompose $s-t$ into $s-u$ and $u-t$, after $s$ sends traffic to $u$, $u$ has the flexibility to use all the capacity in $e_4$ and $e_5$ to send to $t$. Second, in \FFCimp{}, only the source node of a tunnel can respond to the failure. However, in the new scheme, the intermediate nodes can also respond. Third, a tunnel from $s$ to $t$ can only be used to send traffic from $s$ to $t$. In the new scheme, we are now allowing the tunnels to be used for other sources and destinations, providing much more flexibility in routing.

More generally, we view $s$ to $t$ as comprising a logical sequence $q$ consisting of hops $s, a_0, a_1,...,a_m, t$. In each segment, it either comprises physical tunnels, or other logical sequences. We will allocate bandwidth so that this logical sequence $q$ can always carry $b_q$ amount of traffic. Then any traffic from $s$ to $t$ can be sent through $q$ by going through series of segments $s-a_0,a_0-a_1,...,a_m-t$. By using a logical sequence, we can also achieve the optimal performance in the topology shown in Figure \ref{fig:parallel_example_g}.

\begin{corollary}
By decomposing the path from $s_0$ to $s_m$ into segments, using a logical sequence can achieve optimal performance with polynomially many tunnels in Figure \ref{fig:parallel_example_g}.
\end{corollary}

{\bf Proof.} 
Let $q$ be the logical sequence $s_0,s_1,...,s_m$. And let each link be a tunnel. There are $p+nm$ tunnels in total. Under $n-1$ simultaneous link failures, in the first segment $s_0, s_1$, there will be at least $1 - \frac{n-1}{p}$ capacity available. In all other segments, there will be at least $1$ capacity available. So the logical sequence can carry at least $1 - \frac{n-1}{p}$ traffic, which meets the optimal.
$\square$

\cj{picture needed?}
%In order to prevent tunnel from competing for capacity, we propose to use logical sequences to guide the routing. A logical sequence for a source-destination pair $(s,t)$ is essentially a sequence of nodes which specifies that traffic from $s$ to $t$ can be routed by going through this sequence of nodes. But unlike physical tunnels, each hop in a logical sequence is not supported by a specific link. Instead, it can use tunnels or even other logical sequences to route for one hop. 

%We consider the original network with physical links as a physical network. Then we consider a tunnel from $s$ to $t$ as a virtual link from $s$ to $t$. We consider the network with such virtual links as a virtual network. Then a logical sequence can be seen as a tunnel on the virtual network, except that a logical sequence only provides a guide to route, without dedicating to any physical link or physical tunnel. By doing so, we are providing more flexibility to the routing. We allocate bandwidth to logical sequences as well as physical tunnels so that together they can achieve as good performance as possible.


\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={6.5cm 13.7cm 10.5cm 3cm}, clip, width=0.48\textwidth]{figures/logical_sequence.pdf}
        \label{fig:logical_sequence}

    \caption{An example of a logical sequence and its underlying support.}
        \label{fig:logical_sequence}
\end{figure}

\cj{comment from meeting: Figure~\ref{fig:logical_sequence} may not be needed}

%Figure~\ref{fig:logical_sequence} shows an example of a logical sequence on the network in Figure~\ref{fig:parallel_example}. A logical sequence from $s$ to $t$ consists of two hops $s$ to $u$ and $u$ to $t$. $e_1$ and $e_2$ support the first hop. $e_3$, $e_4$ and $e_5$ support the second hop. Under any single link failure, 1 unit of capacity can be guaranteed in the first hop and $2/3$ unit of capacity can be guaranteed in the second hop. So a maximum of $2/3$ capacity can be guaranteed on this logical sequence under any single link failure. And if we use this logical sequence to route traffic from $s$ to $t$, we can meet the optimal of $2/3$.

Note that in Figure \ref{fig:logical_sequence}, the 5 physical tunnels we are using are different from the original 6 physical tunnels from $s$ to $t$. But the number of tunnels in two schemes are close. If there are more hops between $s$ and $t$ with similar patterns, the number of all tunnels from $s$ to $t$ will grow exponentially while the total number of tunnels between hops will grow only linearly with each tunnel much shorter. In \S\ref{sec:evaluation} we will show that logical sequence works well with just simple heuristics to choose physical tunnels and logical sequences. And routing with logical sequences provides significantly better performance guarantee than routing only through physical tunnels. 

\subsection{Virtual network model}
In order to model bandwidth allocation with logical sequences, we will need to introduce some new notations here. We use $L(s,t)$ to denote the set of logical sequences from $s$ to $t$. For each logical sequence $q$, we use $\tau_q$ to denote the sequence of hops, and each hop is represented as an ordered node pair. Then we can modify \eqref{eq:tp_model} by including the usage of logical sequence as

\begin{align}
\begin{split}
& \max_{z,a,b} \quad \Theta(z) \\
\mbox{s.t.} \quad & 
\sum_{l \in T(s,t)} a_{l}(1 - y_{l}) + \sum_{q \in L(s,t)} b_{q} \\
& \ge \sum_{q: (s,t) \in \tau_{q}} b_{q} + z_{st}d_{st} \quad \forall s,t \in V, \forall y \in Y\\
& a_{l} \ge 0 \quad \forall s,t \in V, l \in T(s,t)\\
& b_{q} \ge 0 \quad \forall s,t \in V, q \in L(s,t)\\
& \sum_{l;\forall s,t \in V, l \in T(s,t)} a_{l} \delta(e \in \tau_{l}^E) \le c_e \quad \forall e \in E\\
\end{split}\label{eq:vn_model}
\end{align}

We call \eqref{eq:vn_model} the virtual network model. We introduce a new variable $b_q$ which represents the amount of reservation we make on the logical sequence $q$. Similar to physical tunnels, we make sure the reservation on the logical sequence should always be non-negative. On the capacity constraint(first constraint), for each node pair $(s,t)$, now we can use both the reservation on physical tunnels($a_l$) and the reservation on logical sequences($b_q$) to route traffic. And if $s-t$ is a segment of a logical sequence, then $s-t$ should also carry traffic for this logical sequence, other than the original demand from $s$ to $t$. Other constraints are exactly the same as in \eqref{eq:vn_model}. Note that in the model, reservation on a physical tunnel is supported by the capacity of underlying physical links. The reservation on a logical sequence is supported by the capacity of both the physical tunnels and logical sequence in the underlying hops. We will show in \S\ref{sec:practical} that a routing scheme with a centralized controller can be easily derived from \eqref{eq:vn_model}'s solution. Furthermore, with additional assumption on the choice of logical sequences, a distributed routing scheme similar to FFC can be easily implemented.

==> yevaluation.tex <==
\section{Evaluations}
\label{sec:evaluation}
\sgr{Experiments: (1) Multi-demand; (2) tunnel sensitivity;
(3) node failure.} \sgr{Too many CDFs.. boring. how to fix? Also, mention a few topology names here and there?} \cj{Should we have case study?}

Our primary evaluation goal is to compare the performance guarantees provided by 
each of the congestion-free mechanisms that we have developed as part of \System{} with \FFC{}, the state-of-the-art congestion-free mechanism. We also compare
\System{} with the performance achieved by the \textbf{optimal} network response
which involves computing the optimal multi-commodity flow for each failure scenario.
Note that while the optimal response allows the network to respond in the most
flexible fashion, analyzing the performance of the scheme across failures is
not tractable~\cite{lancet:sigmetrics18}. In contrast, all congestion-free
mechanisms including \FFC{}, and all of \System{}'s schemes are associated
with tractable models for analyzing performance under failures.

We consider the following schemes associated with \System{}:
%$\bullet$ \textit{FFC.} This refers to using routing flexibility and failure model in FFC~\cite{ffc_sigcomm14}. More accurately, (P) with the failure set modeled as \eqref{eq:ffc_failure}.

$\bullet$ \textit{\FFCimp{}.}
This refers to our scheme (\S\ref{sec:monotonicity}) which has the exact
same mechanism as \FFC{} to respond to failures, while modeling network
structure more explicitly.

%This refers to our model with the same flexibility as FFC while with a better failure model. That is (P) with failure set modeled as \eqref{eq:tunnel_model}.

$\bullet$ \textit{\SysLS{}.} This refers to our approach where \LS{}s are used but not associated with any condition (\S\ref{sec:vs_model}).
For each node pair $(s,t)$, we provide a single \LS{} that includes the set
of nodes in the shortest path from $s$ to $t$. Constructing \LS{}s in this
fashion guarantees that the topological sort assumption is met, which ensures
the scheme can be implemented as a locally proportional routing scheme similar to
\FFC{} (\S\ref{sec:topsortls}).

%This refers to \eqref{eq:vs_model}, our unconditional \LS{} model. For each node pair $(s,t)$, we provide a shortest \LS{}. The segments in the shortest \LS{} form the shortest path for $(s,t)$. This way to construct \LS{}s guarantees that the set of \LS{}s satisfies the topological sort assumption. Thus, it can be practically implemented as a distributed routing scheme.

$\bullet$ \textit{\SysCLS{}.} This refers to our approach where \LS{} are
used but are only activated under certain conditions (\S\ref{sec:ls_with_hint}). \cj{does this imply we only use ls with hints?}
%Here, we provide an unconditional logical sequence for each node pair. Besides, for each node pair who are connected by a direct link, we provide a conditional logical sequence with the hint of this direct link fails. In other words, we provide alternative routes for $(i,j)$ if the link $(i,j)$ is dead. 
We get these logical sequences by solving a restricted form of the logical flow model
where the only conditions considered are no link failures, or single link failures. \sgr{Chuan, please review this for correctness, and edit.} \cj{a point is missing here that the logical sequence we provide is for the failed link.(i-j fails, we have a ls from i to j.)}
and decomposing our results. Constructing \LS{}s in this fashion does not 
satisfy the topological sort assumption. The scheme can be realized by 
solving a linear system of equations on each failure, a much simpler
task than solving an optimization problem such as a multi-commodity flow (\S\ref{sec:Centralized_LS_scheme}). Further, in \S\ref{sec:eval:pruning} we will evaluate a heuristic that derives topologically sorted \LS{}s from an initial set of \LS{} generated in the above fashion.

%This refers to our conditional \LS{} model. That is using \eqref{eq:hint_constraint} as capacity constraint and modeling hints as \eqref{eq:hint_model}. Here, we provide an unconditional logical sequence for each node pair. Besides, for each node pair who are connected by a direct link, we provide a conditional logical sequence with the hint of this direct link fails. In other words, we provide alternative routes for $(i,j)$ if the link $(i,j)$ is dead. We get these logical sequences by solving our logical flow model and decomposing our results. This does not guarantee the set of \LS{}s will satisfy the topological sort assumption. But later we will show a variant which satisfies the assumption. \cj{should I explain more on this?} 

We implement all our optimization models in Python, and use Gurobi 8.0~\cite{gurobi} to solve them. \sgr{Do you mean Python interface of Gurobi? Could you rework?}


\textbf{Topologies.}
We evaluate our models on 21 topologies summarized in Table~\ref{tab:topology} \sgr{Include Table} including two large networks containing more than 100 nodes and 100 edges. We remove one-degree nodes in the topologies recursively so that the networks are not disconnected with any single link failure. We use the gravity model~\cite{gravity_model} to generate traffic matrices with the utilization of the most congested link (MLU) in the range [0.6, 0.63] across the topologies. 




 \begin{figure}[t]
	\centering
      
	    \includegraphics[ trim={0.7cm 0.7cm 0.4cm 0.5cm}, clip, width=0.48\textwidth]{figures/deltacom_monotonicity.pdf}
        \label{fig:deltacom_monotonicity}

    \caption{Demand scale guaranteed by FFC and \FFCimp{} with 2, 3 and 4 tunnels per node pair on Deltacom}
        \label{fig:deltacom_monotonicity}
\end{figure}

  
\subsection{Results}
We report the performance achieved by a scheme when designing for a given set of failure scenarios. 
We start by reporting the demand scale ($z$), which is the factor by which the traffic demand of all pairs can be scaled and yet supported by a given scheme. For example, $z=0.5$ indicates that for all source and destination pairs, half the demand can be served, while $z=2$ indicates twice the demand of all pairs can be handled; Note that $z$ is also the inverse of the MLU, or the utilization of the most congested link. Later in this section, we also report results with the throughput metric.




\textbf{Benefits of modeling network structure.}
We begin by presenting results for Deltacom (the topology with the most nodes), and an
example traffic matrix. Fig.\ref{fig:deltacom_monotonicity} shows the demand scale
guaranteed by \FFC{} and \FFCimp{} when these schemes are designed for all
single link failures. We select physical tunnels so that they are as disjoint as possible, preferring shorter ones when there are multiple choices. With all our topologies including Deltacom, any node pair has at least two disjoint physical tunnels. When three or four tunnels are selected, it is not possible to guarantee that they are disjoint, but our strategy ensures that between all node pairs in the three tunnels case and most node pairs in the four tunnels case, the failure of any link causes at most two tunnels to fail. \cj{Can I desribde as this?} Fig.\ref{fig:deltacom_monotonicity} shows that the performance of \FFC{} does not monotonically grow with the number of tunnels confirming our observations in \S\ref{sec:motivation}. In contrast, \FFCimp{} matches the performance of \FFC{} when 2 tunnels are used, and performs better as more tunnels are added given that it better models network structure. \sgr{If time permits,
add 5/6 tunnels for both.}

We have observed similar results in all our other settings (different topologies,
and across demands).  Fig.\ref{fig:234tunnels} shows FFC's performance with 2, 3 and 4 tunnels across 12 different demands for the Deltacom topology. We can see that using 2 tunnels consistently outperforms using 3 or 4 tunnels. Also, there is a big gap between the optimal and the best of FFC. In the remaining experiments, the various \System{} schemes use 3 tunnels (this is conservative, since adding more tunnels would result in better performance), while our results with \FFC{} involve 2 tunnels (this represents the best setting for \FFC{} and choosing more tunnels leads to poorer performance).

\begin{figure}[t]
	\centering
	    \includegraphics[ trim={0.5cm 0.3cm 0.7cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k1f1_deltacom.png}
        \label{fig:234tunnels}
    \caption{FFC's performance with different number of tunnels per node pair}
        \label{fig:234tunnels}
\end{figure}

\begin{figure}[t]
	\centering
	    \includegraphics[ trim={0.5cm 0.3cm 0.7cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k1f1_deltacom_ffc.png}
        \label{fig:case_study}
    \caption{Multiple demands study on Deltacom}
        \label{fig:case_study}
\end{figure}


\textbf{Benefits of more flexible response.}
Fig.~\ref{fig:case_study} compares the performance of \FFC{} with all our schemes \sgr{too busy?}
across 12 different demands for the Deltacom topology. The figure shows 
the demand scale for different schemes normalized to the demand scale achieved by the optimal approach (a value of $1$ is the maximum and indicates the scheme matches optimal). 
The optimal is obtained by exhaustively enumerating all failure scenarios in the desired set, and running a multi-commodity flow on each scenario. In the median case, \FFC{} achieves a normalized demand scale of only $0.7$, while \FFCimp{} achieves a normalized demand scale of $0.7$ for all topologies. When logical sequences are included which
provides more flexibility of response, the performance is even better -- \SysLS{}
achieves a normalized demand scale of over $0.8$ for all topologies, while
\SysCLS{} does even better and matches optimal for most topologies.







%\textbf{Case study} \sgr{This will be replaced by new graphs.}
%\sgr{Fig.~\ref{fig:case_study} shows the demand scale for different 
%different models. We can see that in $k=1$ case, to guarantee performance under any single link failure, FFC can only scale to less than $0.49$. By simply using a better failure model, \FFCimp{} doubles the scale factor to $0.70$. By providing unconditional \LS{}s, \SysLS{} can again improve to guarantee a scale factor of $0.78$. And \SysCLS{} matches the optimal value of $0.85$. 
%In $k=2$ case, note that FFC can not guarantee any positive scale factor under 3 simultaneous link failures because FFC over-estimates the number of simultaneous tunnel failures. If between a node pair, there are two tunnels sharing a common link, FFC will assume that all $6$ tunnel are dead under 3 link failures. So it will not be able to serve any traffic for this node pair, and the scale factor can only be 0. In fact, this happens for the majority of the node pairs among all topologies. \FFCimp{} clearly can help to solve this issue, and it achieves $0.35$. \SysLS{} can improve over \FFCimp{} to achieve $0.40$. \SysCLS{} again reaches the optimal value of $0.42$. }


 %\begin{figure}[t]
%	\centering
%        
%	    \includegraphics[ trim={0.5cm 0.3cm 0.5cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k1f1_optimal.png}
%        \label{fig:cdf_k1f1}

%    \caption{CDF of demand scale of different schemes across topologies, normalized to the optimal scheme under single failure scenarios.}
%        \label{fig:cdf_k1f1}
%\end{figure}

\begin{figure}[t]
	\centering
        
	    \includegraphics[ trim={0.5cm 0.3cm 0.7cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k1f1_ffc.png}
        \label{fig:cdf_k1f1_ffc}

    \caption{CDF of the demand scale of each scheme relative to FFC ratio on scale factor metric(k=1)\cj{With FFC2, it is not as impressive as before, not sure if we still want to keep it.} \sgr{I dropped one. We can drop this too if space tight. but would be good to have some text.}}
        \label{fig:cdf_k1f1_ffc}
\end{figure}


\textbf{Analysis across multiple topologies.}
Fig.~\ref{fig:cdf_k1f1_ffc} shows the normalized demand scale of the various schemes across
the 21 topologies. The trends are similar. In the median case, \FFC{} achieves a normalized
demand scale of $XX$, while the corresponding values are $XX$ for \FFCimp{} and \SysLS{}.
\SysCLS{} achieves the optimal for $80\%$ of the cases. 
\sgr{Chuan, please fill and check the numbers.} 

%All our schemes significantly bridge the gap, with \SysCLS{} matching the optimal for more than 70\% of cases. 

%Next, we show the comparison between each scheme and optimal value. We get FFC versus optimal ratio, and each our scheme versus optimal ratio, then plot cdf for each of them. Fig.~\ref{fig:cdf_k1f1} shows the cdf graph for $k=1$ case. We can see that there is a big gap between FFC and optimal. Even in the best case, FFC can only guarantee about 65\% of the optimal scale factor. 

To more directly compare the benefits over \FFC{} for each topology, we consider the ratio of the demand scale for a given scheme to the demand scale with \FFC{} for each topology. Fig.~\ref{fig:cdf_k1f1_ffc} presents a CDF of the ratios for each scheme across topologies. 
All our schemes provide significant benefits - further there are topologies for which both 
\SysLS{} and \SysCLS{} provides a 2.6X higher scale factor. \sgr{Please check numbers. Which topology gives the highest?}

%All our schemes provide significant benefits. \FFCimp{} performs a factor of $1.25$ to a factor of $2$ \sgr{Check numbers} better than \FFC{}. While \SysLS{} provides some additional benefit for many topologies, the benefits are particularly strong for the last 20\% of the topologies,
%and it provides a 4X benefit over \FFC{} in one case. Finally, \SysCLS{} provides
%even greater benefits. \sgr{Which topology does LS provide so much benefit?}
%\sgr{I am OK dropping the optimal curve here if you prefer this.}

%We can see that all of our schemes improve 50\% over FFC among more than 70\% of topologies. And using \LS{}s can get huge improvements which can even guarantee to scale 4 times what FFC can provide. \sgr{Anything interesting.. which topology?}
 
%\begin{figure}[t]
%	\centering
%	    \includegraphics[ trim={0.5cm 0.3cm 0.7cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k2f3_ffc.png}
%        \label{fig:cdf_k2f3_ffc}

%    \caption{CDF of the demand scale of each scheme relative to FFC ratio on scale factor metric(k=2)\cj{new graph, same issue as in the previous graph}}
%        \label{fig:cdf_k2f3_ffc}
%\end{figure}

  

%\begin{figure}[t]
%\centering
        
%	\includegraphics[ trim={0.5cm 0.3cm 0.5cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k2f3_optimal.png}
%    \label{fig:cdf_k2f3}

%    \caption{cdf of scheme/optimal ratio on scale factor metric(k=2)}
%    \label{fig:cdf_k2f3}
%\end{figure}


\textbf{Multiple simultaneous failures.}
We next evaluate the performance of the schemes under simultaneous link failures. Since this could result in the topology getting disconnected, we split the capacity of each link evenly across two sub-links that fail independently. We report the performance of all schemes when designing for all possible scenarios involving the simultaneous failure of three links. For all schemes we pick 6 tunnels, choosing them to be as disjoint as possible. For similar reasons as above, we found \FFC{} achieved significantly better performance with 4 tunnels (in fact \FFC{} resulted in a scale
factor of 0 with 6 tunnels). \footnote{With 6 tunnels, not all could be disjoint and two 
shared a common link. Under three failures, \FFC{} would need to provision for the case all tunnels failed.} Fig.~\ref{fig:cdf_k2f3} shows the normalized demand scale. The trends are very similar to 
the single failure case. Note that though the normalized values under 3 failures is similar to
single failure, the absolute values were significantly lower -- for e.g., for Deltacom, the
optimal under 3 failures is $XX$, while under single failure $XX$. \sgr{Chuan please fill/correct}.


%We use $k=1$ to denote cases without splitting capacity and use $k=2$ to denote cases with splitting link capacity. And For $k=2$ cases, we select 6 physical tunnels.

%Across all topologies, any node pair has at least 2 disjoint physical tunnels in $k=1$ case and at least 4 disjoint physical tunnels in $k=2$ case. \sgr{Sensitivity to tunneling result - oblivious?}




 \begin{figure}[t]
	\centering
        
	    \includegraphics[ trim={0.5cm 0.3cm 0.5cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k2f3_tp_lossreduction.png}
        \label{fig:cdf_k2f3_tp}

    \caption{CDF of reduction in loss ratio of each scheme comparing to FFC(k=2)\cj{is the benefit insignificant?}}
        \label{fig:cdf_k2f3_tp}
\end{figure}

\textbf{Throughput metric.} 
While we have focused so far on the demand scale metric, we next report results for the various schemes when optimizing for the throughput metric, which is the sum of the traffic assigned to each pair (here the demand is not scaled, and different fractions of each pair's demand may be served).
Fig.\ref{fig:cdf_k2f3_tp} shows the throughput of each scheme relative to \FFC{}. \FFCimp{}
and \SysLS{} give noticeable improvement over \FFC{}, achieving an increase in throughput of 
$20\%$ relative to \FFC{} for $10\%$ and $20\%$ of the topologies. \cj{this doesn't look nice.. Other numbers are $15\%$ improvement with $20\%$,$38\%$ of topologies, and $10\%$ improvement with $66\%$,$50\%$ of topologies.}
The benefits are even stronger with \SysCLS{} with more than $50\%$ of the topologies providing
an increase in throughput of more than $23\%$.
\sgr{Is the f=1 case worse? Also, what if we do more tunnels for \FFCimp{} and \SysLS{}}?

%Besides maximum traffic scale factor, we also evaluate our schemes using throughput as our metric. We compare the throughput guarantee achieved by different schemes with the total demand, and compute the loss percentage.  Fig.~\ref{fig:cdf_k2f3_tp} shows different schemes' cdf of loss percentage for $k=2$.  We can see that FFC loses more than 40\% demand among all topologies, and in more than 80\% of all topologies, FFC will lose more than 70\% demand. In some cases, it even loses almost all demand. \FFCimp{} and \SysLS{}, however, can guarantee to serve around 60\% of demand in more than 80\% of topologies. Even in the worst case, they can serve around half of the demand. \SysCLS{} further improves to guarantee 75\% demand in more than 80\% of topologies and 60\% demand in the worst case.

%In summary, our schemes significantly improve over FFC in all topologies for both the scale factor and throughput metrics. For the scale factor metric, \SysCLS{} even matches the optimal in most of the cases.

  

%   \begin{figure}[t]
%	\centering
%        
%	    \includegraphics[ trim={1.5cm 0.6cm 0.8cm 0.8cm}, clip, width=0.48\textwidth]{figures/case_study.pdf}
%        \label{fig:case_study}
%
%    \caption{Case study of Deltacom}
%        \label{fig:case_study}
%\end{figure}
 
 
   
 %\begin{figure}[t]
% \centering
%      
%	    \includegraphics[ trim={0.5cm 0.3cm 0.5cm 0.5cm}, clip, width=0.48\textwidth]{figures/cdf_k1f1_prune.png}
%        \label{fig:prune}
%    \caption{cdf of \SysPrune{}/optimal ratio on throughput metric(k=1)\cj{same line as \SysCLS{} in figure 12}}
%        \label{fig:prune}
%\end{figure}

  
 
 \textbf{Alternate tunnel selection.}
 Try oblivious with Deltacom, show what happens? We might move it earlier
 along with changing number of tunnels.
 
\subsection{Feasibility of local yet optimal routing}
\label{sec:eval:pruning}
As discussed earlier, \FFCimp{} uses a routing mechanism identical to \FFC{}, while \SysLS{} uses topologically sorted logical sequences and can be realized using a locally proportional routing (\S\ref{sec:topsortls}) similar to
\FFC{}. However, the \LS{}s chosen in \SysCLS{} are not explicitly guaranteed to be topologically sorted by default. 

We consider a new scheme, which we refer to as \SysPrune{}, that starts with the \LS{}s initially generated by \SysCLS{}, and picks a subset which are topologically sorted. To achieve this, we use a simple greedy algorithm that adds \LS{}s one by one from the original set, omitting any sequence that violates the topological sort property. Note that \SysCLS{} uses a \LS{} per
node pair at all times, and an \LS{} that is only activated when a link fails (with a different \LS{} activated on each link failure). It suffices to ensure the topological sort property is maintained across all the \LS{}s active in any given failure scenario.

Interestingly, when single link failures are considered, we
found the sequences generated by \SysCLS{} are already topologically sorted by default for 16 of our 21 topologies. 
For the remaining 5 topologies, we applied the \SysPrune{}
strategy. In all cases, the number of pruned \LS{}s was fairly small -- e.g., Deltacom required the most pruning with 55
sequences out of a total of 51811 pruned. Further, for 4 of the 5 topologies, \SysPrune{} performs identically with \SysCLS{}
for the demand scale metric - for Ion alone there was a modest performance degradation (from a demand scale of $XX$ with \SysCLS{} to $XX$ with \SysLS{}).

This result is significant because it indicates that for single failure scenarios, a local proportional routing mechanism is
sufficient to ensure optimal performance for $XX$ topologies
(and near optimal for $XX$ topologies). For 3 failure scenarios, the \SysPrune{} strategy has more significant degradation than \SysCLS{} (and performs comparably to \SysLS{}). This is still useful because (i) \SysPrune{} and \SysLS{} significantly out-perform \FFC{} and are realizable as local algorithms;
and (ii) while \SysCLS{} nearly matches optimal, it only requires that a linear system of equations is solved on
each failure as opposed to the optimal which requires that 
an optimization problem is solved. \sgr{Talk about distributing linear systems, better optimizing pruning etc.}

%Fig.~\ref{fig:prune} shows the cdf of the ratio of \SysPrune{} versus optimal traffic scale factor for $k=2$ case. We can see that \SysPrune{}'s performance is close to the optimal, which means that pruning doesn't impare the performance in these scenarios.
 
%\begin{figure}[t]
%\centering
%    \includegraphics[ trim={1cm 1.3cm 0.1cm 0.7cm}, clip, width=0.48\textwidth]{figures/solving_time_k1.pdf}
%    \label{fig:time_k1}

%    \caption{Solving time for $k=1$.}
%    \label{fig:time_k1}
%\end{figure}

 
    \begin{figure}[t]
	\centering
        
	    \includegraphics[ trim={1cm 1.3cm 0.1cm 0.7cm}, clip, width=0.48\textwidth]{figures/solving_time_k2.pdf}
        \label{fig:time_k2}

    \caption{Solving time for $k=2$. \cj{only show \SysCLS{}} \sgr{k=2 or k=1?} \sgr{Show PCF-TF too?}}
            \label{fig:time_k2}
\end{figure}

\subsection{Tractability of formulations}
We next consider the tractability of our formulations by considering the solving time
for our schemes. Fig.~\ref{fig:time_k2} shows a scatter plot with each point corresponding
to a topology. The X-Axis is the number of sub-links in the topology, and the Y-Axis is 
the solving time when \SysCLS{} is used to design for all simultaneous three link
failure scenarios. Note that the solving time for all other schemes is lower.
For most topologies, the solving times is under $10$ seconds \sgr{Chuan: please check}.
For the two largest networks (Deltacom and Ion) with 250-300 links, the solving
time is under $100$ seconds. Note that for these topologies, determining the optimal
by exhaustively enumerating all scenarios took 1.5-2 days. \sgr{Why are we so much higher than FFC?}

This is reasonable because our formulation only need to be run offline at the granularity 
of tens of minutes, when recomputing reservations as traffic demands shift. Note that 
the online operations that must take place on any failure does not involve solving
an optimization problem (\SysCLS{} solves a linear system, while the other schemes
do a completely local proportional scheme).

Another benefit of our formulations is they can enable a network architect to appropriately
provision the capacity of the network, by deciding how best to augment link capacities
to ensure the network can handle desired failures. Solving such problems with the optimal
scheme is challenging since this would require exhaustively enumerating topologies with
different capacity assignments, as well as enumerating all failure scenarios for each
candidate topology, and is often done today through an ad-hoc mix of simulations and optimization
~\cite{ciscoWAE,googlesimulator}.



%And even the two large network with more than 100 edges for $k=1$ and more than 250 edges for $k=2$ can be solved within 2 minutes.

%Next, we will show that the solving time for our models is insignificant. So it will not create much delay when the routing needs to be updated. Fig.~\ref{fig:time_k1} and Fig.~\ref{fig:time_k2} show the scatter plots of solving time versus number of edges in the topology. We can see that for most of the topologies, the solving times for \SysLS{} and \SysCLS{} are negligible. And even the two large network with more than 100 edges for $k=1$ and more than 250 edges for $k=2$ can be solved within 2 minutes.
 
% Deltacom: MCF can take 2-3 days for our large topologies.
 

==> zdesign.tex <==
\section{Design}
In this section, we will illustrate the details of \vn{} model. We start by giving the insight of the deficiencies of \rthree{} and \FFC{}(\S\ref{sec:insight}). By explaining the solutions to improve  \rthree{} and \FFC{}, we introduce the key ides of our \vn{} model and the challenges to make it feasible. We then explain \vn{} design in the formal formulation.

\subsection{Insight of \rthree{} and \FFC{}}\label{sec:insight}
From \S\ref{sec:analysisr3} and \S\ref{sec:analysisffc}, we already see examples where \rthree{} and \FFC{} are giving undesirable performance. \rthree{} computes its routing on physical links, and its recovery mechanism is also built to construct bypass for each link. Hence, when a link fails, it can only reroute the traffic on the failed link, without making changes on other part of the flow. This puts a big constraint on the routing flexibility, and is also root cause of why \rthree{} model can not be extended to handle node failures.

\FFC{} routes on the given tunnels. Unlike \rthree{}, its recovery mechanism operates in a more global manner where it abandons the tunnels containing the failed links, and move the flow to the working tunnels. This prevents the \rthree{}'s constraint on routing flexibility. However, \FFC{} can only route traffic on the given tunnels, which is much less flexible than link-based routing.

\subsection{Virtual links and virtual network}\label{sec:vnlink}

Given a network topology and traffic demand $d_{st}$ for all source destination pairs, the problem we want to solve is to design a routing to serve the demand which is congestion free under $f$ simultaneous link failures. We are given the set of edges $E$, and $\forall e \in E$, $c_e$ representing the capacity of the edge $e$. We are also given the tunnels in the network, and $L(i,j)$ representing all the tunnels we can use from source $i$ to destination $j$. We need to design formulation to solve for a set of variables to describe the routing in terms of the amount of traffic going through the given edges or the given tunnels, and to describe how the routing will be changed upon failures. 

In order to improve \rthree{} and \FFC{}, a natural way to think is to combine their advantages together, which is to build a link-based routing that is able to do tunnel bypass upon link failures. 

Though these properties describe a more flexible routing, it is not intuitive to develop a model to capture them. However, the model becomes more achievable if we think of a virtual network. Two nodes are connected as long as there is a physical link between them or a tunnel connecting them. So a virtual link can be composed by a physical link and multiple tunnels. Now if we compute a routing on the virtual network, both physical links and tunnels will be used. And if we design bypass routing on it,  both physical links and tunnels may be bypassed. Then we will have a model which has the flexibility both to route on physical links and to bypass tunnels.

Our \vn{} model is mainly built on this idea that we can introduce virtual links to construct a virtual network and route on it. This will provide richer adaptation than both \rthree{} and \FFC{} as explained above. Though the idea seems straight-forward, we still need to address several challenges when bringing in the virtual links.

\textbf{Failure on tunnels.} We need to model tunnel failures since the failure scenarios are given in the form of link failures. For a tunnel, any failure on the underlying physical links will cause it to fail. \FFC{} provides a way to model tunnel failures by pre-computing the maximum number of simultaneous tunnel failures. This modeling doesn't describe the connection between physical links and tunnels well enough, hence can give quite conservative results.

\textbf{Capacity of virtual links.} For physical links, we are given the link capacity. For virtual links, however, the capacity is unknown. They are built upon physical links and tunnels, and different virtual links may share underlying physical links. How to plan the capacity is crucial to the performance. Note that in the virtual network, routing is link-based. And each virtual link can use physical link or tunnels. So when it converts to a practical routing, not only physical links are sending the traffic as in \rthree{}, tunnels are also routing the traffic as in \FFC{}, which makes the capacity planning even more complicated. We need to come up with a capacity planning which can always satisfy the physical capacity constraint while can also flexibly adapt to the failures.

\textbf{Converting to practical routing.}
One of the advantages of \rthree{} and \FFC{} is that they can adapt to changes on the network quickly. Using the offline-computed bypass, they are able to reroute traffic upon failures. In order to make \vn{} practical, we also need to design an update scheme to instantly respond to the failures and update the routing.

% \begin{itemize}
%     \item R3 operates on physical; FFC could be viewed as a virtual (explain).
%     \item R3 supports a link-based recovery mechanism. The straight-forward FFC does not support on the virtual
%     \item Key idea: Have a virtual network abstraction, and provide link-based recovery on top. More flexible than FFC because it has the richer adaptation on the virtual network. More flexible than R3 because it operates on the virtual, not just the physical. In addition, create a better model of path with FFC to better model disjointness issues.
% \end{itemize}


%\subsection{Main Ideas}

%\begin{itemize}
%    \item Difference from R3: Concept of virtual link. Link is not physical link, can also be tunnel. Allow link-based protection on the virtual network.
%    Can use tunnel to protect a link.
%    \item Difference from FFC: treat the link as a tunnel, and can do link-based
%           routing and link-based protection. 
%    \item Diffrence from FFC: explicilty modeling relation paths between links.
%         FFC-improved aspects.
%\end{itemize}



% 1) FFC-improved

% 2) R3 and improve. Bring in virtual networks
%   Breaks the R3 structure. R3 would like to plan
%   when this network dies

%   R3 on a virtual network.
%   Bypass for every tunnel dying. Clique. Protection for
% 	every node pair. Too expensive.
%   Keep it for actual link dying to keep it under control.
%   Tunnel depends on every underlying link.
%     Bypass for each link dying.. MCF not a s-d pair,
% 	many tunnels going on, one for each tunnel

%     How do we create virtual network from physical network?

% 	Add virtual links by drawing capacity from physical links
% 	to virtual links.

% 	We are assuming given virtual links and how they map to the
% 	physical network.

% 	Determine the capacity for each virtual link

% 	Need not create a bypass for link $c_{ij}$ fully. Bypass all the
% 	traffic it can get upto k-1 failures

% 	Combine all the virtual links for the same <i,j>
% 	  Separate constraints: 

% 	Not requiring each to be under $c_e$


% In a 2-failure problem, sum of any 2 of $a_{el}$ may be less than $a_{0l}$


% 	Bypass for each edge.


%       Capacity reservations on the tunnel


%   Source of link rerouting to the destination
%   Rerouting tunnel source
% 	Tunnel: structure available: capacities have to be determined
% 	so they are optimally chosen.




%   Between nodes i and j, many paths from i to j, some being tunnels,
%   some being arcs. Constraints no longer on link basis, but on node
%   pairs.





% Flexibility:

% --Do link and tunnel bypass both

% --Use a tunnel to handle a tunnel

% —




% Formulation



% Advantages on some examoles

\begin{table}[t]
\centering
 \begin{tabular}{||c c||} 
 \hline
 Name & Definition \\ [0.5ex] 
 \hline\hline
 $E$ & Set of all edges. \\
 \hline
 $E_{core}$ & Set of edges in the core network. \\
 \hline
  $N_{core}$ & Set of nodes in the core network. \\
 \hline
   $N_{edge}$ & Set of edge nodes. \\
 \hline
 $L(i,j)$ & Set of tunnels going from node $i$ to node $j$. \\
 & This set also includes the physical link (i,j)\\
 \hline
  $T(i,j)$ & Set of tunnels traversing link (i,j) \\
 \hline
 $x_e$ & Variable indicating if link $e$ fails\\ 
 \hline
 $y_l$ & Variable indicating if tunnel $l$ fails. \\
 & Tunnel $l$ fails when any link in $l$ fails.\\ 
 \hline
  $a_{0l}$ & Reserved capacity on tunnel $l$ when $l$ doesn't fail \\
  \hline
  $a_{el}$ & Reserved capacity on tunnel $l$ when link $e$ fails \\
  \hline
  $P_{eijt}$ & Protection routing on virtual link $(i,j)$ to destination $t$ \\
  & when link $e$ fails \\
  \hline
  $r_{ijt}$ & regular flow on virtual link $(i,j)$ to destination $t$ \\
  \hline
 \end{tabular}
\caption{Symbol definition}
\end{table}

\subsection{Model tunnel failures}\label{sec:vnmodel}


Compare to \FFC{}, we use a more accurate way to model tunnel failures and draw the connection between link failures and tunnel failures directly. Suppose $x_e$ is the variable indicating if link $e$ fails, we model $y_l$ by 

\begin{align}
\begin{split}
& \sum_{e \in E} x_e \le f \\
& x_e - y_l \le 0 \quad \forall l, e \in l \\
& y_l - \sum_{e \in l} x_e \le 0 \quad \forall l  \\
\end{split}\label{eq:tunnel_model}
\end{align}

The first constraint bounds the maximum number of simultaneous link failures. The second ensures that any failed underlying link of a tunnel will cause the tunnel to fail. The third ensures that a tunnel only fails when at least one underlying link fails. This set of constraints equations depict the exact connection between link failures and tunnel failures, thus it will eliminate the gap caused by conservative estimation of tunnel failures in \FFC{}. Note that we can easily add node failures into this following the same idea. But we only focus on link failures in this work.

We will show in \S\ref{sec:evaluation} that the tunnel-based routing scheme in \FFC{} can achieve better performance by improving the tunnel failure modeling as above. But even if we improve \FFC{} by adopting this better way to model tunnel failures, it still can only send traffic on the provided tunnels and doesn't have the flexibility to freely exploit the topology as in \rthree{}. \vn{}, however, allows link-based routing. Thus, it can provide much more flexibility.

\subsection{Virtual link capacity}\label{sec:vncapacity}

\begin{figure*}
\begin{minipage}[t]{0.45\textwidth}
    \includegraphics[trim={0 0.5cm 0cm 0cm}, clip, width=0.95\textwidth]{figures/vn_example.png}
    \captionof{figure}{A 4-node network with 2 tunnels and its corresponding virtual network.} \label{fig:vn_example}
\end{minipage}\hspace{0.1in}
%
\begin{minipage}[t]{0.22\textwidth}
    \includegraphics[trim={0 0cm 0cm 0cm}, clip, width=\textwidth]{figures/normal.png}
    %\vspace{-0.1in}
    % \captionof{figure}{Worst-case design effectiveness with GEANT $k = 2$.}
    \captionof{figure}{Usable capacity under no failure.}
    \label{fig:vn_normal}
\end{minipage}
%
\begin{minipage}[t]{0.224\textwidth}
    \includegraphics[trim={0 0cm 0cm 0cm}, clip, width=\textwidth]{figures/fail.png}
    %\vspace{-0.1in}
    % \captionof{figure}{Worst-case design effectiveness with GEANT $k = 2$.}
    \captionof{figure}{Usable capacity with one link failing.}
    \label{fig:vn_fail}
\end{minipage}
\end{figure*}

Besides modeling tunnel failure, the other challenge in designing the model is to plan the virtual link capacity. In order to give \vn{} more flexibility, we plan the tunnel capacity both when the tunnel is alive and when the tunnel is dead. We use $a_{0l}$ to represent tunnel $l$'s capacity we reserve when $l$ is alive. To support $a_{0l}$, all underlying links in tunnel $l$ will need to carry $a_{0l}$ amount of traffic if $l$ is alive.

If $l$ fails, we know that some underlying link $e$ must fail and cause $l$ to fail. So we reserve $a_{el}$ capacity upon $e$'s failure for $l$ to use. $a_{el}$ will be built through other paths from source of $l$ to the destination of $l$. Note that this idea is similar as the link protection in \rthree{} which uses reserved paths to bypass a failed link. But here, we can even bypass a tunnel(a list of links), which handles the major defects in \rthree{}. For convenience and consistency, we also treat a single physical link as a tunnel.

Figure~\ref{fig:vn_example}-Figure~\ref{fig:vn_fail} shows an example of virtual network. ~\ref{fig:vn_example} shows a simple 4-node network and its corresponding virtual network. The network contain 4 physical links and 2 tunnels. Note that in the virtual network, there is a virtual link whenever there is a physical link. Besides, there is a virtual link between $s$ and $t$ because they are connected by tunnels. Figure~\ref{fig:vn_normal} shows the usable capacity when there is no failure on the network. Virtual link $\langle s, t \rangle$ can use the reserved capacity $a_{0l_1}$ and $a_{0l_2}$. Other links can use the physical capacity on themselves. Figure~\ref{fig:vn_fail} shows the usable capacity when there $e_1$ fails. Since $e_1$ fails, its capacity can not be used, and tunnel $l_1$ is also broken. But we can use the bypass for $e_1$ and $l_1$ when $e_1$ fails, i.e. $a_{e_1e_1}$ and $a_{e_1l_1}$. An important thing to notice here is that, except physical capacity $c_e$, we need to 'pay' for other usable capacity. For example, in order to reserve $a_{0l_1}$, we need to add load on $\langle s, 1\rangle$ and $\langel 1, t\rangle$. In order to reserve bypass $a_{e_1e_1}$ or $a_{e_1l_1}$, we need to add load on alternative paths when $e_1$ fails. We use an optimization model to plan this reservation.



\subsection{\vn{} model}\label{sec:vnmodel}

Suppose $r_{ijt}$ represents the flow on virtual link $\langle i, j \rangle$ to destination $t$. Our \vn{} model to handle MLU problem can be abstracted as

\begin{align}
\begin{split}
& \min \quad U \\
\mbox{s.t.} \quad & a) r_{ijt} \text{ builds the flow to serve demand } d_{st} \\
& b) \text{For any failure scenario, } r_{ijt} \text{ will not exceed the usable} \\
& \text{virtual capacity composed by } a_{0l}, a_{el} \text{ and } Uc_{\langle i,j \rangle} \\
& c) a_{0l} \text{ and } a_{el} \text{ can be reserved without exceeding capacity}
\end{split}
\end{align}

a) is a simple flow balance constraint which we can write as 

\begin{align}
\begin{split}
& \sum_{j}  r_{ijt} - \sum_{j}  r_{jit} = 
\begin{cases}
d_{it} & i \ne t\\
-\sum_{j}d_{jt} & i = t\\
\end{cases} 
\end{split}
\end{align}

b) and c) define the flexibility of \vn{} and how the routing is decided. We first build the paths for $a_{el}$, i.e. the reserved bypass for tunnel $l$. As mentioned in \S\ref{sec:vncapacity}, this is similar as building the protection for failed link in \rthree{}. We use $P_{eijt}$ to represent the extra load on link $\langle i,j \rangle$ to destination $t$ when link $e$ fails. Then, $P_{eijt}$ should build the flow to serve $a_{el}$, i.e.

\begin{align}
\begin{split}
& \sum_{j} P_{eijt} - \sum_{j}  P_{ejit} = 
\begin{cases}
\sum_{l \in L(i,t)} a_{el}  \quad \forall i \ne t, e \\
-\sum_{j} \sum_{l \in L(j,t)} a_{el}  \quad \forall i=t, e
\end{cases} 
\end{split}
\end{align}

Now, for any virtual link $\langle i,j \rangle$, we calculate the total usage on it and the total usable capacity. First, from b), we have $\sum_{t} r_{ijt}$ traffic to route in order to serve the demand. And for tunnels between $(i,j)$, we have total virtual capacity of $ \sum_{l \in L(i,j)} a_{0l}(1-y_l) + \sum_{e \in E \atop l \in L(i,j)} x_e a_{el}$ depending on the failure scenario.

From c), we know that $\langle i,j \rangle$ will also be needed to reserve the tunnel capacity $a_{0l}$ and  bypass $a_{el}$. So it also uses $\sum_{t,e \in E} x_e P_{eijt}$ to build bypass and $\sum_{l \in T(i,j)}a_{0l}(1-y_l)$ to reserve the capacity of tunnels upon it. Note that if $\langle i,j \rangle$ also contains a physical link, then the physical capacity $U c_{\langle i,j \rangle}$ is also usable.

Combine all the usage and usable capacity, we can write the capacity constraint for virtual links as

\begin{align}
\begin{split}
& \sum_{t} r_{ijt} + \sum_{t,e \in E} x_e P_{eijt} + \sum_{l \in T(i,j)}a_{0l}(1-y_l) \\
& \le U c_{\langle i,j \rangle} (1-x_{\langle i,j \rangle}) + \sum_{l \in L(i,j)} a_{0l}(1-y_l) + \sum_{e \in E \atop l \in L(i,j)} x_e a_{el}
\end{split}
\end{align}

And we can write the full \vn{} model as

\begin{align}
\begin{split}
& \min \quad U \\
\mbox{s.t.} \quad & \sum_{t} r_{ijt} + \sum_{t,e \in E_{core}} x_e P_{eijt} + \sum_{l \in T(i,j)}a_{0l}(1-y_l) \\
& \le U c_{\langle i,j \rangle} (1-x_{\langle i,j \rangle}) + \sum_{l \in L(i,j)} a_{0l}(1-y_l) + \sum_{e \in E \atop l \in L(i,j)} x_e a_{el} \\
& \quad \quad \quad \quad \quad\quad\quad\quad\quad\quad\quad\quad\quad\forall x,y \in X(f), \forall i,j \\
& \sum_{j}  r_{ijt} - \sum_{j}  r_{jit} = 
\begin{cases}
d_{it} & i \ne t\\
-\sum_{j}d_{jt} & i = t\\
\end{cases} \\
& \sum_{j} P_{eijt} - \sum_{j}  P_{ejit} = 
\begin{cases}
\sum_{l \in L(i,t)} a_{el}  \quad \forall i \ne t, e \\
-\sum_{j} \sum_{l \in L(j,t)} a_{el}  \quad \forall i=t, e
\end{cases} \\
& r_{ijt} \ge 0 \quad \forall i,j,t\\
& a_{el} \ge 0 \quad \forall e\in l\\
& a_{0l} \ge 0 \quad \forall l
\end{split}\label{eq:vnmodel}
\end{align}

The last three constraints make sure that the virtual link capacity is positive and the traffic is non-negative. $X(f)$ defines the set of all link failure scenarios and the resulting tunnel failures, which can be described in \eqref{eq:tunnel_model}. $r$, $P$, $a_{0l}$ and $a_{el}$ describe the routing achieved by this model.

\eqref{eq:vnmodel} describes the general \vn{} model. It can be easily turned into an edge-core network model. In the edge-core network, nodes are classified into two sets, edge nodes and core nodes. In our edge-core network model, we only allow traffic demand between edge nodes and edge nodes. And we don't allow any edge node to serve as an intermediate point to route traffic to other edge nodes. So we add two constraints to ensure this,

\begin{align}
\begin{split}
& r_{ijt} = 0 \quad \forall j \in N_{edge}, j\ne t\\
& p_{eijt} = 0 \quad \forall j \in N_{edge}, j\ne t, e\\
\end{split}
\end{align}

Sometimes we only model link failure between core nodes and core nodes in edge-core model. This can be easily achieved by adding $\forall e \in E_{edge}:x_e=0$ to the $X(f)$ definition.


% \begin{align}
% \begin{split}
% & \min \quad U \\
% \mbox{s.t.} \quad & \sum_{t} r_{ijt} + \sum_{t,e \in E_{core}} x_e P_{eijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & \le U c_{\langle i,j \rangle} (1-x_{\langle i,j \rangle}) + \sum_{l \in L(i,j)} (a_{0l}\prod_{e \in l\cap E_{core}}(1-x_e)) + \sum_{e \in E_{core} \atop l \in L(i,j)} x_e a_{el}
% \quad \forall x \in X, \forall i,j \\
% & r_{ijt} \ge 0 \quad \forall i,j,t\\
% & r_{ijt} = 0 \quad \forall j \in N_{edge}, j\ne t\\
% & p_{eijt} = 0 \quad \forall j \in N_{edge}, j\ne t, e\\
% & a_{el} \ge 0 \quad \forall e,l\\
% & a_{el} = 0 \quad \forall e \notin l\\
% & a_{0l} \ge 0 \quad \forall l\\
% & \sum_{j}  r_{ijt} - \sum_{j}  r_{jit} = 
% \begin{cases}
% d_{it} & i \ne t\\
% -\sum_{j}d_{jt} & i = t\\
% \end{cases} \\
% & \sum_{j} P_{eijt} - \sum_{j}  P_{ejit} = 
% \begin{cases}
% \sum_{l \in L(i,t)} a_{el}  \quad \forall i \ne t, e \\
% -\sum_{j} \sum_{l \in L(j,t)} a_{el}  \quad \forall i=t, e
% \end{cases} 
% \end{split}
% \end{align}

% \textbf{Notes}
% \begin{itemize}
%     \item Add $c_{ij}$ = 0 unless physical link
% \end{itemize}


% \textbf{Assumptions:}
% \begin{itemize}
%     \item Tunnels exist only if both end points are edge nodes
%     \item Edge node $i$ cannot send traffic to an edge node $k$ through another edge node $j$
%     \item only core links fail [may be important for final compensation. currently may be assuming that no tunnels to failed link end in tail of failed link.]
%     \item [TODO: Check if we need assumption] Traffic is only between edge nodes.
% \end{itemize}

% \textbf{Intuition.}

% \begin{itemize}
% \item Think of an R3 and an FFC network. We can decide how much goes on R3 and how much goes
% on FFC. But if a link fails, we can revisit the split (i.e., not only can we change within
% R3 and FFC, but we can change how much goes on the R3 portion, and how much on the FFC portion).
% \item $f_{ij}$ is how much is carried on FFC (across all the FFC tunnels).
% \item $a_{\epsilon,l}$ can be interpreted as how much carried on one of the FFC tunnels $l$ is redirected to the R3 network on failure of $\epsilon$
% \item $\tilde{r}_{ijt}$ reflects the increased load on the R3 network accounting
% for traffic moved from FFC.
% \item $r'_{ijt}$ reflects further adjustments within R3 network to avoid traffic on
%     $\epsilon$.
% \item $p_{eijt}$ is non-zero only if $<i,j>$ is a physical link. That is, if $e$ fails,
% traffic can only be redirected on physical links, not on tunnels. That is, it stays
% within R3. \textbf{Needs to be proven.}
% \end{itemize}

\subsection{Extract routing from edge-core model}

Assume in the edge-core network, we only build tunnels between two different edge nodes and there are no physical links between two edge nodes. For any two nodes, either there are tunnels between them while no physical links, or there is an physical link between them while no tunnels. If $i$ and $j$ are two different edge nodes, $r_{ijt}$ is only meaningful when $j=t$, because tunnels between $i$ and $j$ will only carry traffic from source $i$ to destination $j$. For convenience, we use $f_{ij}$ to replace $r_{ijj}$ when $i$ and $j$ are edge nodes. Now the capacity constraint can be written for two different types of links.

For an phycial link $\langle i,j\rangle$, i.e. $\exists e' \in E, e'=\langle i,j\rangle$:

\begin{align}
\begin{split}
& \sum_{t} r_{ijt} + \sum_{t,e \in E_{core}} x_e P_{eijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
& \le U c_{\langle i,j \rangle} (1-x_{\langle i,j \rangle}) + x_{\langle i,j \rangle} a_{\langle i,j \rangle \langle i,j \rangle}
\quad \forall x \in X 
\end{split}\label{eq:capa_act}
\end{align}

For virtual links between edge nodes, i.e. $\forall e' \in E, e' \ne \langle i,j\rangle$:

\begin{align}
\begin{split}
& f_{ij} \le \sum_{l \in L(i,j)} (a_{0l}\prod_{e \in l\cap E_{core}}(1-x_e)) + \sum_{e \in E_{core} \atop l \in L(i,j)} x_e a_{el} \quad \forall x \in X 
\end{split}\label{eq:capa_vir}
\end{align}

Now, $r_{ijt}$ represents the real routed traffic on physical link $\langle i,j\rangle$ in addition to the flow on any tunnel through $\langle i,j\rangle$. The demand $d_{it}$ can be split into two parts $\Bar{d}_{it}$ and $f_{it}$. $\Bar{d}_{it}$ is the part routed by physical links as in R3. $f_{it}$ is the traffic sent through tunnels from $i$ to $t$. Flow balance constraint can be rewritten as 

\begin{align}
\begin{split}
& \sum_{j}  r_{ijt} - \sum_{j}  r_{jit} = 
\begin{cases}
\Bar{d}_{it} & i \ne t\\
-\sum_{j}\Bar{d}_{jt} & i = t\\
\end{cases} \\
& \Bar{d}_{it} + f_{it} = d_{it} \quad \forall i, t \in N_{edge}
\end{split}\label{eq:flow_balance_}
\end{align}

When there is no failure on the topology, $r$ is the routing variable which describes a link-based routing, and it will carry $\Bar{d}_{it}$ as in R3. $f_{it}$ describes the traffic routed through tunnels from $i$ to $t$, and it can be proportionally assigned

\begin{align}
\begin{split}
g_l = f_{it} * \frac{a_{0l}}{\sum_{l' \in L(i,t)} a_{0l'}}
\end{split}
\end{align}

Clearly, $\sum_{l' \in L(i,t)} g_{l'} = f_{it}$, which means the assigning is full. And from \eqref{eq:capa_vir} we know that $f_{it} \le \sum_{l' \in L(i,t)} a_{0l'}$. Thus $g_l \le a_{0l}$, which means the traffic we assign to tunnel $l$ is less than the reserved capacity for $l$.



Suppose link $\epsilon=\langle m,n\rangle$ fails, we need to use protection routing to share part of $f_{it}$, so that tunnels containing $\epsilon$ can be released. And this will go to $r$ since protection is done using the actual links. We also need to remove the traffic routed to link $\epsilon$, i.e. make $r_{mnt}=0$ for any $t$. And we cannot use $\epsilon$ to do any protection, i.e. $p_{e mnt}=0$ for any $e,t$. The updating rules are as follows

\begin{align}
& f'_{ij} = max\{f_{ij} - \sum_{l \in L(i,j)} a_{\epsilon l}, 0\} \quad \forall i,j \in N_{edge} \label{eq:f_update1}\\
& \tilde{r}_{ijt} = r_{ijt} + p_{\epsilon ijt} \quad \forall \langle i,j \rangle \in E, t\ne n\label{eq:r_update1}
\\
& r'_{ijt} = 
\begin{cases}
\tilde{r}_{ijt} + r_{mnt} * p_{\epsilon ijn}/a_{\epsilon \epsilon} & \forall \langle i,j \rangle \in E \backslash \{\epsilon\},t  \\
0 & \forall \langle i,j \rangle=\epsilon,t
\end{cases}\label{eq:r_update}
\\
& \tilde{p}_{eijt} = 
\begin{cases}
p_{eijt} + p_{emnt} * p_{\epsilon ijn} / a_{\epsilon \epsilon} & \forall e \in E \backslash \{\epsilon\}, \langle i,j \rangle \in E \backslash \{\epsilon\},t \\
0 &\forall e \in E \backslash \{\epsilon\}, \langle i,j \rangle = \epsilon,t\\
\end{cases}\label{eq:p_update} \\
& a'_{ee} = a_{ee} - \sum_{t}\tilde{p}_{ei'j't} \quad \forall e=\langle i',j' \rangle \in E \backslash \{\epsilon\}\label{eq:a_update}\\
& a'_{el} = a_{el} \quad \forall e=\langle i',j' \rangle \in E \backslash \{\epsilon\},l\\
& p'_{eijt} = 
\begin{cases}
0, \quad \forall e=\langle i,j \rangle \in E \backslash \{\epsilon\}\\
\tilde{p}_{eijt} + \tilde{p}_{ei'j't} * \tilde{p}_{eijj'} / (a_{ee} - \tilde{p}_{ei'j'j'}), \\
\quad \forall e=\langle i',j' \rangle, \langle i,j \rangle \in E \backslash \{\epsilon, e\},j'\ne t \\
\tilde{p}_{eijt} - \sum_{t'\ne j'}\tilde{p}_{ei'j't'} * \tilde{p}_{eijj'} / (a_{ee} - \tilde{p}_{ei'j'j'}), \\
\quad \forall e=\langle i',j' \rangle, \langle i,j \rangle \in E \backslash \{\epsilon,e\},j'= t \\
\end{cases}\label{eq:p_update_final}
\end{align}

\textbf{Overview of the updating scheme} \eqref{eq:f_update1} pulls out traffic on the tunnels in order to make sure that the remaining traffic can be handled using the remaining non-failed tunnels. \eqref{eq:r_update1} puts the protection in the routing on actual links to serve the pulled out traffic in \eqref{eq:f_update1}. \eqref{eq:r_update} and \eqref{eq:p_update} are similar with the updates in R3, which makes sure that the new routing and the new protection routing will not go through the failed link. \eqref{eq:a_update} and \eqref{eq:p_update_final} serve the same purpose of the final step of R3 updates, which is to cancel the protection using the link which it protects for(caused by \eqref{eq:p_update}). In R3 updates, we remove $p_\epsilon(\epsilon)$ from $a_\epsilon$ and makes $p_\epsilon(\epsilon)$ to be 0. The reason it becomes more complicated in here is that, $p_\epsilon(\epsilon)$ here is not only for $\epsilon$, but also for protecting tunnels. We can simply remove the former one, but need to reroute the latter one. 

% proof of update
% \textbf{Updated flow balance on $r$.}
% \eqref{eq:f_update1} pulls out $\sum_{l \in L(i,j)} a_{\epsilon l}$ from $f_{ij}$. In order to serve the pulled out traffic, we use \eqref{eq:r_update1} to add protection routing on $r$ to serve $\sum_{l \in L(i,j)} a_{\epsilon l}$. The max operation in \eqref{eq:f_update1} means that if $\sum_{l \in L(i,j)} a_{\epsilon l}$ is more than $f_{ij}$, we simply pull out all $f_{ij}$. Under this situation, the added flow is more than the flow pulled out. So we have the ability to serve more. Next, we show that the new protection routing is balanced in the intermediate nodes and can serve the given demand $d$. Different from \eqref{eq:flow_balance_}, we won't show the updated $r$ will exactly serve $d$. Instead, we show that $r$ serves at least $d$.

% \begin{align}
% \begin{split}
% & \sum_{j}  \tilde{r}_{ijt} - \sum_{j}  \tilde{r}_{jit} \\
% & =\sum_{j}  (r_{ijt} + p_{\epsilon  ijt}) - \sum_{j}   (r_{jit} + p_{\epsilon jit}) \\
% & =\sum_{j}  r_{ijt} - \sum_{j} r_{jit} + \sum_{j}  p_{\epsilon ijt} - \sum_{j} p_{\epsilon jit} \\ 
% & =\begin{cases}
% \Bar{d'}_{it} & i \ne t\\
% -\sum_{j}\Bar{d'}_{jt} & i = t\\
% \end{cases} \\
% & where \quad \Bar{d'}_{it} = \Bar{d}_{it} + \sum_{l \in L(i,t)} a_{\epsilon l} \\
% & \Bar{d'}_{it} + f'_{it} \\
% & = \Bar{d}_{it} + \sum_{l \in L(i,t)} a_{\epsilon l} + max\{f_{it} - \sum_{l \in L(i,t)} a_{\epsilon l}, 0\} \\ 
% & \ge \Bar{d}_{it} + \sum_{l \in L(i,t)} a_{\epsilon l} + f_{it} - \sum_{l \in L(i,t)} a_{\epsilon l} \\
% & = \Bar{d}_{it} + f_{it} \\
% & = d_{it} \quad \forall i, t \in N_{edge}
% \end{split}
% \end{align}

% $\epsilon$ is not just used in tunnels. It is also used to route traffic as in R3 with variable $r_{mnt}$. In order to pull out this traffic, we update $r$ with \eqref{eq:r_update} as in R3. By definition, $r_{mnt} = 0$, which means $\epsilon=\langle m,n \rangle$ will not be used to route any traffic. We show that the updated $r$ is still balanced and capable to serve the demand. For convenience, let $\sum_{j}  \tilde{r}_{ijt} - \sum_{j}  \tilde{r}_{jit} = g(i,t)$.

% \begin{align}
% \begin{split}
% & \sum_{j}  r'_{ijt} - \sum_{j}  r'_{jit} \\
% & = (\sum_{j; \langle i,j \rangle \in E \backslash \{\epsilon\} } \tilde{r}_{ijt} - \sum_{j; \langle j,i \rangle \in E \backslash \{\epsilon\}} \tilde{r}_{jit}) + \\
% & \frac{r_{mnt}}{a_{\epsilon \epsilon}}(\sum_{j; \langle i,j \rangle \in E \backslash \{\epsilon\} } p_{\epsilon ijn} - \sum_{j; \langle j,i \rangle \in E \backslash \{\epsilon\}} p_{\epsilon jin}) \\
% & = \begin{cases}
% g(i,t) - r_{mnt} + \frac{r_{mnt}}{a_{\epsilon \epsilon}}*a_{\epsilon \epsilon} & i=m\\
% g(i,t) + \frac{r_{mnt}}{a_{\epsilon \epsilon} }*0 & i \ne m, i \ne n\\
% g(i't) + r_{mnt} - \frac{r_{mnt}}{a_{\epsilon \epsilon}}*a_{\epsilon \epsilon} & i = n \\
% \end{cases} \\
% & = g(i,t)
% \end{split}\label{eq:r'_flow}
% \end{align}

% \textbf{Capacity constraints on the updated variables}  \eqref{eq:r_update} follows the same structures and arguments in R3, which pulls out the traffic on the failed link and distribute to other links using the protection. $p$ is in two parts, one is used to protect the failed link, which ends in the end point of the failed link. This is completely done in the core network and is the same as in R3. The other part is used to protect the tunnels containing the failed link.

% It is easy to show that the capacity constraint still holds on virtual links between edge nodes(i.e. \eqref{eq:capa_vir}). From the capacity constraint on virtual link $\langle i,j \rangle$ for any failure scenario $x \in X$ with $x_{e'}=1$, we have
% \begin{align}
% \begin{split}
% f_{ij} \le \sum_{l \in L(i,j)} (a_{0l}\prod_{e \in l\cap E_{core}}(1-x_e)) + \sum_{\atop l \in L(i,j)} a_{e'l} + \sum_{e \in E_{core} \backslash \{ e'\} \atop l \in L(i,j)} x_e a_{el} 
% \end{split}
% \end{align}

% which gives us

% \begin{align}
% \begin{split}
% f_{ij} - \sum_{\atop l \in L(i,j)} a_{e'l} \le \sum_{l \in L(i,j)} (a_{0l}\prod_{e \in l\cap E_{core}}(1-x_e)) + \sum_{e \in E_{core} \backslash \{ e'\} \atop l \in L(i,j)} x_e a_{el} 
% \end{split}\label{eq:f_proof1}
% \end{align}

% It is trivial that 

% \begin{align}
% \begin{split}
% 0 \le \sum_{l \in L(i,j)} (a_{0l}\prod_{e \in l\cap E_{core}}(1-x_e)) + \sum_{e \in E_{core} \backslash \{ e'\} \atop l \in L(i,j)} x_e a_{el} 
% \end{split}\label{eq:f_proof2}
% \end{align}

% Combining \eqref{eq:f_proof1} and \eqref{eq:f_proof2} we can show that 

% \begin{align}
% \begin{split}
% & f'_{ij} = max\{f_{ij} - \sum_{l \in L(i,j)} a_{e'l}, 0\} \\  
% & \le \sum_{l \in L(i,j)} (a_{0l}\prod_{e \in l\cap E_{core}}(1-x_e)) + \sum_{e \in E_{core} \backslash \{ e'\} \atop l \in L(i,j)} x_e a_{el} 
% \end{split}
% \end{align}

% It is more complicated to show that the capacity constraint holds on actual links(i.e. \eqref{eq:capa_act}). We first show that $r', \tilde{p}, a$ satisfies capacity constraints. Note that this step(\eqref{eq:p_update}) ensures that future protection routing will not use the failed link $\epsilon$.

% From the capacity constraint on $\epsilon$ for any failure scenario $x \in X$ with $x_\epsilon=1$, we have:
% \begin{align}
% \begin{split}
% & ~~\sum_{t} r_{mnt} + \sum_{t,e \in E \backslash \{\epsilon\}} x_ep_{emnt} \le a_{\epsilon\epsilon}
% \\
% \end{split}\label{eq:g_define}
% \end{align}
% And from the capacity constraint on $\langle i, j \rangle \in E, \langle i, j \rangle \ne \epsilon$ for any failure scenario $x \in X$ with $x_\epsilon=1$, we have:
% \begin{align}
% \begin{split}
% & ~~\sum_{t} r_{ijt} + \sum_{t} p_{\epsilon ijt} + \sum_{t,e \in E \backslash \{\epsilon\}} x_ep_{eijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & \le  U c_{\langle i,j \rangle} (1-x_{\langle i,j \rangle}) + x_{\langle i,j \rangle} a_{\langle i,j \rangle \langle i,j \rangle}
% \\
% \end{split}\label{eq:g_define}
% \end{align}

% \begin{align}
% \begin{split}
% & \forall \langle i, j \rangle \in E\backslash \{\epsilon\}, \\
% & ~~\sum_{t} r'_{ijt} + \sum_{t,e \in E \backslash \{\epsilon\}} x_e\tilde{p}_{eijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & = \sum_{t} r_{ijt} + \sum_{t \ne l} p_{\epsilon ijt} + r_{mnt}\frac{p_{\epsilon ijl}}{a_{\epsilon\epsilon}} +  \\
% & \sum_{t, e \in E\backslash \{\epsilon\}} x_e( p_{ejit} + p_{emnt}\frac{p_{\epsilon ijn}}{a_{\epsilon\epsilon}}) + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & = \sum_{t} r_{ijt} + \sum_{t \ne l} p_{\epsilon ijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) + \\
% & \sum_{t,e \in E \backslash \{\epsilon\}} x_ep_{eijt} + \frac{p_{\epsilon ijn}}{a_{\epsilon\epsilon}} (\sum_{t} r_{mnt} + \sum_{t,e \in E \backslash \{\epsilon\}} x_ep_{emnt}) \\
% & \le \sum_{t} r_{ijt} + \sum_{t \ne l} p_{\epsilon ijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) + \\
% & \sum_{t,e \in E \backslash \{\epsilon\}} x_ep_{eijt} + \frac{p_{\epsilon ijn}}{a_{\epsilon\epsilon}} a_{\epsilon\epsilon} \\
% & = \sum_{t} r_{ijt} + \sum_{t} p_{\epsilon ijt} + \sum_{t,e \in E \backslash \{\epsilon\}} x_ep_{eijt} + \\
% & \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & \le U c_{\langle i,j \rangle} (1-x_{\langle i,j \rangle}) + x_{\langle i,j \rangle} a_{\langle i,j \rangle \langle i,j \rangle} \\
% \end{split}
% \end{align}

% \eqref{eq:p_update} creates some invalid protection in which a link may use itself to do protection. \eqref{eq:a_update} and \eqref{eq:p_update_final} are used to pull out these invalid protection routing. By definition, $p'_{eijt} = 0 \forall e = \langle i,j \rangle$, which means no protection will use itself. Now we show that after this final update, the flow balance constraint still holds, i.e. $r', p', a'$ satisfies capacity constraints. 

% \begin{align}
% \begin{split}
% & \forall \langle i,j \rangle \in E\backslash \{\epsilon\}, e = \langle i',j'
% \rangle \in E\backslash \{\epsilon, \langle i,j \rangle\}\\
% & \sum_{t} p'_{eijt} \\
% & = \sum_{t \ne j'} p'_{eijt} + p'_{eijj'}\\
% & = \sum_{t \ne j'} \tilde{p}_{eijt} + \tilde{p}_{ei'j't} * \tilde{p}_{eijj'} / (a_{ee} - \tilde{p}_{ei'j'j'})  \\
% & + \tilde{p}_{eijj'} - \sum_{t'\ne j'}\tilde{p}_{ei'j't'} * \tilde{p}_{eijj'} / (a_{ee} - \tilde{p}_{ei'j'j'})\\
% & = \sum_{t \ne j'} \tilde{p}_{eijt} + \tilde{p}_{eijj'} \\
% & = \sum_{t} \tilde{p}_{eijt}
% \end{split}
% \end{align}

% \begin{align}
% \begin{split}
% & \forall e'=\langle i,j \rangle \in E\backslash \{\epsilon\}, \\
% & ~~\sum_{t} r'_{ijt} + \sum_{t,e \in E \backslash \{\epsilon\}} x_ep'_{eijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & = \sum_{t} r'_{ijt} + \sum_{t} x_e'p'_{e'ijt} + \sum_{t,e \in E \backslash \{\epsilon,e'\}} x_ep'_{eijt} + \\
% & \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & = \sum_{t} r'_{ijt} + 0 + \sum_{t,e \in E \backslash \{\epsilon,e'\}} x_e\tilde{p}_{eijt} + \sum_{l \in T(i,j)}(a_{0l}\prod_{e \in l \cap E_{core}}(1-x_e)) \\
% & \le  U c_{e'} (1-x_{e'}) + x_{e'} a_{e'e'} - \sum_{t} x_{e'}\tilde{p}_{e'ijt} \\
% & =  U c_{e'} (1-x_{e'}) + x_{e'}( a_{e'e'} - \sum_{t}\tilde{p}_{e'ijt} )\\
% & =  U c_{e'} (1-x_{e'}) + x_{e'} a'_{e'e'}
% \end{split}
% \end{align}

% \textbf{Updated flow balance on $p$ and $a$.} With proof similar with \eqref{eq:r'_flow}, we can show flow balance on $\tilde{p}$ and $a$. Now we show the flow balance on $p'$ and $a'$.

% For convenience, let $\sum_{j} \tilde{P}_{eijt} - \sum_{j}  \tilde{P}_{ejit} = h(e,i,t)$.

% \begin{align}
% \begin{split}
% & \forall e = \langle i', j' \rangle \in E \backslash \{\epsilon \}, t \ne j' \\
% & \sum_{j}  p'_{eijt} - \sum_{j}  p'_{ejit} \\
% & = (\sum_{j; \langle i,j \rangle \in E \backslash \{\epsilon, e\} } \tilde{p}_{eijt} - \sum_{j; \langle j,i \rangle \in E \backslash \{\epsilon, e\}} \tilde{p}_{ejit}) + \\
% & \frac{\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}(\sum_{j; \langle i,j \rangle \in E \backslash \{\epsilon,e\} } \tilde{p}_{eijj'} - \sum_{j; \langle j,i \rangle \in E \backslash \{\epsilon,e\}} \tilde{p}_{ejij'}) \\
% & = \begin{cases}
% h(e,i,t) - \tilde{p}_{ei'j't} + \frac{\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}*(a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}) & i=i'\\
% h(e,i,t) + \frac{\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}*0 & i \ne i', i \ne j'\\
% h(e,i,t) + \tilde{p}_{ei'j't} - \frac{\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}*(a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}) & i = j' \\
% \end{cases} \\
% & = h(e,i,t)
% \end{split}\label{eq:r'_flow}
% \end{align}

% \begin{align}
% \begin{split}
% & \forall e = \langle i', j' \rangle \in E \backslash \{\epsilon \}, t = j' \\
% & \sum_{j}  p'_{eijt} - \sum_{j}  p'_{ejit} \\
% & = (\sum_{j; \langle i,j \rangle \in E \backslash \{\epsilon, e\} } \tilde{p}_{eijt} - \sum_{j; \langle j,i \rangle \in E \backslash \{\epsilon, e\}} \tilde{p}_{ejit}) - \\
% & \frac{\sum_{t \ne j'} \tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}(\sum_{j; \langle i,j \rangle \in E \backslash \{\epsilon,e\} } p_{eijj'} - \sum_{j; \langle j,i \rangle \in E \backslash \{\epsilon,e\}} p_{ejij'}) \\
% & = \begin{cases}
% a_{ee} - \tilde{p}_{ei'j'j'} - \frac{\sum_{t \ne j'}\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}*(a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}) & i=i'\\
% 0 + \frac{\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}*0 & i \ne i', i \ne j'\\
% -a_{ee} + \tilde{p}_{ei'j'j'} + \frac{\sum_{t \ne j'}\tilde{p}_{ei'j't}}{a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}}*(a_{\epsilon \epsilon} - \tilde{p}_{ei'j'j'}) & i = j' \\
% \end{cases} \\
% & = \begin{cases}
% a_{ee} - \sum_{t}\tilde{p}_{ei'j't} = a'_{ee} & i=i'\\
% 0 & i \ne i', i \ne j'\\
% -a_{ee} + \sum_{t}\tilde{p}_{ei'j't} = -a'_{ee} & i = j' \\
% \end{cases} 
% \end{split}\label{eq:p'_flow}
% \end{align}


\section{design}
\label{sec:design}

Suppose we have a set of flows $F$ where each flow in $F$ has SLO requirement to sustain desirable performance with probability of $\beta$. To achieve that, we want to design a routing to optimize the SLO performance of the worst application. Because if even the worst application has desirable performance with probability of $\beta$, we can guarantee that each application will have desirable performance with probability of $\beta$. We first introduce a metric to capture this application-level SLO performance. \cj{roadmap for this section? metric, formulation, decomposition}

%Based on the definition of \AppOptLoss{}, we know that all applications will have no more than loss of \AppOptLoss{} with probability of $\beta$. For example, if $\beta$ is $0.99$ and we have a routing which provides \AppOptLoss{} of $10\%$, then this routing ensures that any application will see no more than $10\%$ loss with probability of $0.99$. So we want to design routing for each failure scenario so that \AppOptLoss{} is minimized. Next, we illustrate our key notations and how we model this problem.

%-For each flow, flow-loss is weighted sum of loss across scenarios, with the weight corresponding to how likely that scenario is bad.
%Pick the best routing.
% $min x$
%-Take a weighted sum of the flow-loss across all the flows with the weight being how likely that flow is a bottleneck flow. Pick the best weights for which scenario is bad for each flow.
%  $max_w min_x$
%-Optimize this across all the possible weights for the bottleneck flow.
%  $max_\lambda max_w min_x$
  
%Write applications with multiple flows, start with single target. Then present multiple targets as a separate thing.

\begin{table}[t]
  %\small
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|| c || p{6cm}||} 
    \hline
      notation  & meaning\\
    \hline\hline
$Q$ & Set of all scenarios \\
$A$ & Set of applications \\
$P$ & Set of source-destination pairs\\
$R(i)$ & Set of tunnels for pair $i$\\
$E$ & Set of edges\\
$d_{ai}$ & Traffic demand of flow set $a$ along pair $i$ \\
$\beta$ & Target probability for which the bandwidth requirement must be met\\
$p_q$ & Probability of scenario q\\
$y_{tq}$ & 1 if tunnel $t$ is alive in scenario $q$, 0 otherwise\\
$x_{tq}$ & Allocated bandwidth on tunnel $t$ in scenario $q$(routing variable)\\
$l_{aq}$ & Loss of application $a$ in scenario $q$\\
$z_{aq}$ & 1 if scenario $q$ is considered for application $a$ to meet the target probability, 0 otherwise \\
\hline    
    \end{tabular}
    }
    \caption{Notation}
    \label{tab:notations}
    \vspace{-0.3in}
\end{table}

\subsection{Problem Formalism} 

\mt{Why not just say, we define $\AppLoss{}(a,\beta)$ to be the $\beta^{\text{th}}$ percentile of loss for service $a$?}
For each application $a \in A$, we define $\AppLoss{}(a,\beta)$ to be the upper bound on the loss of $a$ for probability of $\beta$. That is to say that the loss experienced by $a$ is no more than $\AppLoss{}(a,\beta)$
with probability of at least $\beta$, i.e., \mt{This notation is confusing. The $|$ in probability means conditioning. Better to write: $P\bigl(q\text{ s.t. } l(a,q) \le \AppLoss{}(a,\beta)\bigr) \ge \beta $ or even $P\bigl(l(a,q) \le \AppLoss{}(a,\beta)\bigr) \ge \beta $.} $P(q\ |\ l(a,q) \le \AppLoss{}(a,\beta)) \ge \beta $. Here, $l(a,q)$ is the loss of $a$ in scenario $q$, and $P(q\ |\ l(a,q) \le \phi)$ represents the cumulative probability
mass of all failure scenarios where application $a$'s loss will be no more than $\phi$. 

Note that the loss of an application can be defined differently under different settings. For example, we can assume each application only contains single flow, and every source-destination pair has only one application running on it. In that case, the loss of an application is simply the loss on the corresponding pair, i.e., $l(a,q) = L_{iq}$ where pair $i$ corresponds to application $a$. In more general cases where an application contains multiple flows, we can define the loss to be the max loss across its flows. For example, based on this definition, if $l(a,q) = 5\%$, we know that all flows of $a$ will not experience more than 5\% loss in scenario $q$. 

As mentioned before, to make sure every application has desirable performance, we should optimize the routing so that even the worst application will not encounter too much loss. So we are interested in 

\begin{align}
\AppOptLoss{} = max_{a \in A}\{\AppLoss{}(a,\beta)\}
\end{align}, 

which represents the worst \AppLoss{} across applications. With $\AppOptLoss{}$, we can claim an SLO guarantee such that with probability of $\beta$, no application will encounter a bandwidth loss of more than \AppOptLoss{}. \cj{example?}

Now, let's compare \AppOptLoss{} with scenario-centric metric used in the state-of-the-art. For example, Teavar tries to optimize \ScenOptLoss{}, which is the upper bound on the \ScenLoss{} for probability of $\beta$, i.e.  $P(q\ |\ \ScenLoss{}_q \le \ScenOptLoss{}) \ge \beta$. Note that the definition of \ScenOptLoss{} doesn't reflect the fact that different applications(or different flows) can meet their SLO through different scenarios. Instead, it is looking for a set scenarios where all applications are performing well, which is more restricted. Thus, the SLO guarantee provided by \ScenOptLoss{} can be more conservative(guarantee a higher loss). We can prove that with any routing, $\ScenOptLoss{}$ is a more conservative metric than $\AppOptLoss{}$, i.e., $\AppOptLoss{}$ is never higher than $\ScenOptLoss{}$.

\begin{proposition}\label{prop:ffcim_beats_ffc}
With any possible routing, $\AppOptLoss{} \le \ScenOptLoss{}.$
\end{proposition}
\textbf{Proof.}


\mt{Isn't it easier to say it the following? 

In our framework, we compute 
\begin{equation*}
\alpha^N := \min_{x\in \text{routing}}\max_{s \in \text{services}} \Var_\beta\bigl(\max_{i \in s}l_{iq}(x)\bigr).
\end{equation*}
In the above notation, $\Var_\beta(\cdot)$ represents the $\beta^{\text{th}}$ percentile of its argument. Here, for each service $s$, we compute the $\beta^{\text{th}}$ percentile as the $\beta^{\text{th}}$ percentile for the worst associated flow. Then, the outer problem chooses a routing that minimizes the $\beta^{\text{th}}$ percentile for the worst service. This guarantees that no service experiences a loss of more than $\alpha^N$ in scenarios with probability more than $1-\beta$. Instead, prior literature solved $\min_{x\in \text{routing}}\Var_{\beta}\bigl(\max_{i\in \text{pairs}} l_{iq}(x)\bigr)$. Assume $\text{services}$ are the same as $\text{pairs}$ and that there is a unique flow in each service. Then, $\alpha^N =  \max_{i \in \text{pairs}} \Var_\beta\bigl(l_{iq}(x)\bigr)$. In essence, we switch the order of maximization and percentile computation. Given an $x$, for any $i$, $\Var_\beta (l_{iq}(x)) \le  \Var_{\beta}(\max_{i\in \text{pairs}} l_{iq}(x))$. Therefore,  
\begin{equation*}
    \max_{i \in \text{pairs}} \Var_\beta\bigl(l_{iq}(x)\bigr) \le \Var_{\beta}\bigl(\max_{i\in \text{pairs}} l_{iq}(x)\bigr),
\end{equation*} 
and it follows that the new metric results in better performance guarantees than previously possible.}





\subsection{Notation and preliminaries}


Consider a network topology, represented as a graph $G= \langle V, E 
\rangle $. Each link $e \in E$ is associated with a link capacity $c_e$. We use $P$ to represent the set of source-destination pairs. Each pair $i$ can use a set of tunnels $R(i)$ to route the traffic. Each application $a \in A$ requires bandwidth to send traffic for multiple source-destination pairs. We are given the traffic demand $d_{ai}$ for pair $i$ in application $a$. %We define the loss of an application $a$ in a failure scenario $q$ $l(a,q)$ as its max loss across pairs. For example, if an application $a$ has $10\%$ loss in a scenario, then at least one of its source-destination pairs $i$ only has $0.9d_{ai}$ bandwidth, and no pair will see a loss more than $10\%$.

$Q$ represents the set of failure scenarios. For each scenario $q \in Q$, $p_q$ represents the probability of $q$. And $y_{tq}$ represents whether a tunnel $t$ is alive in scenario $q$. We use $x_{tq}$ to denote the bandwidth assigned to tunnel $t$ in scenario $q$, i.e., our designed routing. %We have to ensure that the assigned bandwidth will not exceed link capacity, i.e.,$\sum_{e \in t} x_{tq} \le c_e$. %Based on our definition of application loss(max loss across pairs), we can compute $l(a,q)$ by $l(a,q) = \max_{i \in P, d_{ai} > 0}  1 - \frac{\sum_{l \in R(i)}x_{tq}y_{tq}}{d_{ai}}$.

In order to make sure each application meets its SLO, we are essentially selecting enough scenarios for each application to cover probability of $\beta$. We use $z_{aq}$ to represent whether we choose the scenario $q$ for application $a$. If $z_{aq}$ is $0$, it means to get to probability of $\beta$, we don't need scenario $q$ for application $a$, so we don't care about $loss(a,q)$. If $z_{aq}$ is $1$, it means that we care about application $a$ in scenario $q$, so the loss of application $a$ cannot exceed \AppOptLoss{}, i.e.,$l(a,q)z_{a,q} \le \AppOptLoss{}$. %And to cover probability of $\beta$ for each application, we have the following constraint $\sum_{q \in Q} z_{aq}p_q \ge \beta$.

Thus, we can write the following formulation to find the best routing and selection of scenarios to achieve the minimized \AppOptLoss{}.

\begin{align}
\mbox{($I$)} \ 
& \min_{z,x,loss,\alpha} \quad \alpha \nonumber \\ 
\mbox{s.t.} 
& \sum_{q \in Q} z_{aq}p_q \ge \beta \quad \forall a \in A \label{eq:availability}\\
& z_{aq} \in \{0,1\} \quad \forall a \in A,q \in Q \label{eq:binary} \\
& 0 \le l_{aq} \le 1 \quad \forall a \in A, q \in Q \label{eq:positive_loss} \\
& \alpha \ge l_{aq} - 1 + z_{aq}  \quad \forall a \in A, q \in Q \label{eq:loss_bound} \\
%& loss(a,q) \ge  1 - \frac{\sum_{l \in R(i)}x_{alq}y_{lq}}{d_{ai}} \quad \forall i \in P, q \in Q, a \in A \label{eq:demand} \\
& \sum_{a \in A} (1-l_{aq})d_{ai} \le  \sum_{t \in R(i)}x_{tq}y_{tq} \quad \forall i \in P, q \in Q \label{eq:demand} \\
& \sum_{e \in t} x_{tq} \le c_e \quad \forall e \in E,q \in Q \label{eq:capacity}\\
&\mt{x_{tq}\ge 0 \quad \forall t\in ??, q\in Q}
\end{align}

In the above formulation, \eqref{eq:availability} is to ensure that for each application, we are selecting enough scenarios to cover the SLO target probability $\beta$. When $z_{aq}=1$, we are selecting scenario $q$ to cover application $a$'s SLO target. \eqref{eq:loss_bound} becomes $\AppOptLoss{} \ge l_{aq}$ meaning we care about the loss $l_{aq}$. When $z_{aq}=0$, \eqref{eq:loss_bound} is satisfied no matter what $\AppOptLoss{}$ and $l_{aq}$ are, meaning we don't care about the loss $l_{aq}$. \eqref{eq:demand} is to ensure that there is enough bandwidth allocated to each pair. The LHS of \eqref{eq:demand} is the total amount of traffic required to be sent on pair $i$, and the RHS is the total allocated bandwidth on tunnels connecting pair $i$. \eqref{eq:capacity} is to make sure the allocated bandwidth on tunnels will never exceed any link's capacity.
%Note that we rewrite $l(a,q)z_{a,q} \le \AppOptLoss{}$ as \eqref{eq:loss_bound} to avoid quadratic term. We use \eqref{eq:positive_loss} to ensure that loss is non-negative. 

%Here, $x_{lq}$ represents the bandwidth we allocate to tunnel $l$ in scenario $q$. $t_{qa}$ represents the loss of application $a$ in scenario $q$, which means that for each flow $i$, at least $(1-t_{qa})d_{ai}$ traffic should be transferred in scenario $q$. The value of $w_{qa}$ represents a selection of scenarios for application $a$. The inner max over $w$ is to find scenarios with most loss for each application and compute the average loss, and max over $a \in A$ is to find the application with worst average loss. Since every application has its own $w$  variable, the selection of worst $1-\beta$ scenarios can be different for each application, unlike Teavar. In other words, different applications can achieve their target availability through different set of scenarios, which allows more flexibility in coordinating traffic across applications to achieve SLO. For example, in the scenario shown in Fig.\ref{fig:flow_example_1}, the above model allows the network to ignore application 2(AD flow) so that application 1(AC flow) gets all the bandwidth, while Teavar forces the two applications to share bandwidth and raises the loss.

\subsection{Decomposition}
\label{sec:decomposition}

With $z_{aq}$ being a binary variable, (I) is an MIP formulation where we try to find enough scenarios for each application, and to design a routing for each scenario at the same time. As mentioned in \S\ref{sec:motivation}, with large size of topology and a large set of scenarios, solving the MIP in (I) can be very difficult. In this section, we introduce how we can decompose (I) and speed up by paralleling the computation.

We use Bender's decomposition~\cite{Benders} algorithm to decompose (I). We can rewrite the objective function of (I) as a two step problem by separating the variables

\begin{align}
\min_{z} \min_{x,loss,\alpha} \alpha
\end{align}.

The outer problem is to decide $z$, which is to determine in each scenario, which flows should be taken care of. With a given $z$, the inner problem is to find the routing for each scenario to minimize the loss, which can be seen as a function of $z$. And then (I) can be rewritten as

\begin{align}
\mbox{($I'$)} \ 
& \min_{z} \quad \AppOptLoss{}(z)  \quad
\mbox{s.t.} \eqref{eq:availability}, \eqref{eq:binary} 
\end{align}

where

\begin{align}
\AppOptLoss{}(z) = \min_{x,loss,\alpha}  \alpha  \quad \mbox{s.t.} 
\eqref{eq:positive_loss},\eqref{eq:loss_bound}, \eqref{eq:demand}, \eqref{eq:capacity} \label{eq:inner_min}
\end{align}

\begin{figure}[t]
	\centering
    	    \includegraphics[trim={8.3cm 12.3cm 15.3cm 1.8cm}, clip, width=0.48\textwidth]{figures/z_function.pdf}
        \label{fig:z_function}
\vspace{-0.25in}
    \caption{An example of function \AppOptLoss{}(z). Solving \eqref{eq:inner_min} on $z_1$ and $z_2$ provides two tangents to estimate \AppOptLoss{}(z). And $z_p$ is the minimal based on this estimation.} 
        \label{fig:z_function}
\end{figure}

\begin{figure}[t]
	\centering
    	    \includegraphics[trim={3.3cm 12.3cm 4.3cm 2.8cm}, clip, width=0.48\textwidth]{figures/bender_procedure.pdf}
        \label{fig:bender_procedure}
\vspace{-0.25in}
    \caption{The master problem decides which flows to consider in each scenario, and the subproblems decide how to route in each scenario. Note that the subproblems can be solved in parallel. } 
        \label{fig:bender_procedure}
\end{figure}

Fig.~\ref{fig:z_function} shows an example \AppOptLoss{}(z) function. \mt{Indeed, the optimal objective value for the inner problem is convex in $z$. This is a well-known property of linear programs. It follows from the fact that if, for all $i$,  $(x^i,\text{loss}^i,\alpha^i)$ is feasible when $z=z^i$, then for some multipliers $\lambda_i\ge 0$ such that $\sum_i \lambda_i = 1$, the solution $\sum_i \lambda_i (x^i,\text{loss}^i,\alpha^i)$ is feasible when $z=\sum_i\lambda_i z^i$. This shows that, the optimal value of the inner problem at $z$ is no more than $\sum_i \lambda_i \alpha^i$.}  Bender's decomposition algorithm provides a systematic way to find the minimizer of \AppOptLoss{}(z) iteratively. Although the exact shape of \AppOptLoss{}(z)'s is unknown at any point in the algorithm, solving \eqref{eq:inner_min} gives us one point on the function \AppOptLoss{}(z). Moreover, the dual form of \eqref{eq:inner_min} provides a tangent of \AppOptLoss{}(z) \mt{(because its feasible region does not depend on $z$)}. Thus, we derive an underestimation of \AppOptLoss{}(z) by evaluating it at various $z^i$. Each tangent is a lower bound of function \AppOptLoss{}(z), and the pointwise maximum of these tangents is an underestimate of \AppOptLoss{}(z). Then, we can find the current estimated minimizer of the estimated function(e.g., $z_p$ in Fig.~\ref{fig:z_function}). Solvng \eqref{eq:inner_min} at $z^p$ gives a new tangent and a more accurate estimate of \AppOptLoss{}(z). \mt{We remark that the inner problem is always feasible with $(x,\text{loss},\alpha) = (0,1,1)$ and bounded between $0$ and $1$. If we use an extreme point of the dual feasible region to generate a tangent (as is the case using dual simplex algorithm), in finitely many iterations, a cut is developed for each extreme point, and we have an accurate representation of \AppOptLoss{}(z). As such, the process converges in finite time with an optimal solution. } The following formulation shows how to find the minimal on the current estimation formed by tangents. We call this the master problem.

\begin{align}
\mbox{($M$)} \ 
& \min_{z,\AppOptLoss{}} \quad \AppOptLoss{} \nonumber \\ 
\mbox{s.t.} 
& \eqref{eq:availability}, \eqref{eq:binary} \nonumber \\
& \AppOptLoss{} \ge f_q(z) \quad \forall f \in F \label{eq:cut_} 
\end{align}
$F$ represents the set of all tangents computed so far. So \eqref{eq:cut_} ensures that all tangents are treated as a lower bound of \AppOptLoss{}, forming an estimation.

As mentioned before, \eqref{eq:inner_min} is to find the routing for each scenario, provided which flows to consider in each scenario. Since the routing in each scenario can be derived independently of that in other scenarios, the problem decomposes by scenarios. Therefore, we solve the following subproblem for each scenario $q\in Q$:
\begin{align}
\mbox{($S_q$)} \ 
& \min_{x,l,\alpha} \quad \alpha \nonumber \\ 
\mbox{s.t.} 
& \alpha \ge l_{aq} - 1 + z_{aq}  \quad \forall a \in A \label{eq:loss_bound_} \\
& 0 \le l_{aq} \le 1 \quad \forall a \in A \label{eq:positive_loss_} \\
& \sum_{a \in A} (1-l_{aq})d_{ai} \le  \sum_{t \in R(i)}x_{tq}y_{tq} \quad \forall i \in P \label{eq:demand_} \\
& \sum_{e \in l} x_{tq} \le c_e \quad \forall e \in E. \label{eq:capacity_}
\end{align}

Note that $z_{aq}$ is a parameter in ($S_q$). Suppose the dual variables for \eqref{eq:loss_bound_}, \eqref{eq:positive_loss_}, \eqref{eq:demand_}
 and \eqref{eq:capacity_} are $w_{aq}$, $o_{aq}$, $v_{iq}$ and $u_{eq}$ respectively. Then we will have the tagent on \AppOptLoss{} as the following function on $z$.
 
 \begin{align}
 f_\mt{q}(z) = \sum_{a}(z_{aq}-1)w_{aq} + \sum_{a}o_{aq} + \sum_{ai}v_{iq}d_{ai} + \sum_{e}u_{eq}c_e. \label{eq:cut_function}
 \end{align}
 
 \begin{algorithm}
\caption{Bender's decomposition algirthom}
 \label{alg:bender}
\begin{algorithmic}[1]

\Function{$solve\_master$}{$F$} 
    \State Solve ($M$) with $F$, and get variable $z$
    \State \Return $z$
\EndFunction
\Function{$solve\_subproblem$}{$z$,$q$}  
    \State Solve ($S_q$) and get routing variable $x$, and dual variables $w_{aq}$, $o_{aq}$, $v_{iq}$ and $u_{eq}$
    \State Construct $f$ as in \eqref{eq:cut_function}
    \State \Return $x$, $f$
\EndFunction
\Function{main}{$max\_iterations$}   
    \State $k \leftarrow 0$ 
    \State $F \leftarrow \emptyset$
    \While{$k < max\_iterations$} 
        \State $z \leftarrow sovle\_master(F)$  
          \For{$q \in Q$}
        \State $x_q,f \leftarrow solve\_subproblem(z,q)$
        \State $F.add(f)$
      \EndFor
      $k \leftarrow k+1$ 
    \EndWhile 
    \State \Return $x$
\EndFunction

\end{algorithmic}
\end{algorithm}

Note that $S_q$ is a small LP, and for each $q\in Q$, $S_q$ can be solved independently of one another. This means that we can parallelize the solution of these LPs to speed up the solution process. Fig.~\ref{fig:bender_procedure} shows the procedure of using Bender's decomposition algorithm on (I). And Algorithm~\ref{alg:bender} provides the pseudocode. \mt{We remark that each iteration, Bender's algorithm yields a routing strategy and the corresponding 
\AppOptLoss{} can be computed easily by sorting the optimal values for $S_q$ and computing the $\beta^{\text{th}}$ percentile.}


%The key idea is to think of (I) as two steps. The first step is to find scenarios to cover SLO target for each application, i.e., deciding $z_{aq}$ variables. With $z_{aq}$ being decided, the applications needed to be taken care of, and the traffic demand needed to be served are also decided for each scenario. Then we can find a routing to minimize the loss in each scenario separately. Bender's decomposition~\cite{Benders} algorithm allows us to iteratively executing the two steps, and use the second step to improve the selection of $z_{aq}$ in the first step. 

%In the first step, we solve the following master problem (M) to decide selection of $z_{aq}$.

%\begin{align}
%\mbox{($M$)} \ 
%& \min_{z,\AppOptLoss{}} \quad \AppOptLoss{} \nonumber \\ 
%\mbox{s.t.} 
%& \sum_{q \in Q} z_{aq}p_q \ge \beta \quad \forall a \in A \label{eq:availability_}\\
%& z_{aq} \in \{0,1\} \quad \forall a \in A,q \in Q \label{eq:binary_} \\
%& \AppOptLoss{} \ge f_{kq}(z) \quad \forall q \in Q, k = 1,2,3,...,K \label{eq:cut_} 
%\end{align}

% \eqref{eq:availability_} and \eqref{eq:binary_} are the same as in (I) to ensure the selection of scenarios is valid and can cover the SLO probability target $\beta$ for each scenario. \eqref{eq:cut_} is where we can improve the selection of $z_{aq}$ iteratively through bounding functions $f_{kq}$. $K$ is the number of iterations finished. In each iteration $k$, we get functions $f_{kq}$ by solving the following sub-problems in the second step.



%Based on Bender's decomposition algorithm, the dual formulation of the sub-problems ($S_q$) gives a bound on the master problem $(M)$. Suppose we solve $S_q$ in $k_{th}$ iteration, and the dual variables for \eqref{eq:loss_bound_}, \eqref{eq:positive_loss_}, \eqref{eq:demand_} and \eqref{eq:capacity_} are $w_{aqk}$, $o_{aqk}$, $v_{iqk}$ and $u_{eqk}$. Then we will have a bound on \AppOptLoss{} as the following function on $z$.
 
 %\begin{align}
 %f_{kq}(z) = \sum_{a}(z_{aq}-1)w_{aqk} + \sum_{a}o_{aqk} + \sum_{ai}v_{iqk}d_{ai} + \sum_{e}u_{eqk}c_e \label{eq:cut_function}
 %\end{align}
 


 
\subsection{Heuristics}
\label{sec:heuristics}

Bender's decomposition algorithm is an iterative algorithm. Here, we introduce a few simple heuristics which can help the algorithm to find better routings more quickly.

\textbf{Starting point}. We want to start with $z$ which is likely to be close to the real minimizer for the outer problem, so that the algorithm requires fewer iterations to converge. As shown in Algorithm~\ref{alg:bender}, the master problem in first iteration will be solved with $F$ being $\emptyset$, which means that there is no tangent to estimate. This will lead to a random $z$, which can be far away from the real minimizer. One way to start with a $z$ closer to its optimal setting is to first assume that $z_{aq}$ is 1 for all $a$ and $q$. 
\mt{If we solve $S_q$ for all scenarios with this setting, we will observe that for certain $(a,q)$, the constraints \label{eq:loss_bound_} are binding. We use some of these flows, particularly, when the flow has no feasible path or the optimal $\alpha$ and the multiplier of \label{eq:loss_bound_} is large to choose $(a,q)$ so that $z_{aq}$ is set to 0.  }

\textbf{Do not allow too many changes in $z$}. \mt{Do not allow too many changes in $z$?} With a proper starting point, we may still end up far away from the minimal due to the current estimation being too coarse(For example, in the first few iterations, we don't have enough tangents). Thus, we want to restrict the step we take when we update $z$. That is, in each iteration, we make sure the new estimated minimizer not too far away from the last iterate. One way to achieve this is to add constraints in (M) to limit the hamming distance between current $z$ variable and $z$ variable achieved from last iteration. \mt{We remark that this constraint can hurt the convergence of the algorithm to the optimal solution. To circumvent this issue, the Hamming distance constraint can be relaxed, when no imrpovement is found.}

\textbf{Scenarios without loss}. \mt{For any scenario $q$ such that all flows can serviced without incurring loss, we need not solve the subproblem since $f_q(z)\le 0$. Indeed, $f_q(1) \le 0$ and $f_q(z)$ is a non-decreasing function of $z$, which shows that $f_q(z) \le 0$ for all $z$. Therefore, such constraints \eqref{eq:cut_} are not useful. We can detect such scenarios by setting solving $S_q$ initially with $z_{aq}$ set to $1$ and, if the objective is $0$, we fix $z_{aq}=1$ in the master problem. This strategy can be generalized. If we find that, for a scenario $q'$, the optimal value of $S_{q'}$ is $\alpha_{q'}$, then we need not solve $S_q$ for scenario that has a smaller loss for a larger $z$. For example, if the optimal value with all $z_{aq} = 1$ is smaller than $\alpha_{q'}$ this problem does not need to be solved.} all flows can be served without loss, then we should always include all flows in this scenario. Before Bender's algorithm, we can run ($S_q$) with $z_{aq}$ being 1 to see which scenarios have such property(objective being 0). Then we add constraints in (M) to make sure that for these scenarios $z_{aq}=1$ for every $a$. 

\textbf{Impossible flow}. \mt{this can be covered under the first set of heuristics.} If under a scenario, a pair gets disconnected, there is obviously no way to send any flow on this pair. So any $a\in A$ involves such pairs should not be included in this scenario. Based on this, we can compute the the disconnected flows in each scenario, and add constraints $z_{aq} =0$ in (M) for those flows.

==> zevaluation.tex <==
\section{Evaluations}\label{sec:evaluation}

\begin{figure*}

\begin{minipage}{0.25\textwidth}
    \begin{center}
    \vspace{-0.4in}
    \begin{tabular}{c c c c } 
    \hline
    MLU & F=0 & F=1 & F=2 \\ 
    \hline\hline
    VN & 0.59 & 1.19 & inf\\  
    R3 & 0.59 & 1.19 & inf\\
    FFC & 0.89 & 1.82 & inf \\
    Optimal & 0.59 & 1.19 & inf\\
    \hline
    \end{tabular}
    \vspace{0.25in}
    \captionof{table}{Abilene MLU result.}\label{tab:abilenemlu}
    \end{center}
\end{minipage}\hspace{0.1in}
%
\begin{minipage}{0.25\textwidth}
    \begin{center}
    \vspace{-0.4in}
    \begin{tabular}{c c c c } 
    \hline
    Throughput & F=0 & F=1 & F=2 \\ 
    \hline\hline
    VN & 49.26 & 47.37 & 30.21\\  
    R3 & 49.26 & 47.37 & 8.24\\
    FFC & 49.26 & 39.19 & 18.92 \\
    Optimal & 49.26 & 47.37 & 31.39\\
    \hline
    \end{tabular}
    \vspace{0.25in}
    \captionof{table}{Abilene throughput result.}\label{tab:abilenethroughput}
    \end{center}
\end{minipage}\hspace{0.1in}
\vspace{-0.3in}
\end{figure*}

We evaluate the effectiveness of our \vn{} model in validating edge-core network designs built upon real network topologies. We do case studies on Abilene network (\S\ref{sec:evalabilene}) and GEANT network  (\S\ref{sec:evalgeant}). We compare our performance with \rthree{} and \FFC{} models. We also enumerate failure scenarios and apply MCF model on each to get the optimal value for comparison. Further, we show that \vn{}'s performance is stable with small number of tunnels even if we scale the network(\S\ref{sec:evalscale}). 

{\bf Topologies evaluated.}
We choose Abilene and GEANT topologies as our base topologies. Since we are evaluting edge-core networks, we make our base topologies as the core networks and then add edge nodes upon them. Each added edge node is connected with two random core nodes. We use the gravity model~\cite{gravity_model} to generate traffic matrices with MLU in the range [0.6, 0.7] across the topologies. And the traffic demand is only between edge nodes. We use uniform capacities on Abilene and GEANT has link capacity ranging from 1 to 100 Gbps. As for added links(between edge nodes and core nodes), we make their capacity large enough to avoid being the bottleneck so that we can focus on the base topologies. We model link failure as link being completely down and losing all capacity. We consider normal scenario where no link is down, 1 link failure scenarios and 2 simultaneous link failures scenarios throughout all our experiments. We evaluate the worst-case performance in the target set of failure scenarios and use both of MLU and overall throughput as the metrics.

{\bf Tunnel selection.}
Since \FFC{} is a tunnel-based routing scheme, we also need to provide tunnels to it. We provide the same tunnels to \vn{} because without tunnels, \vn{} will become \rthree{}. We provide 3 tunnels for every source-destination pair in order to handle 2 simultaneous link failures. We use a simple method to generate tunnels. For each source-destination pair, we generate all possible simple paths and try to find 3 disjoint tunnels. If there exist 3 disjoint tunnels, we make sure that the shortest tunnel is as short as possible. Given that, we make sure the second tunnel is as short as possible, and then the third one is as short as possible. If we can't find 3 disjoint tunnels, we will search 2 disjoint tunnels, and use the same scheme to pick the shortest two tunnels. Then we pick the shortest one in the remaining tunnels as the third tunnel, which may not be completely disjoint with the first two. In all of our experiments, two disjoint tunnels always exist and there are more than 3 different tunnels for all source-destination pairs. So this scheme is guaranteed to be able to generate 3 tunnels.

\subsection{Abilene topology}\label{sec:evalabilene}

Abilene topology has 11 nodes and 14 edges. We add 11 additional nodes as edge nodes and use the method described above to generate an edge-core network using the original Abilene as the core network. We repeat the same procedure to randomly generate 5 different networks and 5 different traffic matrices, and carry out the same evaluation.\cj{How do we display the result of different random topologies? Do we just pick one?} Table~\ref{tab:abilenemlu} and Table~\ref{tab:abilenethroughput} show one of the 5 sets of results. From the result, we find that it is hard to predict whether \rthree{} or \FFC{} is better in different topologies. Even in the same topology, \rthree{} and \FFC{} can beat each other under different scenarios. In this example, \FFC{} doesn't match the optimal even when there is no failure and is also the worst when there is 1 link failure. \rthree{} matches the optimal when $F=0$ and $F=1$. But it becomes extremely bad when $F=2$, even worse than \FFC{}. However, \vn{} can consistently perform as well as, if not better than, the best of \rthree{} and \FFC{}. Under 2 simultaneous failures, \vn{} can beats  \rthree{} and \FFC{}, and is closer to the optimal value.

\subsection{GEANT topology}\label{sec:evalgeant}

GEANT topology has 32 nodes and 50 edges. We add 16 additional edge nodes into the topology. We also randomly generate 5 different edge-core networks. In all 5 experiments, neither \rthree{} or \FFC{} can match the optimal even with only 1 link failure. Under 2 failures, \rthree{} gives MLU of infinity. Though \FFC{} can give real numbers, they are way off the optimal values. \vn{}, however, always matches the optimal MLU. As for the metric of overall throughput, the best of \rthree{} and \FFC{} can only serve around or less than 50\% of the optimal. \vn{} can always serve more than 85\% of the optimal, beating the other two scheme by a large amount.

\subsection{Scaled topology}\label{sec:evalscale}

It's evident that providing more tunnels will improve the performance of tunnel-based schemes. In this section, we show that on more complicated topologeis, \vn{} doesn't need more tunnels to keep its performance stable. We still use GEANT topology as the base topology. Then we add 24 edge nodes, 32 edge nodes respectively to make larger edge-core networks, using the same schemes as above to randomly generate edges and traffic demands. We also use the same schemes to find 3 tunnels for each source-destination pair. From the result, we can see that \rthree{}'s results are stable. The gap between \rthree{}'s MLU result and optimal MLU is similar as in the smaller topology. And it can serve 40\%-50\% of optimal throughput under 2 failures, also similar as in the smaller topology. \vn{} is also relatively stable. It can serve almost the same traffic as the optimal throughput under 1 failure, and can serve more than 85\% of the optimal under 2 failures. However, the gap between \FFC{} and optimal value becomes much larger on larger networks. \FFC{}'s MLU can be 40-50 times more than the optimal MLU on large networks. And it is around 10 times more than the optimal MLU on smaller network. This indicates that more tunnels should be provided to \FFC{} for larger networks. 

==> zffc.tex <==
\subsection{Analysis of FFC}\label{sec:analysisffc}

%\textbf{Include figure to show FFC problem. Note this will get solved by FFC-improved. Discussion question: should we show something that even FFC-improved has a problem?}

\cj{arbitrarily bad example needed here.}

On the other hand, \FFC{}~\cite{ffc_sigcomm14}, a path protection scheme, allows making decision earlier at the source of a tunnel when a link on this tunnel fails. But \FFC{} needs to pre-allocate link capacity to tunnels, and only make decision at the source nodes of flows, and only allows the source of a flow to make routing decision. Figure~\ref{fig:ffc_example} shows a topology with 6 tunnels from $S$ to $T$. 3 tunnels are connected by 2 intermediate nodes, and the other 3 are connected by 3 intermediate nodes with a common node $7$. In order to send 1 unit of traffic from $S$ to $T$ under at most 2 link failures, we can use a simple policy based on whether link $S-7$ is alive. If $S-7$ is alive, we can send 0.5 traffic using first 3 tunnels, and send 0.5 traffic using last 3 tunnels. Note that under any failure scenario where $S-7$ is alive and at most 2 other links fail, this is always achievable. If $S-7$ is dead, at most 1 other link can fail. We can always send 1 traffic using first 3 tunnels. However, \FFC{} can not plan such policy. \FFC{} needs to pre-allocate the capacity to last 3 tunnels. Since they all share the same link $S-7$, the minimal of the 3 tunnels can at most get $1/6$ capacity. When $S-7$ is alive, 2 of last 3 tunnels may die due to 2 link failures, leaving only $1/6$ capacity in the worst case. 2 of first 3 tunnels can also be dead due to 2 link failures, leaving at most $0.5$ capacity. So in total, at most $2/3$ traffic can be guaranteed, which is $1/3$ less than the optimal. 

When modeling failures in \FFC{}, the authors assume that no more than $p$ tunnels for each source-destination pair have a common point of failure. Then under $f$ link or node failures, it simply uses $fp$ to bound the number of simultaneous tunnel failures on the topology, and computes routing to prepare for any $fp$ tunnel failures. Suppose $y_l$ is the variable indicating if tunnel $l$ fails. \FFC{} bounds $y_l$ by

\begin{align}
\begin{split}
& \sum_{l}y_{l} \le fp\\
\end{split}
\end{align}

Though this method is simple, it is also conservative since not all link failures will cause $p$ tunnels to fail. In \FFC{}, all $fp$ tunnel failure combinations will be considered and it needs to prepare for the worst-case among them. However, it is likely that not all failure combinations will be caused by $f$ link failures. $f$ link failures might not even cause $fp$ tunnel failures in any case. And by modeling failures this way, \FFC{} is not monotonic of tunnels. That is, providing more tunnels may result in worse performance. Because adding tunnels may increase $p$, hence force \FFC{} model to prepare for worse scenarios. Figure~\ref{fig:ffc_example} shows an simple topology where \FFC{} is not monotonic. In this example, with 3 tunnels $S-1-T$, $S-2-T$ and $S-3-4-T$, \FFC{} can send 2 unit of traffic from $S$ to $T$ under any one link failure and can send 1 unit of traffic under any two simultaneous links failure, which is the optimal. However, if we add another tunnel $S-5-3-4-T$, \FFC{} will perform worse with these 4 tunnels. Note that $S-3-4-T$ and $S-5-3-4-T$ share links. So $p$ increases from 1 to 2 after adding tunnel $S-5-3-4-T$. Under 1 link failure, \FFC{} will prepare for failure of simultaneous $fp$ tunnels, which is 2 tunnels in this case. The worst of 2 simultaneous tunnels failure is $S-1-T$ and $S-2-T$ both failing, and leaving 1 unit of capacity from $S$ to $T$. Similarly, under 2 links failure, \FFC{} will prepare for failure of simultaneous 4 tunnels, which is failure of all tunnels, leaving no capacity from $S$ to $T$. Non-monotonicity not only affects the performance, but also brings difficulty in designing tunnels. In Section~\ref{sec:vnmodel}, we propose a better modeling for tunnel failures, which can improve \FFC{} to be a monotonic model.

%In \FFC{}, they also require that, upon failure, the source diverts the traffic from failed paths to other operational paths. This diversion of traffic is done so that, on the operational paths, the relative ratio of similar traffic is preserved. To ensure such re-routing remains feasible, FFC\cite{ffc_sigcomm14} reserves sufficient capacity along the tunnels. The reason such reservation is possible is that, given the assumption regarding common points of failure, at most a pre-determined number of tunnels can fail under any $f$ simultaneous edge or node failures.
%Unfortunately, the approach assumes that with each failure, the number of tunnels that fail are as many as the maximum number of tunnels with a common point of failure, a gross over-estimate. Consequently, the traffic that can be admitted by FFC is likely much more conservative than necessary. 
%Finally,~\cite{DRCN14} does not tackle node failures, but addresses link failures
%by adding edges to the network. The original excess capacity of the network is not used, and the number of edges added may be substantial.

\begin{table}[t]
  \small
    \centering
    \begin{tabular}{||c c c c c||} 
    \hline
    Network & failure & FFC & R3 & Optimal\\ 
    \hline\hline
    Fig.1 & f=1 & 0.5 & 0.5 & 0.5\\  
    Fig.1 & f=2 & 1 & inf & 1\\ 
    Fig.2 & f=1 & 1 & 0.5 & 0.5\\  
    Fig.2 & f=2 & inf & inf & 1\\ 
    \hline
    \end{tabular}
    \caption{Comparison between FFC, R3 and the optimal MLU on the toy topology examples.}
    \label{tab:ffc_r3}
    \vspace{-0.4in}
\end{table}

%\subsection{Analysis of a new example}\label{sec:analysisffc}

%Figure~\ref{fig:new_example} shows another example by adding a node to the first toy example presented in Figure~\ref{fig:r3_example}. It's obvious that R3 will fail under 2 failures for the same reason in Figure~\ref{fig:r3_example}. FFC's performance, however, depends on the tunnel selection. We need at least 4 tunnels to full-utilize the network, which means using any 3 or less tunnels can't achieve optimal even when there is no failure. If we select 4 tunnels, then at least 2 tunnels will share a link. Then under 2 link failures, FFC will prepare for 4 tunnel failures, which will prevent any flow to pass. Note that if we choose 3 tunnels as in Figure~\ref{fig:r3_example}'s example, though it will not achieve optimal, it will allow some traffic to flow under 2 failures. This shows that FFC is not monotonic on tunnels. That is, by adding tunnels, the performance might be even worse.  

\subsection{Comparison on the toy examples}
Table~\ref{tab:ffc_r3} shows the comparison of MLU achieved from FFC and R3, and the optimal MLU. In the first toy topology with 1 link failure, FFC and R3 can both achieve the optimal MLU. With 2 link failures, FFC is doing well while R3 gives MLU of infinity because under 2 failures, no link bypass can be guaranteed. In the second toy topology, R3 is working well with 1 link failure while FFC is sub-optimal because its estimate of the tunnel failures is conservative. With 2 link failures, both FFC and R3 give MLU of infinity.  The first observation here is that it is hard to predict whether FFC or R3 will perform better. There is a case where FFC beats R3. And there is also a case where R3 beats FFC. The other observation is that even the best of these two schemes can be sub-optimal, which is shown in the second toy topology with 2 link failures.


\textbf{Understanding intrinsic capability of network.}
The lack of a clear benchmark for comparison is a key challenge in using existing response mechanisms. For instance, consider FFC. If it is unable to reserve sufficient bandwidth to guarantee that critical traffic can withstand failures, it remains unclear whether the inability was due to poor tunnel choice, over-estimation of failed capacity on the tunnels, an artifact of path protection which only allows the source to reroute traffic, or owing to the restriction that traffic is merely rescaled on unimpacted tunnels. 
Comparing the ability of each devised scheme to an intrinsic measure of network 
performance capability will provide a firm basis to guide the choice of response 
mechanisms and to understand the value of any proposed changes to them.


\subsection{Model tunnel failures}\label{sec:vnmodel}
Compare to \FFC{}, we use a more accurate way to model tunnel failures and draw the connection between link failures and tunnel failures directly. Suppose $x_e$ is the variable indicating if link $e$ fails, we model $y_l$ by 

\begin{align}
\begin{split}
& \sum_{e \in E} x_e \le f \\
& x_e - y_l \le 0 \quad \forall l, e \in l \\
& y_l - \sum_{e \in l} x_e \le 0 \quad \forall l  \\
\end{split}\label{eq:tunnel_model}
\end{align}

The first constraint bounds the maximum number of simultaneous link failures. The second ensures that any failed underlying link of a tunnel will cause the tunnel to fail. The third ensures that a tunnel only fails when at least one underlying link fails. This set of constraints equations depict the exact connection between link failures and tunnel failures, thus it will eliminate the gap caused by conservative estimation of tunnel failures in \FFC{}. Note that we can easily add node failures into this following the same idea. But we only focus on link failures in this work.

We will show in \S\ref{sec:evaluation} that the tunnel-based routing scheme in \FFC{} can achieve better performance by improving the tunnel failure modeling as above. But even if we improve \FFC{} by adopting this better way to model tunnel failures, it still can only send traffic on the provided tunnels and doesn't have the flexibility to freely exploit the topology as in \rthree{}. \vn{}, however, allows link-based routing. Thus, it can provide much more flexibility.

\subsection{Theoretical results}
\begin{itemize}
    \item FFC-improved beats FFC
    \item FFC-improved is monotonic
\end{itemize}


==> zmotivation.tex <==
\section{Background and Motivation}
\label{sec:motivation}


\subsection{Background}
In the wide-area context, the common sources of failures are IP links, IP routers, and optical related failures~\cite{Sprint,OpticalfailuresIMC16,failures:sigcomm2010,failures:sigcomm2011}. The last two categories can simultaneously impact multiple links, and constitute a Shared Risk Link Group (SRLG) \cite{JenSigmetrics11,Sprint}.

In MPLS settings, two classes of recovery mechanisms have been explored~\cite{MPLSReroute}.
In a \emph{link-based protection} scheme, upon the failure of a link $l$, traffic previously on $l$ is rerouted along pre-computed detour paths that do not include $l$. In a \emph{path-based protection} scheme, backup paths are calculated in advance for traffic from each source $s$ to every destination $t$, and when a particular path fails (e.g., an underlying link, or a node fails), the traffic is diverted to those back-up paths. R3 is representative of link-based. FFC is representative of path-based.

\textbf{Description of R3} 
R3~\cite{r3:sigcomm10} is a routing scheme which considers networks under $f$ simultaneous failures and attempts to produce a link-based protection mechanism to ensure that the network is congestion-free under all such failures. The essential idea is to build a bypass for each link which will be used when that link fails. The way it models this, is to have a base routing to specify how the network routes the traffic under no failures, and to have a protection routing to reserve some bypass capacity for each link. When a link fails, the bypass for the failed link will be triggered to take over the traffic. To implement this scheme, each router will be installed with the base routing along with the protection routing, which is a compact expression of how it should adapt to failures under all scenarios the model solves. When the router detects a failure, it will compute an updated routing based on its current routing and its protection routing for the failed link.



\textbf{Description of FFC} FFC~\cite{ffc_sigcomm14} is a path-based routing scheme which computes the bandwidth allocated to each tunnel in order to maximize the throughput on the network under $k_e$ simultaneous link failures and $k_v$ simultaneous switch failures. FFC model needs to know the max number of tunnels traversing a common link, and the max number of tunnels traversing a common switch. Based on this information, FFC will pre-compute the max number of simultaneous tunnel failures. Then it solves an optimization problem to plan the tunnel routing so that the throughput will be maximized in the worst tunnel failure case. When a link or a switch fails, the router will detect the failed tunnels and normalize the allocated bandwidth to the alive tunnels so that the ratios between them will not change.


\begin{figure}[t]
	\centering
        \includegraphics[trim={0 4cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/r3_example_1.png}
        \label{fig:r3_example_1}
    
        \includegraphics[trim={0 3cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/r3_example_2.png}
        \label{fig:r3_example_2}

    \caption{Examples that cannot be handled by R3~\cite{r3:sigcomm10}, or performance is poor.
        }
    \label{fig:r3_example}
\end{figure}
\subsection{Analysis of R3}\label{sec:analysisr3}
Unfortunately, as we will illustrate, R3 is unable to handle various commonly occurring failure scenarios such as node failures and certain kinds of link failures. With R3, the end point of a failed link will use a bypass to reroute the traffic which is originally on the failed link. The key limitation of R3 is that only the end point of a failed link can reroute traffic. And the rerouted traffic has to go to the other end point of the failed link. R3 doesn't provide the flexibility to make the reroute decision earlier, or to reroute to other nodes. In the topology shown in Figure~\ref{fig:r3_example}, if any two links fail, it is feasible to route the traffic from the source $s$ to the destination $t$ without exceeding any link capacities. Nevertheless, under such failures, R3 fails to deliver the $s-t$ traffic. More specifically, R3 is unable to protect against the simultaneous failures of links $l_1$ and $l_2$ since, when these links fail, there are no viable bypass paths for either of the links. Because a bypass for $l_1$ has to start at $s$ and end at $5$, and a bypass for $l_2$ has to start at $5$ and end at $6$. Instead, an obvious feasible strategy is to route the traffic along the path $s-3-4-t$, an option that is not considered by R3 because $t$ is not an end point of either $l_1$ or $l_2$.

Figure~\ref{fig:r3_example} presents another challenging example on an edge-core network (common in ISP settings), where R3 was adapted to meet the requirement that an edge node only receives traffic destined to itself. While it is easy to protect against a single link failure by using whichever path among $s-m-n-t$ or $s-i-j-t$ survives, R3 routes traffic as shown in the figure and results in an MLU (Maximum Link Utilization, or utilization of most congested link) of $5$. For the same reason stated above, when link $l$ fails, $i$ is the only node to make the reroute decision, and the reroute traffic has to go to $j$. To meet the edge-core network requirement, $i$ can only bypass traffic along the path $i-m-n-j$, thereby exceeding the capacity of links $l_1$ and $l_2$. If a reroute decision can be made earlier at source node $s$ and doesn't need to go through either $i$ or $j$, a better path $s-m-n-t$ may be found to protect the failure. We remark that these deficiencies in R3 are largely unknown in the literature.

%To understand why, it helps to realize that R3 does not distinguish bypass traffic based on its source and, therefore, when $l$ fails, it bypasses all its traffic along the path $i-m-n-j$, thereby exceeding the capacity of links $l_1$ and $l_2$. We remark that these deficiencies in R3 are largely unknown in the literature.


\begin{figure}[t]
	\centering
        
	    \includegraphics[trim={0 0.4cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/ffcexample2.png}
        \label{fig:ffc_example2}
        
        \includegraphics[trim={0 0.2cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/ffc_shared.png}
        \label{fig:ffc_shared}
        
        \includegraphics[trim={0 0.2cm 0cm 0cm}, clip, width=0.48\textwidth]{figures/ffcexample.png}
        \label{fig:ffc_example}
        
    \caption{Examples that FFC~\cite{ffc_sigcomm14} performs poorly on.
        }
        \label{fig:ffc_example}
\end{figure}

%\begin{figure}[t]
%	\centering
%        \includegraphics[trim={8cm 10.5cm 10cm 7cm}, clip, width=0.48\textwidth]{figures/soph_example.pdf}

%    \caption{An example that both \FFC{}~\cite{ffc_sigcomm14} and R3~\cite{r3:sigcomm10} perform poorly on. All solid edges have capacity of 1 and all dotted edges have capacity of 0.5.
%        }
%    \label{fig:new_example}
%\end{figure}



\subsection{Analysis of FFC}\label{sec:analysisffc}

%\textbf{Include figure to show FFC problem. Note this will get solved by FFC-improved. Discussion question: should we show something that even FFC-improved has a problem?}

\cj{arbitrarily bad example needed here.}

On the other hand, \FFC{}~\cite{ffc_sigcomm14}, a path protection scheme, allows making decision earlier at the source of a tunnel when a link on this tunnel fails. Thus, it can prevent the issues of  R3 illustrated above. In examples in Figure~\ref{fig:r3_example}, \FFC{} can simply bypass the failed links using other alive tunnels. But \FFC{} needs to pre-allocate link capacity to tunnels, and only make decision at the source nodes of flows, and only allows the source of a flow to make routing decision. Figure~\ref{fig:ffc_example} shows a topology with 6 tunnels from $S$ to $T$. 3 tunnels are connected by 2 intermediate nodes, and the other 3 are connected by 3 intermediate nodes with a common node $7$. In order to send 1 unit of traffic from $S$ to $T$ under at most 2 link failures, we can use a simple policy based on whether link $S-7$ is alive. If $S-7$ is alive, we can send 0.5 traffic using first 3 tunnels, and send 0.5 traffic using last 3 tunnels. Note that under any failure scenario where $S-7$ is alive and at most 2 other links fail, this is always achievable. If $S-7$ is dead, at most 1 other link can fail. We can always send 1 traffic using first 3 tunnels. However, \FFC{} can not plan such policy. \FFC{} needs to pre-allocate the capacity to last 3 tunnels. Since they all share the same link $S-7$, the minimal of the 3 tunnels can at most get $1/6$ capacity. When $S-7$ is alive, 2 of last 3 tunnels may die due to 2 link failures, leaving only $1/6$ capacity in the worst case. 2 of first 3 tunnels can also be dead due to 2 link failures, leaving at most $0.5$ capacity. So in total, at most $2/3$ traffic can be guaranteed, which is $1/3$ less than the optimal. 

When modeling failures in \FFC{}, the authors assume that no more than $p$ tunnels for each source-destination pair have a common point of failure. Then under $f$ link or node failures, it simply uses $fp$ to bound the number of simultaneous tunnel failures on the topology, and computes routing to prepare for any $fp$ tunnel failures. Suppose $y_l$ is the variable indicating if tunnel $l$ fails. \FFC{} bounds $y_l$ by

\begin{align}
\begin{split}
& \sum_{l}y_{l} \le fp\\
\end{split}
\end{align}

Though this method is simple, it is also conservative since not all link failures will cause $p$ tunnels to fail. In \FFC{}, all $fp$ tunnel failure combinations will be considered and it needs to prepare for the worst-case among them. However, it is likely that not all failure combinations will be caused by $f$ link failures. $f$ link failures might not even cause $fp$ tunnel failures in any case. And by modeling failures this way, \FFC{} is not monotonic of tunnels. That is, providing more tunnels may result in worse performance. Because adding tunnels may increase $p$, hence force \FFC{} model to prepare for worse scenarios. Figure~\ref{fig:ffc_example} shows an simple topology where \FFC{} is not monotonic. In this example, with 3 tunnels $S-1-T$, $S-2-T$ and $S-3-4-T$, \FFC{} can send 2 unit of traffic from $S$ to $T$ under any one link failure and can send 1 unit of traffic under any two simultaneous links failure, which is the optimal. However, if we add another tunnel $S-5-3-4-T$, \FFC{} will perform worse with these 4 tunnels. Note that $S-3-4-T$ and $S-5-3-4-T$ share links. So $p$ increases from 1 to 2 after adding tunnel $S-5-3-4-T$. Under 1 link failure, \FFC{} will prepare for failure of simultaneous $fp$ tunnels, which is 2 tunnels in this case. The worst of 2 simultaneous tunnels failure is $S-1-T$ and $S-2-T$ both failing, and leaving 1 unit of capacity from $S$ to $T$. Similarly, under 2 links failure, \FFC{} will prepare for failure of simultaneous 4 tunnels, which is failure of all tunnels, leaving no capacity from $S$ to $T$. Non-monotonicity not only affects the performance, but also brings difficulty in designing tunnels. In Section~\ref{sec:vnmodel}, we propose a better modeling for tunnel failures, which can improve \FFC{} to be a monotonic model.

%In \FFC{}, they also require that, upon failure, the source diverts the traffic from failed paths to other operational paths. This diversion of traffic is done so that, on the operational paths, the relative ratio of similar traffic is preserved. To ensure such re-routing remains feasible, FFC\cite{ffc_sigcomm14} reserves sufficient capacity along the tunnels. The reason such reservation is possible is that, given the assumption regarding common points of failure, at most a pre-determined number of tunnels can fail under any $f$ simultaneous edge or node failures.
%Unfortunately, the approach assumes that with each failure, the number of tunnels that fail are as many as the maximum number of tunnels with a common point of failure, a gross over-estimate. Consequently, the traffic that can be admitted by FFC is likely much more conservative than necessary. 
%Finally,~\cite{DRCN14} does not tackle node failures, but addresses link failures
%by adding edges to the network. The original excess capacity of the network is not used, and the number of edges added may be substantial.

\begin{table}[t]
  \small
    \centering
    \begin{tabular}{||c c c c c||} 
    \hline
    Network & failure & FFC & R3 & Optimal\\ 
    \hline\hline
    Fig.1 & f=1 & 0.5 & 0.5 & 0.5\\  
    Fig.1 & f=2 & 1 & inf & 1\\ 
    Fig.2 & f=1 & 1 & 0.5 & 0.5\\  
    Fig.2 & f=2 & inf & inf & 1\\ 
    \hline
    \end{tabular}
    \caption{Comparison between FFC, R3 and the optimal MLU on the toy topology examples.}
    \label{tab:ffc_r3}
    \vspace{-0.4in}
\end{table}

%\subsection{Analysis of a new example}\label{sec:analysisffc}

%Figure~\ref{fig:new_example} shows another example by adding a node to the first toy example presented in Figure~\ref{fig:r3_example}. It's obvious that R3 will fail under 2 failures for the same reason in Figure~\ref{fig:r3_example}. FFC's performance, however, depends on the tunnel selection. We need at least 4 tunnels to full-utilize the network, which means using any 3 or less tunnels can't achieve optimal even when there is no failure. If we select 4 tunnels, then at least 2 tunnels will share a link. Then under 2 link failures, FFC will prepare for 4 tunnel failures, which will prevent any flow to pass. Note that if we choose 3 tunnels as in Figure~\ref{fig:r3_example}'s example, though it will not achieve optimal, it will allow some traffic to flow under 2 failures. This shows that FFC is not monotonic on tunnels. That is, by adding tunnels, the performance might be even worse.  

\subsection{Comparison on the toy examples}
Table~\ref{tab:ffc_r3} shows the comparison of MLU achieved from FFC and R3, and the optimal MLU. In the first toy topology with 1 link failure, FFC and R3 can both achieve the optimal MLU. With 2 link failures, FFC is doing well while R3 gives MLU of infinity because under 2 failures, no link bypass can be guaranteed. In the second toy topology, R3 is working well with 1 link failure while FFC is sub-optimal because its estimate of the tunnel failures is conservative. With 2 link failures, both FFC and R3 give MLU of infinity.  The first observation here is that it is hard to predict whether FFC or R3 will perform better. There is a case where FFC beats R3. And there is also a case where R3 beats FFC. The other observation is that even the best of these two schemes can be sub-optimal, which is shown in the second toy topology with 2 link failures.

\subsection{Likey cut or use as needed}
\sgr{Not sure we need paragraphs below.. keeping for now.}
\textbf{Exploiting new forms of flexibility in network response.}
While R3 and FFC consider two specific ways in which networks respond to failures,
networks increasingly respond in more flexible ways, further facilitated
by the emergence of SDNs~\cite{b4,swan,ATTNetworkWorld,ATTGagan} which allow architects more explicit control on how traffic is managed. For instance, FFC considers a restricted response mechanism where the source diverts the traffic from failed paths to other operational paths while preserving the relative ratio of traffic on operational paths. However, recent work from Facebook~\cite{semi_oblivious_nsdi18} offers a viable alternative, where the the split of traffic across unimpacted tunnels is adjusted more flexibly than merely rescaling the flows. Likewise, our discussions with practitioners suggests that, in large-scale geographically distributed networks, path protection schemes such as FFC can incur a large response time to react to failure, since failure information must propagate to the source. R3 is similarly restrictive in that link bypass paths do not protect against node failures, whereas a more flexible response mechanism may easily provide such a protection. For instance, when a  node $i$ fails, the preceding node $j$ may quickly realize the failure and re-route the traffic along alternate paths. The flow adjustment can occur before the rest of the network learns about the failure and, thus, the recovery may be quicker than that using a path-based recovery scheme. In general, designing ways to exploit such flexibility in network response to failures is an open area of investigation.

\textbf{Understanding intrinsic capability of network.}
The lack of a clear benchmark for comparison is a key challenge in using existing response mechanisms. For instance, consider FFC. If it is unable to reserve sufficient bandwidth to guarantee that critical traffic can withstand failures, it remains unclear whether the inability was due to poor tunnel choice, over-estimation of failed capacity on the tunnels, an artifact of path protection which only allows the source to reroute traffic, or owing to the restriction that traffic is merely rescaled on unimpacted tunnels. 
Comparing the ability of each devised scheme to an intrinsic measure of network 
performance capability will provide a firm basis to guide the choice of response 
mechanisms and to understand the value of any proposed changes to them.












==> zoverview.tex <==
\section{Design Overview}
In order to improve the existing tunnel-based routing scheme, we start from the insight of weakness in FFC and make a new routing design which can handle the issues in FFC.

\subsection{Tunnel splitting}

One of the reasons why FFC is not able to handle the example in Figure~\ref{fig:ffc_example} is that FFC can not distinguish the shared part among tunnels. Hence when it is doing reservation, it has to reserve the shared part multiple times in order to allocate to different tunnels, leading to a capacity bottleneck. For example, in Figure~\ref{fig:ffc_example}, link $S-7$ is a shared link for 3 tunnels. In FFC model, all these three tunnels are competing the capacity in $S-7$, resulting in a lower utilization. Our solution for this issue is to split the tunnels. More specifically in this example, we can split the 3 tunnels into a short tunnel from $S$ to $7$, and 3 tunnels from $7$ to $T$. In this way, tunnels will not compete for capacity in link $S-7$ anymore. If there is any traffic going from $S$ to $7$, $7$ will decide which tunnels to use instead of letting $S$ decide. Note that comparing to FFC, this is not simply changing the provided tunnels. It is fundamentally different from FFC because FFC only allows tunnels from the source of a flow to the destination of flow. Here, we will not pose any limitation on how the tunnels will be used.

\subsection{Conditional reservation}
Unfortunately, isolating shared part in tunnels is not enough to handle the example in Figure~\ref{fig:ffc_example}. The main reason is that under 2 simultaneous link failures, we can't guarantee capacity from $S$ to $7$ with only one path to send the traffic. Thus, we are not able to utilize the new tunneling. However, the capacity from $S$ to $7$ is not always needed. As in the policy mentioned in  \S\ref{sec:analysisffc}, if $S-7$ dies, the 3 tunnels without involving $7$ can handle the traffic. We only need the other 3 tunnels when $S-7$ is alive. In other words, we only need to send traffic from $S$ to $7$ when $S-7$ is alive. To achieve this, we are introducing conditional reservation which provides richer flexibility in routing. A conditional reservation means we require a certain amount of capacity only when the associated condition is satisfied. And we also only use it when the same condition is true. In the example in Figure~\ref{fig:ffc_example}, we can make conditional reservation from $S$ to $7$ with the condition being that $S-7$ is alive. Similarly, we can make a conditional reservation from $7$ to $T$ with the same condition. With the associated condition being satisfied, enough capacity can be reserved so that the throughput on the network will met the optimal.



==> zpractical.tex <==
\section{Deriving practical routing schemes(old text)}\label{sec:practical}

In \S\ref{sec:system}, we introduced our \System{} and how we can generalize the model to provide more flexibility in routing hence to give better performance guarantee. Next, we will illustrate how to practically implement routing schemes obtained from our model. 

We claim that (i) with help of a controller, our generalized model can be implemented as a centralized routing scheme which only needs to solve a linear system upon any link failure; (ii) with an additional assumption on the choice of \LS{}s, our \LS{} model can be implemented as a distributed routing scheme which does proportional assigning traffic just as FFC does.  

%\begin{itemize}
%    \item Proposition: Solving the general case involves solving a linear system globally
%and reinstall the rules.
%    \item Theorem: (Harder): Need to show that the solution of the linear system is between 0 and 1.
%    \item Centralized, but linear system is quick to solve Discuss results below that show distributed possible.
%\end{itemize}

\subsection{Centralized routing by solving linear systems}

In this centralized scheme, upon the update on the failure scenario(initialization, link failure, link recovery), we need a controller to recompute the weights and reinstall the weights in the routers. We claim that the recomputation only requires solving $|V|^2$ linear systems with $|V|^2$ variables and $|V|^2$ equations. A linear system only contains equations, which is usually much less complicated to solve than an LP with similar size. Thus, the update of routing weight can be much faster comparing to update by solving an LP.

Upon failure scenario $x$, let $T_x(s,t)$ denote the set of alive tunnels from $s$ to $t$, $W_x(s,t)$ denote the set of active virtual flow from $s$ to $t$ and $R_x(s,t)$ denote the amount of capacity available to transmit traffic from $s$ to $t$. Then we have $R_x(s,t) = \sum_{l \in T_x(s,t)} a_{l} + \sum_{w \in W_x(s,t)}b_{w}$. Suppose $\forall s,t \in V$, we actually use $u(s,t)$ fraction of $R(s,t)$ for routing, and all available tunnels and \LS{}s are used proportionally according to to their reservation. Then to make the used capacity match the traffic going through, we will have $u(s,t)R(s,t) = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(st)u(s',t') + z_{st}d_{st}$. Thus, we can write a linear system as
\begin{align}
\begin{split}
& \quad u(s,t)\big(\sum_{l \in T_x(s,t)} a_{l} + \sum_{w \in W_x(s,t)}b_{w} \big) \\
& = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(st)u(s',t') + z_{st}d_{st} \quad \forall s,t \in V
\end{split}\label{eq:linear_system_vf}
\end{align}
where $u(s,t)$ are the variables.

If there exists a solution $u^*(s,t)$ to this linear system and $\forall s,t \in V, u^*(s,t) \in [0,1]$, then $\forall l \in T_x(s,t)$, $u^*(s,t)a_l$ is the amount of traffic that will be carried by tunnel $l$. And we can prove that with the capacity constraint \eqref{eq:vn_capacity_constraint} being satisfied, such solution always exists.

\begin{proposition}\label{prop:linear_system}
There always exists a solution $u^*(s,t)$ to the linear system in \eqref{eq:linear_system_vf} which can be converted to a valid routing.
\end{proposition} \cj{proof needed here} \cj{proof sketch, appendix for details}

In \System{}, a tunnel from $s$ to $t$ can be used to route traffic for other source-destination pairs. So we solve similar linear systems, one for each demand entry $d_{\bar{s}\bar{t}}$. That is, $\forall \bar{s}, \bar{t} \in V$, we solve a linear system which only accounts for the demand from $\bar{s}$ to $\bar{t}$. And the linear system is
\begin{align}
\begin{split}
& \quad u_{\bar{s}\bar{t}}(\bar{s},\bar{t})\big(\sum_{l \in T_x(\bar{s},\bar{t})} a_{l} + \sum_{w \in W_x(\bar{s},\bar{t})}b_{w} \big) \\
& = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(\bar{s}\bar{t})u_{\bar{s}\bar{t}}(s',t') + z_{\bar{s}\bar{t}}d_{\bar{s}\bar{t}} \\ 
& \quad u_{\bar{s}\bar{t}}(s,t)\big(\sum_{l \in T_x(s,t)} a_{l} + \sum_{w \in W_x(s,t)}b_{w} \big) \\
& = \sum_{s',t' \in V,w' \in W_x(s',t')} p_{w'}(st)u_{\bar{s}\bar{t}}(s',t')  \quad \forall s,t \in V, (s, t) \ne (\bar{s}, \bar{t})
\end{split}\label{eq:linear_system_vf_single}
\end{align}

$\forall l \in T_x(s,t)$, $u^*_{\bar{s}\bar{t}}(s,t)a_l$ is the amount of traffic from $\bar{s}$ to $\bar{t}$ that will be carried by tunnel $l$, which is the weight needed to be installed in router $s$. Based on the same argument for above proposition, there always exists a solution $u^*_{\bar{s}\bar{t}}(s,t)$ to the linear system in \eqref{eq:linear_system_vf_single} such that $\forall s,t \in V, u^*_{\bar{s}\bar{t}}(s,t) \in [0,1]$. And it is obvious that $u^*(s,t) = \sum\limits_{\forall \bar{s},\bar{t} \in V} u^*_{\bar{s}\bar{t}}(s,t)$ is a solution to \eqref{eq:linear_system_vf}. So this routing is valid. 

\subsection{Distributed routing by proportionally assigning traffic}

FFC uses a distributed routing scheme. It installs the value of tunnel reservation($a_l$) as the weight in the source nodes of tunnels. On each scenario, FFC distributes traffic to the alive tunnels proportionally to the weights. It doesn't require help of a centralized controller. After the tunnel weights are installed, routers can adapt to failures by themselves. Our \FFCimp{}, which improves the failure model of FFC, clearly can use the same distributed routing strategy. Next, we will show that even our \System{}, under some assumption on the provided \LS{}s, can also use a similar distributed routing scheme. In this routing strategy, we need to install both the tunnel reservation($a_l$) and \LS{} reservation($b_q$) as the weight in the source nodes. Routers will then distribute traffic to the alive tunnels and alive \LS{} proportionally to the weights. \cj{not sure how to talk about it here...use an example? Do I say using labels?}

This routing strategy doesn't work for all \LS{} choices. Because we allow a \LS{} to use another \LS{} and hence the traffic might be distributed recursively. For example, suppose a \LS{} $q_1$ from $i_1$ to $j_1$ has a segment $i_2j_2$ in it, while a \LS{} $q_2$ from $i_2$ to $j_2$ has a segment $i_1j_1$ in it. Then traffic from $i_1$ to $j_1$ might be distributed to $q_1$, which will need to go through segment $i_2j_2$. When going from $i_2$ to $j_2$, $q_2$ might be chosen to be used, which will need to go through $i_1j_1$ and cause recursion. In order to make proportionally distributing scheme work, we need to choose \LS{}s so that such recursion will never occur. \cj{should we stick with the 'topological sort', or use something like 'cycle-free'? Not sure what's the best mathematical way to describe this. Right now I'm using relation and topological sort}
\cj{topological sort}

We define a relation '$>$' on $\langle V^2, V^2 \rangle$. If when routing from $i$ to $j$, it's possible to use a \LS{} which passes through segment $i'j'$, we say that $(i,j) > (i', j')$. More formally, if there exists $q \in L_b(i,j)$ such that $i'j'$ is a segment in $q$, we define that $(i,j) > (i',j')$. Now we claim that if \LS{}s are chosen in a way that $V^2$ can be topologically sorted on the '$>$' relation at each failure scenario, then the routing scheme described above can be deployed without recursion.

\begin{proposition}\label{prop:topological_assumption} Under the topologically sorted assumption, a local proportionally
distributed routing scheme similar to FFC scheme works for \LS{} model. 
\end{proposition}

\cj{proof needed here}

We find that some simple heuristics to choose \LS{}s can ensure topologically sorted assumption. For example, we can use the shortest path(segment) as the unconditional logical sequence for each source-destination pair. Then the assumption is satisfied under any failure scenario. \cj{do we need argument/proof here?} We will show in \S\ref{sec:evaluation} that using this set of \LS{}s can greatly improve the performance. Another way to ensure the assumption is to start with a more sophisticated set of \LS{}s which may violate the assumption. Then we can prune the set so that the remaining set makes $V^2$ able to be topologically sorted.





==> zpractical2.tex <==
\section{Deriving practical routing schemes}\label{sec:practical}

\subsection{Proportionally distributed in physical tunnels}

In \S\ref{sec:system}, we introduced our \System{} and how we can generalize the model to provide more flexibility in routing hence to give better performance guarantee. Next, we will illustrate how to practically implement routing schemes obtained from our model. 

Our \FFCimp{} can be implemented exactly as FFC's implementation because its improvement is in the better failure model while it has the same routing flexibility as FFC does. In FFC's implementation, it normalizes the values of tunnel reservations and install them as the weights in the source routers of tunnels. Under each failure scenario, source routers will rescale the traffic to
the alive tunnels in proportion to installed weights. For example, there are 3 tunnels from $s$ to $t$ and they get reservations of $(2,3,5)$ in the optimization. Then $(0.2, 0.3, 0.5)$ will be installed in $s$ as the weights of these tunnels. If the first tunnels fails, $s$ will split traffic sent to $t$ based on weights  $(0, \frac{0.3}{0.8}, \frac{0.5}{0.8})$.

\subsection{Proportionally distributed in \LS{}s}
\label{sec:local_LS_scheme}

  \begin{figure}[t]
	\centering
        
	    \includegraphics[ trim={6.7cm 6.2cm 12cm 5cm}, clip, width=0.45\textwidth]{figures/implementation_example2.pdf}
        \label{fig:implementation_example}

    \caption{A topology with 6 physical tunnels and two \LS{}s $L_1(AC,CD)$ and $L_2(AD,DB)$. The tables are installed in router A.}
        \label{fig:implementation_example}
\end{figure}

In the implementation of our \LS{} model, we start with the same idea of proportional distribution as in FFC. But we include \LS{}s in the distribution. Figure~\ref{fig:implementation_example} shows an example topology with \LS{}s and router $A$'s tables. When $A$ needs to send traffic to $B$, it will first looks up its table for $B$, which tells it the available paths are a physical tunnel $T_6$ and a \LS{} $L_2$ and it should split traffic equally. If it chooses $T_6$, the traffic will go through tunnel $T_6$ as in FFC. If it chooses $L_2$, the traffic will be sent though segments $AD$ and $DB$. The next hop table will tell that the next hop for $L_2$ is $D$. So it will need to again check the table for $D$, which shows the two ways to go to $D$ are $T_3$ and $L_1$ with equal weights. It will then split traffic between these two choices which will either send the traffic directly through $T_3$ to $D$, or use $L_1$ and eventually send through $T_1$ to $C$, the next hop of $L_2$. When the traffic on $L_2$ goes to $D$, $D$ will know from its table that the next hop of $L_2$ is $B$, and loop up paths to route to $B$. 

Note that, just as we model the \LS{}, we allow a logical sequence to use other logical sequences to route for its segments. So in this example, $L_1$ can be used to route $AD$ segment in $L_2$. As a result, even though we never provide a physical tunnel or a \LS{} as $A-C-D-B$, such routing can be achieved in our implementation. As in FFC's implementation, the installed weights of tunnels and \LS{}s are normalized values of reservations($a_l$ and $b_q$). The optimization model is solved at the beginning to achieve these values. After the weights are installed, under each scenario, a router will update its table to disable the failed tunnels and inactive \LS{}s, and renormalize the remaining weights. As described in \S\ref{sec:vs_model} and \S\ref{sec:ls_with_hint}, an unconditional  \LS{} is always active and a conditional \LS{} will be inactive when the attached hint is not satisfied under current scenario.

\subsection{Recursion in routing}
%mutually dependent
The above routing scheme of proportional distribution will not add much extra complexity in implementation other than what is already in FFC's implementation. However, for some choices of \LS{}s, it may cause recursion in routing. Suppose we have an additional \LS{} $L_3$ from $D$ to $B$ which goes through segments $DA$ and $AB$. Routing from $A$ to $B$ will follow the same strategy as described above. When $L_2$ is chosen as the routing path, the traffic will go through segment $DB$. When $D$ tries to route send to $B$, it will choose from available paths to $B$ including $L_3$. However, if $L_3$ is chosen, it will again need to go through segment $AB$ and cause recursion.

Theoretically, since the traffic will also be split into other tunnels, the traffic which goes into recursion will be less and less. When this procedure repeats, it will eventually converges to the state where all the traffic is sent through. But this is not desirable in the practical routing. So here, (i) we derive the condition under which the proportional distribution scheme will not cause recursion and (ii) we propose a routing scheme with help of a centralized controller for more general cases.

Note that no matter how traffic is routed on the \LS{}s, it will eventually go to some physical tunnels. If we know how much traffic each physical tunnel will eventually carry in order to serve the traffic demand, then we can directly deploy the routing without going through \LS{}s. In the \LS{} model, we make reservations on tunnels and \LS{}s so that the reservations are sufficient to handle the traffic for a set of failure scenarios. Now, in a particular scenario $x$, we need to figure out exactly how much reservation we are using. Let $T_x(s,t)$ denote the set of alive tunnels from $s$ to $t$ and $L_x(s,t)$ denote the set of active \LS{}s from $s$ to $t$. We can describe the reservations in a matrix $Mat \in \mathbb{R}^{P \times P}$, where $P$ is the set of node pairs of interest. Each row stands for how a node pair $ij$ services all the needs on it. The diagonal of $Mat$ is the sum of available reservations on the pair, i.e. $Mat_{ij, ij} = \sum_{l \in T_x(i,j)} a_{l} + \sum_{q \in L_x(i,j)}b_{q}$. And other entries of $Mat$ denote how much a node pair needs to carry for other node pairs, i.e. $Mat_{ij, mn} = -\sum_{q \in \tau(i,j) \cap L_x(m,n)} b_{q}$ if $(i,j) \ne (m,n)$. For example, the matrix for the topology in Figure~\ref{fig:implementation_example} can be written as

\begin{align}
\begin{split}
& Mat_{1} = 
\begin{blockarray}{ccccccc}
AC & CD & AD & DA & DB & AB \\
\begin{block}{(cccccc)c}
  T_1 & 0 & -L_1 & 0 & 0 & 0 & AC \\
  0 & T_2 & -L_1 & 0 & 0 & 0 & CD \\
  0 & 0 & T_3 + L_1 & 0 & 0 & -L_2 & AD \\
  0 & 0 & 0 & T_4 & 0 & 0 & DA \\
  0 & 0 & 0 & 0 & T_5 & -L_2 & DB \\
  0 & 0 & 0 & 0 & 0 & T_6 + L_2 & AB \\
\end{block}
\end{blockarray} \\
& \quad \quad \quad = \begin{blockarray}{ccccccc}
AC & CD & AD & DA & DB & AB \\
\begin{block}{(cccccc)c}
  1 & 0 & -1 & 0 & 0 & 0 & AC \\
  0 & 1 & -1 & 0 & 0 & 0 & CD \\
  0 & 0 & 2 & 0 & 0 & -1 & AD \\
  0 & 0 & 0 & 1 & 0 & 0 & DA \\
  0 & 0 & 0 & 0 & 1 & -1 & DB \\
  0 & 0 & 0 & 0 & 0 & 2 & AB \\
\end{block}
\end{blockarray}
\end{split}\label{eq:matrix}
\end{align}


Suppose we always split traffic in proportion to the values of reservation, then the reservations(on physical tunnels and \LS{}s) in a segment $ij$ are all used by the same factor $U_{ij} \in [0,1]$. Thus, $Mat \times U$ denotes the amount of reservation that will be used to carry demand, where $U \in [0,1]^{P}$. Let $D \in \mathbb{R^*}^{P}$ be the demand vector where $D_{ij}$ represents the traffic demand from $i$ to $j$. Then the solution $U^*$ for $Mat \times U = D$ will tell us how much traffic will be sent on each tunnel. Such solution always exists when the condition $Mat \times 1^P \le D$ is satisfied.

\begin{proposition}\label{prop:linear_system}
There always exists a solution $U^*$ to the linear system $Mat \times U = D$ which can be converted to a valid routing, if $Mat$ and $D$ satisfy the constraints in \LS{} model.
\end{proposition}
\cj{significance of this proposition}
For example in Figure~\ref{fig:implementation_example}, if the demand from $A$ to $B$ is 1, then we have 
\begin{align}
\begin{split}
& \begin{blockarray}{cccccc}
AC & CD & AD & DA & DB & AB \\
\begin{block}{(cccccc)}
  1 & 0 & -1 & 0 & 0 & 0 \\
  0 & 1 & -1 & 0 & 0 & 0  \\
  0 & 0 & 2 & 0 & 0 & -1 \\
  0 & 0 & 0 & 1 & 0 & 0 \\
  0 & 0 & 0 & 0 & 1 & -1 \\
  0 & 0 & 0 & 0 & 0 & 2 \\
\end{block}
\end{blockarray} \times U = 
\begin{blockarray}{cc}
  \\
\begin{block}{(c)c}
  0 & AC\\
  0 & CD\\
  0 & AD\\
  0 & DA\\
  0 & DB\\
  1 & AB\\
\end{block}
\end{blockarray}
\end{split}\label{eq:matrix}
\end{align}
and solving this linear system will give us
\begin{align}
\begin{split}
U^* = 
\begin{blockarray}{cc}
  \\
\begin{block}{(c)c}
  1/4 & AC\\
  1/4 & CD\\
  1/4 & AD\\
  0 & DA\\
  1/2 & DB\\
  1/2 & AB\\
\end{block}
\end{blockarray}
\end{split}\label{eq:matrix}
\end{align}
This solution tells us that to send 1 unit of traffic from $A$ to $B$, we can send 1/2 on $T_6$ directly, and send 1/4 on $T_1$, $T_2$ and $T_3$ so that 1/2 will be sent from $A$ to $D$, then send $1/2$ on $T_5$ from $D$ to $B$. $T_4$ is not used at all. Note that if we use the routing scheme described in \S\ref{sec:local_LS_scheme}, we will end up the exact same way of using the tunnels. This is because $Mat_1$ is an upper triangular matrix, and proportional distribution is the procedure to solve this linear system. In fact, we have the below proposition. \cj{this avoids topological sort, but not sure if it is the right way to do.}

\begin{proposition}\label{prop:topological_assumption} If the reservation matrix can be organized as an upper triangular matrix, a local proportionally
distributed routing scheme works for \LS{} model. 
\end{proposition}

If we include $L_3$($DA$,$AB$) from $D$ to $B$ in the network, the reservation matrix will become

\begin{align}
\begin{split}
& Mat_{2} = 
\begin{blockarray}{ccccccc}
AC & CD & AD & DA & DB & AB \\
\begin{block}{(cccccc)c}
  T_1 & 0 & -L_1 & 0 & 0 & 0 & AC \\
  0 & T_2 & -L_1 & 0 & 0 & 0 & CD \\
  0 & 0 & T_3 + L_1 & 0 & 0 & -L_2 & AD \\
  0 & 0 & 0 & T_4 & -L_3 & 0 & DA \\
  0 & 0 & 0 & 0 & T_5+L_3 & -L_2 & DB \\
  0 & 0 & 0 & 0 & -L_3 & T_6 + L_2 & AB \\
\end{block}
\end{blockarray} \\
& \quad \quad \quad = \begin{blockarray}{ccccccc}
AC & CD & AD & DA & DB & AB \\
\begin{block}{(cccccc)c}
  1 & 0 & -1 & 0 & 0 & 0 & AC \\
  0 & 1 & -1 & 0 & 0 & 0 & CD \\
  0 & 0 & 2 & 0 & 0 & -1 & AD \\
  0 & 0 & 0 & 1 & -1 & 0 & DA \\
  0 & 0 & 0 & 0 & 2 & -1 & DB \\
  0 & 0 & 0 & 0 & -1 & 2 & AB \\
\end{block}
\end{blockarray}
\end{split}\label{eq:matrix}
\end{align}

We can't organize the matrix to make it an upper triangular matrix because $DB$ and $AB$ are using each other. Thus, proportional distribution can not solve the linear system $Mat_2 \times U = D$. But we can still solve this linear system in a centralized controller, then deploy the solution. For example, if we want to send 1 unit of traffic from $A$ to $B$, and 1 unit of traffic from $D$ to $B$, we will have the demand vector as
\begin{align}
\begin{split}
D(AB) = 
\begin{blockarray}{cc}
  \\
\begin{block}{(c)c}
  0 & AC\\
  0 & CD\\
  0 & AD\\
  0 & DA\\
  0 & DB\\
  1 & AB\\
\end{block}
\end{blockarray},
D(DB) = 
\begin{blockarray}{cc}
  \\
\begin{block}{(c)c}
  0 & AC\\
  0 & CD\\
  0 & AD\\
  0 & DA\\
  1 & DB\\
  0 & AB\\
\end{block}
\end{blockarray}
\end{split}\label{eq:matrix}
\end{align}
By solving the linear system $Mat_2U=D(AB)$ and $Mat_2U=D(DB)$, we will get
\begin{align}
\begin{split}
U^*(AB) = 
\begin{blockarray}{cc}
  \\
\begin{block}{(c)c}
  1/3 & AC\\
  1/3 & CD\\
  1/3 & AD\\
  1/3 & DA\\
  1/3 & DB\\
  2/3 & AB\\
\end{block}
\end{blockarray},
U^*(DB) = 
\begin{blockarray}{cc}
  \\
\begin{block}{(c)c}
  1/6 & AC\\
  1/6 & CD\\
  1/6 & AD\\
  2/3 & DA\\
  2/3 & DB\\
  1/3 & AB\\
\end{block}
\end{blockarray}
\end{split}\label{eq:matrix}
\end{align}
Removing the loops in the solution(e.g., $AD$ and $DA$ can cancel each other's value), for each tunnel $l \in T(s,t)$, we can deploy $a_lU^*(AB)_{st}$ as the weight to route from $s$ to $t$ and $a_lU^*(DB)_{st}$ as the weight to route from $D$ to $B$.

%  \begin{figure}[t]
%	\centering
%        
%	    \includegraphics[ trim={6.5cm 8.6cm 16cm 8cm}, clip, width=0.48\textwidth]{figures/implementation_example_bad.pdf}
%        \label{fig:implementation_example_bad}

%    \caption{A topology with three \LS{}s $(AC,CD,DB)$, $(AE,EC)$ and $(CA,AB,BD)$ where recursion may occur in routing. }
%        \label{fig:implementation_example_bad}
%\end{figure}


